Hierarchical Experimentalist Agents

Large language models (LLMs) are increasingly used to act in the real world and augment human decision-making, yet most systems rely on parametric knowledge acquired through imitation, optionally improved by post-training, retrieval, or search over fixed data. This paradigm struggles in novel domains or on complex queries that require information unavailable from prior knowledge alone; knowing the laws of physics, for example, does not by itself enable reliable reasoning or long-horizon actions in a complex physical system. We argue that agents need active experimentation: the ability to gather targeted query-specific evidence, discover general principles of unseen environments, and convert interaction experience into reusable skills. We introduce Hierarchical Experimentalist Agents (HExA), an in-context, experiment-centric self-improvement framework that (1) iteratively designs and refines query-relevant experiments, (2) incrementally distills experience into reusable and composable skills that accelerate experimentation within and across tasks, and (3) integrates experimental evidence to act or answer queries. HExA can work with any LLM including frontier black-box models, and requires no external supervision, oracle solutions, or offline data. We evaluate HExA on multi-step reasoning, interactive partially observable games, and physics law discovery tasks. To further evaluate when active experimentation is necessary, we introduce Interphyre, a set of hard procedural physics tasks where we enable tool-calling and intervention APIs. Current frontier LLMs including GPT-6 Astra fail in these settings: on the most challenging Interphyre tasks, we show that HExA can enable such models to near 100% success. Moreover, HExA improves token efficiency compared to naive agentic and memory baselines and enables generalization via hierarchical skill transfer from easier to harder tasks.

==> appendices/app_HeXA.tex <==
% ============================================================
%  Appendix: HExA
% ============================================================
\section{HExA: More Methodological Details}
\label{app:hexa}





\subsection{Overview}
\label{sec:overview}
 
Many agentic tasks require an LLM to go beyond its parametric knowledge and actively interact with an environment to gather the instance-specific information needed to complement existing parametric knowledge in complex queries or experimental tasks; or to fundamentally interact and experiment in an unseen domain to reason, act and correctly complete some novel user task or query beyond the model's existing parametric knowledge and capabilities.
An intuitive paradigm for learning in such settings and retaining useful reusable information is via inference-time in-context skill augmentation: distilling reusable strategies and common pitfalls from \textbf{\emph{interaction experience and active experimentation}} into compact natural-language \textbf{\emph{skills}} that are reusable in the agent's context at the start of each new episode, amortizing cost of exploration and skill reuse in newer tasks or domains.
Turning this idea into a working self-improving framework, however, faces three difficulties: (1) the agent has no access to oracle solutions, expert demonstrations, or optimal offline data from the task family; (2) there is no human or oracle guided skills to start with and no external reward model or verifier beyond the interaction feedback on the unseen domain to bootstrap the learning; and (3) the skill library must be autonomously evolved and remain compact and bounded to fit within the agent's context window while still capturing the most useful knowledge.

In our paper, we introduce \textbf{\textit{HExA}} (Hierarchical Experimentalist Agents), shown in Figure~\ref{fig:hexa_main}, a training-free, in-context reinforcement learning framework that autonomously discovers, evolves, and transfers reusable skills without parameter updates, external feedback, or human annotation.
At its core, HExA operates a two-agent loop over a sequence of rounds (\ref{sec:framework}): an \emph{actor} $\pi_{\mathrm{act}}$ actively experiments with the environment through a tool-call interface, generating trajectories of successes and failures; an \emph{evolver} $\pi_{\mathrm{ev}}$ reads batches of these trajectories, contrasts high-reward against low-reward episodes, and distills the result into an evolving external \emph{skill bank} $\mathcal{K}$ via a two-phase contrastive and failure-analytic distillation process (\ref{sec:distillation}).
A reward-weighted \emph{retriever} (\ref{sec:retrieval}) selects the most relevant skills and injects them into the actor's context before each subsequent episode, so that the cost of exploration is amortized across problem instances rather than paid from scratch each time.


A key risk in any iterative skill-evolution loop is \emph{skill drift}: the evolver may accumulate increasingly narrow strategies that overfit to the particular instances seen so far, while discarding general principles that would transfer to new instances.
To address this, HExA supports multiple initialisation and update regimes (\ref{sec:regimes}) that control the balance between retaining proven skills and incorporating new evidence, ranging from a frozen offline bank to a fully online evolution strategy.
Beyond within-task learning, HExA further enables \emph{cross-task skill transfer} (\ref{sec:transfer}): skill banks evolved on one or more source task families are re-grounded by the evolver onto a structurally related target task, enabling zero-shot transfer with no target-task interaction.
In this way, HExA autonomously constructs task-specific skills that can be deployed with any frozen LLM at inference time to enable in-context self-improvement without weight updates.







\subsection{Problem Formulation}
\label{sec:problem-formulation}

We consider a task family $\ell$ consisting of a set of task instances $\{(\ell, s_j)\}$, where each instance is identified by an index $s_j$ (e.g., a random seed) that determines the specific configuration of the environment (geometry, parameters, initial conditions).
The agent interacts with each instance through a tool-call interface exposing a set of tools $\mathcal{F}$, and the environment defines a binary success predicate $\textsc{Goal}_\ell$ that evaluates the outcome of a completed simulation.
 
At each iteration $t$ of an episode, the agent observes the conversation history $h_t = (o_0, a_1, o_1, \ldots, a_{t-1}, o_{t-1})$, where $o_i$ is an observation returned by a tool call and $a_i \in \mathcal{F}$ is a tool invocation, and selects the next action according to its policy $\pi$.
The episode terminates after at most $T$ iterations or when the agent issues a terminal action.
We define a success indicator $y_j$ for task instance $s_j$ as:
%
\begin{equation}
\label{eq:success}
y_j(\pi;\, \ell,\, \mathcal{G}) \;=\; \mathbb{I}\bigl[\textsc{Goal}_\ell\!\left(\textsc{Sim}(\tau_j)\right) = \text{true}\bigr], \qquad \tau_j \sim \pi(\cdot \mid \ell,\, s_j,\, \mathcal{G}),
\end{equation}
%
where $\tau_j$ is the trajectory generated by $\pi$, $\textsc{Sim}$ runs the environment simulation to completion, and $\mathcal{G}$ is an optional skill context.
 
Our goal is to maximize the solve rate across instances of $\ell$ without any parameter updates to $\pi$.
To this end, we introduce a natural-language \emph{skill bank} $\mathcal{K}$, a structured collection of reusable strategies and common-mistake records that is prepended to the agent's system prompt at the start of each episode:
%
\begin{equation}
\label{eq:skill-augmented}
\tau_j \sim \pi(\cdot \mid \ell,\, s_j,\, \mathcal{G}), \qquad \mathcal{G} = \textsc{Retriever}(\mathcal{K},\, \ell,\, M,\, N),
\end{equation}
%
where $\textsc{Retriever}$ selects the top-$M$ skills by reward and top-$N$ mistakes from $\mathcal{K}$.
The skill bank $\mathcal{K}$ is constructed and evolved entirely through HExA's actor-evolver loop (Section~\ref{sec:framework}), with no human annotation, external teacher, or access to oracle solutions.
Each trajectory is additionally assigned a scalar reward $r(\tau_j) \in [-1, +1]$ that reflects both outcome and efficiency (Eq.~\ref{eq:reward}), providing the evolver with a richer learning signal than the binary success indicator alone.

\subsection{The HExA Framework}
\label{sec:framework}


\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{figures/Feedback_Loop.png}
  \caption{%
    \textbf{The \textsc{HExA} actor-evolver loop.}
    The actor receives distilled skills in its system prompt and runs on
    physics puzzles, producing trajectories annotated with rewards
    (successes~\cmark, failures~\xmark).
    The Skill Evolver analyzes these trajectories and curates the
    evolving Skill Bank: skills (max~M) are merged, pruned, or promoted
    by reward signal, and common mistakes (max~N) are updated accordingly.
    Each skill carries a generation index tracking its lineage across
    evolution rounds (Eq.~\ref{eq:confidence}).
    The updated bank is injected back into the actor's system prompt for
    the next round, closing the loop.
  }
  \label{fig:hexa_loop}
\end{figure}



\begin{figure}[h]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/skill_hexa_catapult.png}
    \caption{Example on \texttt{catapult} with its skill bank.}
    \label{fig:running_example}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Feedback_Loop.png}
    \caption{\textsc{HExA} actor--evolver--retriever loop.}
    \label{fig:hexa_loop2}
  \end{subfigure}
  \caption{%
    \textbf{\textsc{HExA} learns reusable skills through an actor--evolver--retriever loop.}
    \textbf{(a)}An example on \texttt{catapult} level illustrates the kind of physics reasoning skills \textsc{HExA} distills.
    \textbf{(b)} In each round, the actor generates reward-tagged trajectories, the evolver
    updates the skill bank, and the retriever injects the most relevant skills back into the
    actor for the next attempt.
  }
  \label{fig:hexa_overview_main}
\end{figure}


HExA instantiates the skill-augmented policy of Eq.~\ref{eq:skill-augmented} through a two-agent architecture operating over a sequence of \emph{rounds}.
An \textbf{actor} $\pi_{\mathrm{act}}$ (any tool-augmented LLM) generates trajectories by interacting with the environment, while an \textbf{evolver} $\pi_{\mathrm{ev}}$ (which may be the same model) reads batches of actor trajectories and distills them into the skill bank $\mathcal{K}$.
At the start of each new episode, the $\textsc{Retriever}$ selects the most relevant skills from $\mathcal{K}$ and injects them into the actor's context, so that each subsequent trajectory benefits from the accumulated experience of all prior ones.
 
This loop can be viewed as an instantiation of in-context reinforcement learning~\citep{laskin2022context,moeini2025survey}: the agent's policy improves over rounds through context augmentation rather than weight updates, and the skill bank serves as a compressed, curated form of the cross-episode context that classical in-context RL methods maintain in raw form.
Unlike standard in-context RL, however, HExA does not require pretraining on a task distribution; it operates on a single frozen model and learns from scratch on each task family.







\subsubsection{Trajectory Reward}
\label{sec:reward}

Not all trajectories are equally informative. A fast, decisive solve reveals a high-reward strategy; a failure that explored extensively yields richer material for the evolver than one that abandoned the episode after a single attempt.
To communicate this signal, we assign a scalar reward $r(\tau) \in [-1, +1]$ to each trajectory $\tau$, reflecting both \emph{outcome} (success or failure) and \emph{efficiency} (iteration count $t$ at termination):
%
\begin{equation}
r(\tau) \;=\;
\begin{cases}
+1.00 & \text{success},\; t \le 3 \\
+0.75 & \text{success},\; t \le 7 \\
+0.50 & \text{success},\; t \le 15 \\
+0.25 & \text{success},\; t \le T \\[3pt]
-0.50 & \text{failure},\; t \ge 10 \\
-0.75 & \text{failure},\; t < 10
\end{cases}
\label{eq:reward}
\end{equation}
%
The asymmetry in failure penalties is deliberate: an agent that explores extensively before failing produces richer interaction records for the evolver to extract partial skills and diagnose mistakes.
 



\begin{algorithm}[h]
\caption{HExA}
\label{alg:HeXa_algo_app}
\DontPrintSemicolon
\KwIn{Base agent $\pi_{\text{act}}$, evolver $\pi_{\text{ev}}$, level $\ell$,
      regime $\mathcal{R} \in \{\text{Offline}, \text{Off2On}, \text{Online}\}$,
      update strategy $\mathcal{U} \in \{\text{Evolution}, \text{Iterative}, \text{None}\}$,
      rounds $R$, trajectories per round $x$, initial batch size $N_0$,
      retrieval sizes $M, N$}
\KwOut{Final skill bank $\mathcal{K}_R$ and per-round trajectories $\{\mathcal{T}^{(n)}\}_{n=1}^{R}$}

\tcp{Stage 1: Initialise skill bank $\mathcal{K}_0$}
\uIf{$\mathcal{R} \in \{\text{Offline},\ \text{Off2On}\}$}{
    Collect batch $\mathcal{T}_0$ of $N_0$ trajectories from $\pi_{\text{act}}$ on $\ell$\;
    $\mathcal{K}_0 \gets \text{Evolver}(\emptyset, \mathcal{T}_0)$ \tcp*{teacher-driven distillation}
}
\Else{
    $\mathcal{K}_0 \gets \emptyset$ \tcp*{cold start (Online)}
}

\BlankLine
\tcp{Stage 2: Iterative rounds of generation, distillation, and update}
\For{$n = 1, 2, \dots, R$}{
    $\mathcal{G}_n \gets \text{Retriever}(\mathcal{K}_{n-1}, \ell, M, N)$ \tcp*{retrieve top-$M$ skills, top-$N$ mistakes}
    $\mathcal{T}^{(n)} \gets \emptyset$\;
    \For{$i = 1, \dots, x$}{
        $\tau_i \gets \pi_{\text{act}}(\ell \mid \mathcal{G}_n)$ \tcp*{run skill-augmented agent}
        $r(\tau_i) \gets \textsc{Reward}(\tau_i)$ \tcp*{Eq.~\ref{eq:reward}}
        $\mathcal{T}^{(n)} \gets \mathcal{T}^{(n)} \cup \{(\tau_i, r(\tau_i))\}$\;
    }
    \uIf{$\mathcal{R} = \text{Offline}$}{
        $\mathcal{K}_n \gets \mathcal{K}_{n-1}$ \tcp*{frozen bank}
    }
    \uElseIf{$\mathcal{U} = \text{Evolution}$}{
        $\mathcal{K}_n \gets \text{Evolver}(\mathcal{K}_{n-1}, \mathcal{T}^{(n)})$ \tcp*{merge, revise, prune}
    }
    \ElseIf{$\mathcal{U} = \text{Iterative}$}{
        $\mathcal{K}_n \gets \text{Evolver}(\emptyset, \mathcal{T}^{(n)})$ \tcp*{re-distil from new trajectories only}
    }
}
\KwRet{$\mathcal{K}_R,\ \{\mathcal{T}^{(n)}\}_{n=1}^{R}$}
\end{algorithm}



\subsubsection{Skill Distillation from Experimentation on Self-Proposed Hypotheses}
\label{sec:distillation}


At each round $n$, the evolver $\pi_{\mathrm{ev}}$ receives the batch of trajectories $\mathcal{T}^{(n)} = \mathcal{T}^{(n),+} \cup \mathcal{T}^{(n),-}$ generated by the actor, where $\mathcal{T}^{(n),+}$ and $\mathcal{T}^{(n),-}$ denote the successful and failed subsets respectively, each annotated with its scalar reward.
The evolver performs a two-phase distillation to extract complementary forms of knowledge.
 
\paragraph{Phase 1: Contrastive skill extraction.}
Given the full batch $\mathcal{T}^{(n)}$ with reward annotations, the evolver contrasts high-reward trajectories against low-reward ones to identify the strategies and insights that distinguish success from failure.
This produces 4--6 \emph{strategy skills}, each consisting of a short title, a 2--3 sentence natural-language principle describing the underlying mechanism, and an applicability predicate specifying when the skill is relevant.
The evolver is instructed to weight its analysis by reward: skills derived from fast, efficient solves are treated as more reliable than those from trajectories that barely succeeded.
 
\paragraph{Phase 2: Mistake and partial-skill extraction.}
Focusing on the failure subset $\mathcal{T}^{(n),-}$, the evolver produces two complementary outputs.
\emph{Common mistakes} are structured records $\mu = (\delta, \rho, \alpha)$, where $\delta$ describes the error, $\rho$ identifies its root cause (the broken causal belief that led to it), and $\alpha$ specifies a concrete corrective strategy.
\emph{Partial skills} capture correct reasoning steps that appeared \emph{within} otherwise failed trajectories: an agent may have identified a valid strategy or correctly diagnosed a mechanism before making an error elsewhere.
These partial successes cannot be discovered from successful trajectories alone and are a distinctive source of learning signal in HExA.


 


\subsubsection{Skill Bank}
\label{sec:skillbank}

Distilled knowledge is stored in the skill bank $\mathcal{K}$ with two collections, both indexed by task family: a set of \emph{skills} (reusable strategy and principles) and a set of \emph{mistakes} (patterns recording and describing recurring failure modes to avoid).
Each skill carries a reward label, computed from the interaction rewards of the trajectories that demonstrated it:
%
\begin{equation}
r_k \;=\; \operatorname{clamp}\!\left(\frac{\bar{r}_{\mathrm{src}} + 1}{2},\; 0.1,\; 1.0\right),
\label{eq:confidence}
\end{equation}
%
where $\bar{r}_{\mathrm{src}}$ is the mean reward of the source trajectories from which the skill was extracted.
Skills derived from fast, efficient solves carry higher rewards; skills surfaced from partial reasoning within failed trajectories carry lower rewards but may still encode valuable discoveries.
The skill bank is hard-capped at $M_{\max}$ skills and $N_{\max}$ mistakes per task family to prevent the injected context from growing without bound and to force the evolver to prioritize the most informative knowledge during evolution rounds. This is where the reward labels and the creation of hierarchical skills, help in improving the skill bank even though it is capped at a maximum number of skills.
 





\subsubsection{Skill Retrieval and Injection}
\label{sec:retrieval}

At the start of each episode, the $\textsc{Retriever}$ selects the top-$M$ skills from $\mathcal{K}$ sorted by reward $r_k$ and the top-$N$ mistakes for the relevant task family, and injects them into the actor's system prompt as the structured skill context $\mathcal{G}$ defined in Eq.~\ref{eq:skill-augmented}.
The actor receives this block alongside the standard task description and tool documentation, and is free to use or disregard individual skills based on its own reasoning about the current instance.
This injection mechanism is deliberately simple: it adds a fixed-size prefix to the prompt rather than modifying the agent's architecture or decoding procedure, making HExA compatible with any tool-augmented LLM, including closed-source API-served models.







\subsubsection{Initialisation, Update Regimes, and Full Algorithm}
\label{sec:regimes}


The loop described above admits several configurations that vary along two orthogonal axes:
how the skill bank is \emph{initialised} before evaluation begins, and how it is
\emph{updated} between rounds.
Algorithm~\ref{alg:HeXa_algo_app} summarizes the full procedure; we now describe the design axes it parameterizes.


\paragraph{Initialisation.}
In the \textbf{Offline} and \textbf{Offline-to-Online} (Off2On) regimes, a warm-start batch of $N_0$ trajectories is collected from the base actor (without any skill context) and distilled into an initial bank $\mathcal{K}_0$ via $\text{Evolver}(\emptyset, \mathcal{T}_0)$ (Algorithm~\ref{alg:HeXa_algo_app}, lines~3--4). In the \textbf{Pure Online} regime, the bank starts empty ($\mathcal{K}_0 = \emptyset$) and the agent must bootstrap skills entirely from its own online interactions (line~6).
 
\paragraph{Update strategy.}
Given trajectories from round $n$, the bank can be updated in two ways.
Under \textbf{Evolution}, the evolver receives both the current bank and the new trajectories, producing $\mathcal{K}_n = \text{Evolver}(\mathcal{K}_{n-1}, \mathcal{T}^{(n)})$ by merging, revising, or pruning existing skills in light of new evidence (line~17).
Under \textbf{Iterative Replacement}, the evolver distills $\mathcal{K}_n = \text{Evolver}(\emptyset, \mathcal{T}^{(n)})$ purely from the new trajectories, discarding all prior skills (line~19).
In the Offline regime, the bank is frozen after initialisation ($\mathcal{K}_n = \mathcal{K}_{n-1}$, line~15).









 
Crossing these axes yields five concrete variants: Offline (static bank), Off2On with Evolution, Off2On with Iterative Replacement, Pure Online with Evolution, and Pure Online with Iterative Replacement.
We compare these empirically in \ref{sec:experiments}.


Finally we see that the Off2On~+~Evolution variant works best across all settings and is thus the variant that we generally refer to as HExA in the rest of the paper.




\subsection{Cross-Task Skill Transfer}
\label{sec:transfer}
 
The skill banks produced by HExA encode task-family-specific strategies, but the underlying principles are often more general: momentum conservation, lever mechanics, collision geometry, and similar structural insights recur across task families that share physical or procedural primitives.
HExA exploits this by synthesizing a \emph{cross-task skill bank} for a target task family from the evolved banks of one or more source families, with no target-task trajectories required.
 
Given source banks $\mathcal{K}_{\ell_1}, \ldots, \mathcal{K}_{\ell_S}$ and a textual description of the target task family $\ell^*$, the evolver receives all source skills together with the target description and is prompted to:
%
\begin{enumerate}[leftmargin=1.5em,itemsep=2pt]
\item identify which source skills encode principles that are structurally relevant to the target (based on shared physical or procedural primitives),
\item re-ground each selected principle in the entities and mechanics of the target scene, and
\item calibrate reward based on how directly the principle transfers (skills corroborated by multiple source banks receive higher reward).
\end{enumerate}
%
The synthesised bank $\mathcal{K}_{\ell^*}$ is then injected into the actor's context via the same $\textsc{Retriever}$ mechanism as within-task skills.
This enables zero-shot transfer: the actor attempts the target task with the benefit of cross-task skills but without having seen any target-task trajectories.
 
Importantly, cross-task transfer and within-task skill evolution are complementary.
The synthesised bank can serve as the initialisation $\mathcal{K}_0$ for a subsequent within-task HExA run, combining the benefits of transferred knowledge with task-specific refinement.





\subsection{Design Principles}
\label{sec:design-principles}
 
Several design choices in HExA merit explicit discussion.
 
\paragraph{Domain agnosticism.}
Nothing in the framework above assumes a particular domain.
The actor interacts with the environment through a generic tool-call interface; the evolver reads trajectory text and produces structured JSON.
The only domain-specific components are the tool suite exposed by the environment and the system prompt describing the task, both of which are inputs to HExA rather than parts of its architecture.
We instantiate and evaluate HExA on physics puzzles in \S\ref{sec:experiments}, but the same framework applies to any setting where an agent must learn from sequential interactions with an environment.

\paragraph{Reward Function Agnostic.}
As we have shown previously in our experiments, rewards from environment interactions and shaped according to the needs of the user help HExA more. But the evolver can guide skill creation and learning even without it. So this reward agnostic nature of HExA make it widely applicable in domains where even environment reward might not be present. Moreover in cases where there is presence of such rewards and additional feedback, we can plug in any reward function to further guide skill acquisition either guided by users or designed by the LLM evolver itself.
 
\paragraph{No weight updates.}
HExA is entirely in-context: neither the actor nor the evolver undergoes any parameter updates.
All adaptation occurs through the evolving skill bank, which modifies the actor's behavior by changing the textual context it conditions on.
This makes HExA compatible with closed-source, API-served models and avoids the computational cost and catastrophic-forgetting risks of fine-tuning.
 
\paragraph{Hierarchical skill structure.}
The skills in $\mathcal{K}$ are hierarchical in two senses.
First, they abstract over low-level actions (specific tool calls and parameter values) into high-level strategy descriptions, compressing lengthy trajectories into concise principles.
Second, skills are learned iteratively while the agent has access to previously distilled skills, so later skills implicitly build on earlier ones.
The evolver may revise a skill in light of new evidence or merge two complementary skills into a more general one, producing a form of meta-learning: the agent learns not just strategies but \emph{how to learn strategies} from interactions.
 





==> appendices/app_ablation.tex <==
% ============================================================
%  APPENDIX — place inside your \appendix block
% ============================================================
 
\section{Prompt Ablation Study: Full Results}
\label{app:ablation}

Table~\ref{tab:ablation_legend} describes the four ablation levels and
the components removed at each step.

% --- Legend table -----------------------------------------
\begin{table}[h]
\centering
\small
\caption{%
  Ablation levels and the prompt components removed at each step.
  Removals are cumulative: each level also removes everything
  stripped at earlier levels.
}
\label{tab:ablation_legend}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{clp{7cm}}
\toprule
\textbf{Level} & \textbf{Name} & \textbf{Component removed} \\
\midrule
Full
  & Full prompt
  & Nothing removed; all hints enabled. \\
\addlinespace[3pt]
Abl.\ 1
  & No strategy tips
  & Explicit tool-invocation order and collision-direction
    instructions (e.g.\ which side of the green ball to strike
    in order to push it toward the target). \\
\addlinespace[3pt]
Abl.\ 2
  & No physics rules
  & Remaining physics heuristics and placement guidelines
    (e.g.\ recommended horizontal offsets; side-of-green-ball
    placement rules for reliable lateral impulse). \\
\addlinespace[3pt]
Abl.\ 3
  & No tool feedback
  & Rich observation outputs: corrective offset messages on
    invalid placements (e.g. how much distance to move away from the overlapping object) \\
\addlinespace[3pt]
Abl.\ 4
  & No geometry tool
  & Level-specific analysis tool
    (\texttt{compute\_gap\_analysis} for \textit{Down to Earth};
    \texttt{compute\_relative\_positions} for
    \textit{Two Body Problem}). \\
\bottomrule
\end{tabular}
\end{table}

==> appendices/app_results_final.tex <==
\section{Additional Experimental and Result Details}
\label{app:exp_res_final}

\input{tables/interphyre_main}
 
\input{tables/reward_ablation_main}

\input{tables/variants_compact}

\input{tables/external_compact}
\input{tables/transfer_merged}






\subsection{Instantiation of HExA}
\label{app:exp_res_final_instantiation}

\textsc{HExA} is also flexible enough to ingest additional experimental evidence
such as trajectory rewards, which are a function of outcome reward and efficiency
(Appendix~\ref{sec:reward}), to further guide skill evolution and retrieval. The
skill reward label $r_k$ is in turn a function of the trajectory rewards of the
trajectories that invoked the skill,
\begin{equation}
\label{eq:weight}
r_k = \operatorname{clamp}\!\left(\frac{\bar{r}_{\mathrm{src}}+1}{2},\,0.1,\,1.0\right),
\end{equation}
where $\bar{r}_{\mathrm{src}}$ is the mean reward of those source trajectories.
Depending on experimental settings, users can define any trajectory reward and skill reward; HExA as a framework is agnostic of these choices. We also tried skill evolution without rewards, using the evolver LLM's prior knowledge itself to guide skill bank update, ignoring the useful environment grounded rewards. Our ablations in Table~\ref{tab:ablations}c show that reward labeled skill banks perform the best. Thus, our default experimental setting for \textsc{HExA} is Off2On~+~Evolution with reward labeled skills.





\subsection{HExA on Interphyre Details}



\paragraph{Does active experimentation and skill creation help agents solve complex tasks?}
On levels where a single \textsc{ReAct} trajectory fails, we test whether
distilling interaction traces into an evolving skill bank improves over both
baselines that accumulate no reusable skills (\textsc{Zero-shot}, \textsc{ReAct},
Reflexion) and external-memory baselines that retain past episodes rather than
distilling them (Episodic RAG, MemRL). On the two hardest levels, where the base
Claude Sonnet model makes little or no progress, \textsc{HExA} reaches
$82.7\pm11.4\%$ on \texttt{catapult} and $96.0\%$ on
\texttt{pass\_the\_parcel}, compared with $0.0\%$/$0.0\%$ for
\textsc{Zero-shot}, $11.0\pm3.0\%$/$20.0\%$ for \textsc{ReAct},
$21.3\pm2.5\%$/$32.0\%$ for Reflexion, $60.8\%$/$60.0\%$ for
Episodic RAG, and $33.3\%$/$46.0\%$ for MemRL
(Table~\ref{tab:interphyre}). Figure~\ref{fig:catapult45_simframes} shows a
representative \texttt{catapult} seed where retrieved skills guide
\textsc{HExA} to a solution in a handful of interactions while \textsc{ReAct}
exhausts its budget.

The pattern also holds for weaker open-weight models. On
\texttt{down\_to\_earth}, \textsc{HExA} raises Qwen-2.5-7B from
$63.3\pm3.4\%$ to $82.7\pm5.2\%$ and Qwen-2.5-3B from
$8.3\pm0.9\%$ to $23.3\pm0.9\%$; on
\texttt{two\_body\_problem}, it raises them from $12.0\%$ to
$50.0\pm3.3\%$ and from $7.3\pm0.9\%$ to $12.0\%$, respectively.
Storing experience alone is not sufficient: on \texttt{down\_to\_earth} with
Qwen-2.5-7B, Episodic RAG and MemRL reach $42.7\%$ and $36.0\%$,
respectively, below memoryless \textsc{ReAct} at $63.3\%$. Reflexion reaches
$76.0\%$ there, but requires a second trial on each seed. These comparisons
indicate that the improvement comes from distilling prior interactions into
reusable strategies rather than from additional retries or merely including past
experience in the prompt.


\paragraph{Can \textsc{HExA} leverage learned skills for more efficient
exploration and experimentation?}
Spending more compute on interaction does not by itself raise task success, so we
record average turns per seed as an efficiency proxy alongside solve rate
(Figure~\ref{fig:cum_iter_both}, Table~\ref{tab:catapult_cost}).
Accuracy and cost move together: \textsc{HExA} lowers the average from $22.9$
turns under \textsc{ReAct} to $12.5\pm0.9$ on \texttt{catapult}, roughly
$45\%$ fewer, and from $18.7$ to $5.8$ on \texttt{pass\_the\_parcel}.
Thus, the additional successes require less interaction per instance rather than
more.

\textsc{HExA} is also the cheapest persistent memory to carry, injecting
$2{,}392$ tokens per episode on \texttt{catapult}, compared with $6{,}706$
for Episodic RAG and $8{,}135$ for MemRL
(Table~\ref{tab:interphyre}). The skill bank has fixed capacity, whereas storing
rollouts scales with the rollout cap rather than with the distilled knowledge.
Converting past experience into a reusable skill bank therefore amortizes the
cost of future experimentation instead of re-paying it each episode.

Figures~\ref{fig:build_then_freeze} and~\ref{fig:astra_catapult} trace the
protocol end to end on \texttt{catapult}: the bank accumulates over the training
seeds, is then frozen, and is evaluated against the same baselines on disjoint
held-out seeds for Claude Sonnet and GPT-6-Astra. The ordering established during
bank construction persists after freezing, while the stronger GPT-6-Astra actor
requires fewer rounds to acquire the useful skills.


\paragraph{How does in-context skill learning compare with gradient-based adaptation?}
The advantage also appears against a weight-update baseline. At a matched
50-unique-seed budget, GRPO fine-tuning Qwen-2.5-3B reaches $20\%$ on
\texttt{down\_to\_earth} and $6\%$ on
\texttt{two\_body\_problem}, compared with \textsc{HExA}'s $23.3\%$ and
$12.0\%$, respectively (Appendix~\ref{app:results:grpo}). Skills distilled
from early trajectories become immediately available to subsequent episodes
through context, whereas gradient-based adaptation must accumulate rollout signal
before the same information is encoded in model weights. With additional training,
GRPO eventually closes or reverses this low-data gap; complete training curves
and settings are reported in Appendix~\ref{app:results:grpo}.


\paragraph{Which ingredients drive improvements in \textsc{HExA}?}
Using the instantiation axes defined in Section~\ref{sec:instantiation}, we study
how each one aids learning from experimentation.



\paragraph{Can \textsc{HExA} leverage learned skills for more efficient
exploration and experimentation?}
Spending more compute on interaction does not by itself raise task success, so we
record the average number of turns per seed as an efficiency proxy alongside
solve rate (Figure~\ref{fig:cum_iter_both}, Table~\ref{tab:catapult_cost}).
Accuracy and cost move together: \textsc{HExA} lowers the average from $22.9$
turns under \textsc{ReAct} to $12.5 \pm 0.9$ on \texttt{catapult}, roughly $45\%$
fewer, and to $5.8$ from $18.7$ on \texttt{pass\_the\_parcel}, so the extra
successes come with less computation per instance rather than more. It is also
the cheapest memory to carry, at $2{,}392$ injected tokens per episode against
$6{,}706$ and $8{,}135$ for the episodic baselines
(Table~\ref{tab:interphyre}); the bank is a fixed size, so its cost is constant
in the number of episodes played, whereas storing rollouts scales with the
rollout cap rather than with anything learned. Converting past experience into a
reusable skill bank therefore amortizes the cost of future experimentation
instead of re-paying it each episode.
\paragraph{Which ingredients drive improvements in \textsc{HExA}?}
Using the instantiation axes defined in Section~\ref{sec:instantiation}, we study
how each one aids learning from experimentation.





\subsection{Detailed Results of HExA on Other Benchmarks and Tasks}


\label{app:results:external}

\paragraph{Do the gains from experimentation and skill reuse hold beyond
\textsc{InterPhyre}?}
We repeat the same frozen-bank protocol on three external benchmark families:
interactive games, reasoning and planning, and open-ended scientific discovery,
against the same non-experimental and external-memory baselines.
Figure~\ref{fig:external_bench} summarizes each family as one score per actor,
averaged over that family's environments; Table~\ref{tab:external} reports the
per-task values. Token budgets, per-episode breakdowns, and exact paired tests are
reported in Appendices~\ref{app:results:external}--\ref{app:results:discovery}.

Across all four actor groups, \textsc{HExA} is the highest-performing memory
method. Neither episodic baseline is consistently beneficial:
\textsc{Episodic RAG} falls below no memory on the interactive games with
\texttt{gpt-oss-120b}, while \textsc{MemRL} falls below no memory on
\textsc{DiscoverPhysics}. Thus, each episodic-memory method imposes a cost in at
least one family, whereas the distilled bank improves every reported actor group.


\paragraph{Do distilled skills help when each instance is replayed?}
For the interactive games, each instance is played for three episodes with the
hidden task held fixed. Figure~\ref{fig:external_bench} reports \texttt{any},
the fraction of instances solved in at least one of the three episodes; the full
results additionally report \emph{ep3}, success on the final episode, which
measures how much the agent carries from its earlier attempts on the same instance.

The bank improves both actors and is also the cheapest persistent memory.
On Mastermind, \textsc{HExA} injects $971$ tokens per episode compared with
$1{,}957$ for Episodic RAG and $3{,}416$ for \textsc{MemRL}; on Maze, the
corresponding costs are $429$, $5{,}457$, and $7{,}027$ tokens.
Thus, the episodic baselines inject between $3.5\times$ and $16\times$ as much
context as the skill bank in these settings.

Storing episodes verbatim does not consistently transfer across instances:
a retrieved transcript from a previous instance can displace the actor's own
cross-episode observations rather than supplement them with a reusable abstraction.
\textsc{MemRL} is statistically indistinguishable from no memory in all three
settings in which it was run. In contrast, \textsc{HExA} compresses prior
experience into a much smaller set of strategies that can be reused across
instances while leaving more context available for the current interaction.


\paragraph{Do distilled skills help on reasoning and planning tasks?}
Every method receives the same rollout budget, so the comparison differs only in
what information is carried between items. \textsc{HExA} improves the frozen actor
on all four tasks, raising mean accuracy from $0.518$ with no memory to $0.744$,
and is the only memory method that improves every task rather than trading gains
on one task against losses on another.

Episodic RAG and \textsc{MemRL} reach mean accuracies of $0.606$ and $0.556$,
respectively. Storing previous rollouts therefore recovers part of the benefit,
but not most of it, despite the equal rollout budget. The additional gain from
\textsc{HExA} comes from making distilled strategies immediately available to
later items through context rather than carrying the original trajectories
themselves.


\paragraph{Do distilled skills help when the task is open-ended scientific discovery?}
On \textsc{DiscoverPhysics}, the skill bank contains experimentation strategies
rather than task solutions. This produces the largest aggregate margin among the
three external families: the judge's explanation score rises from $0.540$ with
no memory to $0.873$ with \textsc{HExA}.

The improvement also appears under the benchmark's strict success criterion.
On \texttt{oscillator}, pass rate at the $0.90$ explanation-score gate rises from
$0/15$ to $11/15$, whereas the baseline never clears the gate. On
\texttt{circle}, the benchmark reward alone does not improve significantly.
This is not inconsistent with the explanation-score gain: the evaluator
re-optimizes the submitted parameters against the agent's own trajectories, so
an incorrect functional form can still fit the observed data well. The explanation
metric therefore exposes improvements in discovering the underlying law that the
fit-based reward may not fully reflect.



%%%%%%%%%%%%% UTSAV Version %%%%%%%%%%%%%%%



\paragraph{Do the gains from experimentation and skill reuse hold beyond
\textsc{InterPhyre}?}
We repeat the same frozen-bank protocol on three external families --- interactive
games, reasoning and planning, and open-ended scientific discovery --- against the
same non-experimental and external-memory baselines.
Figure~\ref{fig:external_bench} reports each family as one score per actor,
averaged over that family's environments; the per-environment rows it averages,
the token budgets and the exact paired tests are in
Appendices~\ref{app:results:external}--\ref{app:results:discovery}.
\textsc{HExA} is the highest bar in all four actor groups. Neither episodic
baseline manages that: \textsc{Episodic RAG} sits below no memory on the games
with \texttt{gpt-oss-120b} and \textsc{MemRL} sits below it on
\textsc{DiscoverPhysics}, so each of them costs the actor something on at least
one family while the distilled bank costs it nothing on any.

\emph{Do distilled skills help when each instance is replayed?} On the two
interactive games every instance is played for three episodes with the hidden
task held fixed, so the panel reports \texttt{any}, success on at least one of
the three; the appendix additionally reports \emph{ep3}, success on the last
episode, which measures how much an agent has learned from its own earlier
attempts on that instance. The bank lifts both actors, and it is the cheapest
memory of the three by an order of magnitude: $971$ injected tokens against
$1{,}957$ for \textsc{Episodic RAG} and $3{,}416$ for \textsc{MemRL} on
Mastermind, and $429$ against $5{,}457$ and $7{,}027$ on Maze. Storing episodes
verbatim does not transfer across instances --- a prior instance's transcript
displaces the agent's own cross-episode observations rather than supplementing
them --- and \textsc{MemRL} is statistically indistinguishable from no memory in
all three settings it was run in, while injecting between $3.5$ and $16\times$ as
many tokens as the bank.

\emph{Do they help on reasoning and planning tasks?} Every arm here is given the
same rollout budget as \textsc{HExA}, so the only difference is what each one
carries between items. The bank improves the frozen model on all four tasks,
raising the mean from $0.518$ to $0.744$, and it is the only arm that improves
every task rather than trading one against another. Both episodic baselines land
between the two, at $0.606$ and $0.556$: storing the rollouts themselves recovers
part of the gain but not most of it, even at an equal budget. What helps is the
distilled strategy, which is available to later items immediately through
context.

\emph{Do they help when the task is open-ended discovery rather than a known
goal?} On \textsc{DiscoverPhysics} the bank holds experimentation strategies
rather than solutions, and it is the widest margin of the three families,
$0.540$ to $0.873$ on the judge's explanation score. The gain is not a graded
one: pass-rate at the strict $0.90$ gate goes from $0/15$ to $11/15$ on
\texttt{oscillator}, a gate the baseline never once clears. On \texttt{circle}
reward alone does not move significantly, which is informative rather than
inconsistent: that world's evaluator re-optimises the declared parameters against
the agent's own trajectories, so a wrong functional form can still fit the data
well.




\subsection{Instantiation and Ablations}



\emph{Does skill bank initialization and update matter?} We test three initializations---\emph{Offline},
\emph{Offline-to-Online} (\emph{Off2On}), and \emph{Online}. Both Offline and
Off2On warm-start the bank from $N_0$ base-actor trajectories collected with no
skill context, distilled into a fixed skill bank
$\mathcal{K}_0=\pi_{\mathrm{ev}}(\emptyset,\mathcal{T}_0)$; Offline then freezes
the bank, whereas Off2On keeps updating it after new rollouts. Online instead
starts empty ($\mathcal{K}_0=\emptyset$) and bootstraps skills purely from the
agent's own interactions. For updates we use two strategies---\emph{Evolving} and
\emph{Iterative Replacement}. In Evolving, we pass the evolver both the current
bank and the new round's trajectories, adding, merging, revising, or pruning
skills in light of this new evidence
($\mathcal{K}_n=\pi_{\mathrm{ev}}(\mathcal{K}_{n-1},\mathcal{T}^{(n)})$).
\emph{Iterative Replacement} instead rebuilds the bank from the current rollouts
alone ($\mathcal{K}_n=\pi_{\mathrm{ev}}(\emptyset,\mathcal{T}^{(n)})$), since in
the in-context RL loop the actor has already ingested prior skills, so the new
skills carry their influence plus the novelty of the latest rollouts. We thus
have five variants of skill bank initialization and update---\textit{Off2On} or
\textit{Online} initialization $\times$ \textit{Evolution} or \textit{Iterative
Replacement} update---plus the frozen Offline bank
($\mathcal{K}_n=\mathcal{K}_{n-1}$). We ablate these settings in
Table~\ref{tab:variants_compact} and Figure~\ref{fig:training_curves}, \emph{Off2On~+~Evolution} clearly performs the best, which is the default setting for HExA in all our final experimental results.
% reaching $84.0\%$ on \texttt{catapult} and $68.0\%$ on \texttt{pass\_the\_parcel}
% against $44.0\%$ and $58.0\%$ for a pure Online start and $56.0\%$ and $48.0\%$
% for Iterative Replacement.
\setlength{\intextsep}{0pt}
\setlength{\columnsep}{10pt}
\begin{wrapfigure}[24]{r}{0.48\linewidth}
  \vspace{-\intextsep}
  \centering
  \setlength{\abovecaptionskip}{3pt}
  \setlength{\belowcaptionskip}{3pt}
  \includegraphics[width=\linewidth]{figures/variants_scatter.pdf}
  \caption{\textbf{Accuracy and cost move together, and one instantiation holds the corner on both levels.} Solve rate against mean turns to termination for every instantiation of the bank (Claude Sonnet, training seeds); colour is the instantiation, shape is the level. Cheap and accurate is the shaded upper left, and Off2On Evolving, written simply as \textsc{HExA}, is its only occupant on either level; arrows run from each level's \textsc{Zero-shot} floor to its \textsc{HExA} point. The remaining variants cluster in the middle and change order between levels. Failures count at the $25$-turn cap; the $x$ axis is compressed below $10$ turns. Solve rates match Table~\ref{tab:variants_compact}.}
  \label{fig:training_curves}
  \label{fig:catapult_var_cum_accuracy}
  \label{fig:ptp_cum_accuracy}
\end{wrapfigure}
As Table~\ref{tab:variants_compact} shows, Off2On reaches $84.0\%$ and $68.0\%$ on
\texttt{catapult} and \texttt{pass\_the\_parcel} versus $44.0\%$ and $58.0\%$ for
a pure Online start. The gap is sharpest on \texttt{catapult}, where a cold start
wastes its early rounds rediscovering the level's basic dynamics, an advantage
that shrinks once enough online experimentation has been done. The update rule
matters on both levels: evolving the existing bank with each round's new
trajectories beats rebuilding it from the current rollouts alone, $84.0\%$ vs
$56.0\%$ on \texttt{catapult} and $68.0\%$ vs $48.0\%$ on
\texttt{pass\_the\_parcel}. Round-$n$ trajectories are generated while the actor
is conditioned on $\mathcal{G}_n=\textsc{Retriever}(\mathcal{K}_{n-1},\ell,M,N)$,
so they already reflect the previous round's skills; the evolutionary update can
then refine an earlier rule, find its boundary conditions, or replace it when
later evidence contradicts it, whereas rebuilding from scratch discards what has
accumulated and amplifies overfitting to the instances seen so far.
Figure~\ref{fig:training_curves} plots accuracy against cost: the
configurations that solve more also finish sooner.


\emph{How do reward labels help learning via experimentation?} We run
\textsc{HExA} with and without the reward labels on the skill bank. In the
ablation without them, every success and failure trajectory, and every skill
distilled out of them, is treated equally, and the LLM evolver implicitly updates
the bank using its existing knowledge rather than environment feedback. Removing
the labels costs accuracy on every level we test
(details in Figure~\ref{fig:reward_ablation}, Table~\ref{tab:reward_ablation_main}): on
\texttt{catapult} the reward-free variant drops Claude Sonnet from
$78.0 \pm 10.7\%$ to $51.0 \pm 10.1\%$, and on Qwen-2.5-7B it reaches
$64.0 \pm 1.7\%$ versus $72.0 \pm 5.2\%$ with rewards on
\texttt{down\_to\_earth} and $20.0 \pm 2.7\%$ versus $42.0 \pm 3.3\%$ on
\texttt{two\_body\_problem}. It also costs efficiency: the
reward-free bank needs $15.8$ iterations per seed on \texttt{catapult} against
$13.3$ with labels, $14.6$ against $12.6$ on \texttt{down\_to\_earth} and $22.2$
against $17.7$ on \texttt{two\_body\_problem},
so the labelled bank solves more seeds with fewer interactions. The reward labels
thus provide environment-grounded feedback from the actor's own exploration that
helps assign credit for effective and efficient skill acquisition, and better
guides the evolver in composing, retaining or pruning skills.




\subsection{Frozen-bank content and ranking ablations}
\label{app:bank-content}

\paragraph{Setup.} Because HExA's skill bank is injected as a textual prefix,
any improvement could in principle be attributed to prompt length, in-context
formatting, or generic priming toward physics reasoning rather than to the
specific knowledge the evolver distilled. We isolate this with frozen banks---no
evolution during evaluation---under four content conditions and four ranking
conditions Figure~\ref{fig:bank_ablation_full} and Table~\ref{tab:interphyre_ablation}.

\begin{figure}[H]
  \centering
  \includegraphics[width=1\linewidth]{figures/bank_ablation.pdf}
  \caption{%
    \textbf{Frozen-bank content and ranking ablations, full results.}
    Held-out solve rate (\%) on 50 unseen seeds of \texttt{two\_body\_problem}
    and \texttt{down\_to\_earth} with Qwen-2.5-7B and a frozen skill bank;
    points are means over 3 independent runs and bars denote $\pm 1$ s.d.
    The dashed line marks \textsc{ReAct} with an empty bank
    ($\mathcal{K} = \varnothing$), the shaded orange region marks performance
    worse than injecting nothing, and the blue band marks $\pm 1$ s.d.\ around
    the full-bank reference. The \emph{injected context} column reports the
    character count of the retrieved prefix, so each condition's accuracy can
    be read against the amount of text it adds.
    \emph{Top:} which components of the bank are injected---full bank,
    strategy skills only, mistake records only, or a length-matched bank
    evolved on a different level.
    \emph{Bottom:} whether the evolver's reward-derived confidence ranking
    carries information---all skills retained, the two lowest-confidence
    skills removed, the two highest removed, or confidences randomly permuted
    while retaining all content.}
  \label{fig:bank_ablation_full}
\end{figure}

\paragraph{Strategy skills and mistake records are not interchangeable.}
Removing either component costs accuracy, but the two behave differently across
levels. Strategy skills alone retain most of the gain on both levels
($46.0\%$ and $71.4\%$). Mistake records alone are nearly sufficient on
\texttt{down\_to\_earth} ($74.8\%$ of a $76.9\%$ ceiling) yet collapse on
\texttt{two\_body\_problem} ($17.3\%$). We read this as a difference in failure
structure: on the easier level most failures are recurring, locally correctable
errors that a record of past mistakes prevents directly, whereas the harder
level requires a positive multi-step strategy---bisection over a contact
parameter, in the worked example of Appendix~\ref{app:worked-example}---that
descriptions of what went wrong do not supply. This supports maintaining both
skill types rather than a single undifferentiated memory.

\paragraph{The evolver's confidences are informative, not decorative.}
On \texttt{down\_to\_earth}, removing the two highest-confidence skills costs
$11.4$ points ($76.7\% \rightarrow 65.3\%$), whereas removing the two lowest
leaves performance unchanged ($76.7\%$) despite halving the injected context
from $0.9$k to $0.5$k characters: the ranking identifies which entries carry the
task, and the low-ranked tail is close to free to discard. Permuting confidences
while retaining all content costs $6.0$ points on \texttt{down\_to\_earth}
($76.7\% \rightarrow 70.7\%$), indicating that retrieval order matters beyond
mere inclusion, though on \texttt{two\_body\_problem} the same manipulation lies
within run-to-run variance ($50.0\% \rightarrow 48.7\%$). We therefore treat
ranking quality as a secondary rather than primary driver of performance.

\paragraph{Relevance, not volume: the wrong-level control.}
We replace the bank with one evolved on a different \textsc{Interphyre} level,
matched in length and indistinguishable in surface form: fluent, well-structured
physics guidance with the same schema of titles, principles and applicability
conditions. On \texttt{two\_body\_problem} this reduces solve rate from $50.0\%$
to $9.3\%$, below the $12.0\%$ empty-bank \textsc{ReAct} baseline, while
injecting $2.9$k characters against the full bank's $4.0$k; the same ordering
holds on \texttt{down\_to\_earth} ($76.9\% \rightarrow 27.9\%$). Injecting
plausible but misapplied procedural knowledge is therefore actively harmful
relative to injecting nothing, which rules out length and priming explanations:
a longer prompt that is wrong about the task is worse than no prompt at all. We
attribute this to misdirected exploration---the actor commits early to a
strategy whose applicability condition does not in fact hold, and spends its
$25$-turn budget refining the wrong hypothesis rather than forming a new one.
This is also why cross-level transfer (Section~\ref{sec:transfer}) requires the
evolver's de-binding and re-grounding step rather than direct reuse of a source
bank.

\paragraph{Summary.} These ablations locate HExA's gain in task-relevant
distilled content and its reward-derived prioritization, not in context length.
Both skill types are load-bearing, their relative importance tracks the failure
structure of the level, and the bank's value concentrates in a small number of
high-confidence strategies.

\input{tables/ablations_merged}

==> appendices/app_results_old.tex <==
\section{Full results}
\label{app:results}

This appendix holds the detailed counterparts of the five compressed tables in
Section~\ref{sec:results}: per-episode metrics, token ranges, iteration counts,
competing published numbers and the full significance blocks.

% =====================================================================
\subsection{\textsc{InterPhyre}}
\label{app:results:interphyre}

The \textsc{Zero-shot} base rate on every level is in the main body
(Table~\ref{tab:direct_baseline_results_main}).
Table~\ref{tab:catapult_cost} gives the cost accounting on the two hard levels
with Claude Sonnet, and Table~\ref{tab:interphyre_qwen_full} the open-weight
head-to-head with per-replicate standard deviations. These are the
sources for the corresponding columns of Table~\ref{tab:interphyre}.

We also ran GPT-OSS-120B on \texttt{catapult}, where \textsc{HExA} lifts it from
$0.0\%$ under \textsc{ReAct} to $54.0\%$. That run predates the fixed split and
is scored on the pooled seed set, with the bank not yet distilled on the seed
being attempted, so it is not paired with the arms in
Table~\ref{tab:interphyre} and we keep it out of that table.

\input{tables/catapult_main}
\input{tables/interphyre_qwen}

\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/catapult_var_cum_avg_iter.pdf}
    \subcaption{Catapult}
    \label{fig:catapult_var_cum_iter}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/ptp_cum_avg_iter.pdf}
    \subcaption{Pass the Parcel}
    \label{fig:ptp_cum_iter}
  \end{minipage}
  \caption{%
    \textbf{Cumulative average turns per seed}, Claude Sonnet; lower is more
    efficient. Off2On Evolving converges to the lowest cost per seed on both
    levels, while the iterative and pure-online variants stay higher, so the gain
    comes from guiding search with accumulated experience rather than from
    spending more computation per instance. The cumulative curves stay separated
    across the whole seed sweep, so the ranking is not an artifact of a few lucky
    seeds. Companion to Figure~\ref{fig:training_curves}.}
  \label{fig:cum_iter_both}
\end{figure}

\begin{figure}[t]
\centering
\setlength{\tabcolsep}{1.2pt}
\renewcommand{\arraystretch}{0.85}
{\footnotesize\itshape \textsc{ReAct} (25 iterations, FAILURE)}\\[1pt]
\begin{tabular}{@{}ccccccc@{}}
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step0.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step30.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step57.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step70.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step91.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step151.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step193.png} \\
\end{tabular}\\[2pt]
{\footnotesize\itshape \textsc{HExA} (6 iterations, SUCCESS)}\\[1pt]
\begin{tabular}{@{}ccccccc@{}}
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step0.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step25.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step57.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step74.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step119.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step140.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step172.png} \\
\end{tabular}
\caption{%
\textbf{How the evolved bank guides the agent on a held-out \texttt{catapult}
seed.} Top: \textsc{ReAct}, with no cross-episode memory, exhausts its
25-iteration budget on ineffective placements. Bottom: \textsc{HExA} opens with
the bank's learned default, reads the resulting failure through the bank's
diagnosis rather than as a reason to keep tuning the same parameter, applies the
corrective rule, and succeeds in six interaction iterations. Frames are sampled
from the final simulations; full prompts, bank entries and trajectories are in
Appendix~\ref{app:trajectories:bank}.}
\utsav{These frames are still rendered from seed 45. They have to be re-made for
seed 64, to match the skill-bank box in the method section and the transcripts in
Appendix~\ref{app:trajectories}. The caption above is already seed-agnostic, so
only the images and the iteration counts need swapping.}
\label{fig:catapult45_simframes}
\end{figure}

\input{tables/baseline_results}

% =====================================================================
\subsection{Interactive games}
\label{app:results:games}

Table~\ref{tab:orbit_memory} is the full head-to-head on Mastermind and Maze:
three task/actor blocks, each arm playing an identical held-out pool, with
first-episode, last-episode and \texttt{any}-episode success, the injected token
budget, and a two-sided paired sign test on episode-3 outcomes against that
block's no-memory arm. Table~\ref{tab:orbit_transfer_full} gives the per-episode
breakdown of the cross-task transfer arms summarised in
Table~\ref{tab:transfer}.

\input{tables/orbit_memory_headtohead}
\subsection{Reasoning and planning}
\label{app:results:reasoning}

Table~\ref{tab:reasoning} gives the per-task head-to-head on the four reasoning
and planning tasks. Every arm is our own run on our provider at the same rollout
budget as \textsc{HExA}, so all rows are paired on identical items; the MemRL
runs at this budget are still in progress.

\input{tables/core_headtohead}

% =====================================================================
\subsection{\textsc{DiscoverPhysics}}
\label{app:results:discovery}

Table~\ref{tab:discovery} gives explanation score, benchmark reward and pass-rate
at both gates for all three worlds, with exact paired tests on the same 15 seeds.

\input{tables/discovery}

% =====================================================================
\subsection{Transfer}
\label{app:results:transfer}

Table~\ref{tab:cross_level_full} reports the source-bank and synthesised-bank
sizes for cross-level transfer within \textsc{InterPhyre}, and
Table~\ref{tab:orbit_transfer_full} the per-episode breakdown for cross-task
transfer on Mastermind.

\input{tables/cross_level_transfer}
\input{tables/orbit_transfer}

% =====================================================================
\subsection{In-context accumulation against gradient-based RL}
\label{app:results:grpo}

To situate \textsc{HExA} in the broader RL landscape, we train the same
Qwen-2.5-3B model on the same two levels with Group Relative Policy Optimization
(GRPO)~\citep{shao2024deepseekmath}, using batch size $1$, $n{=}4$ rollouts per
step, and a binary $\{0, 1\}$ reward from the environment. With 50 training seeds
and batch size $1$, one epoch of GRPO corresponds to 50 gradient updates --- the
same number of unique puzzle instances seen by \textsc{HExA} in a single pass.
Figure~\ref{fig:grpo_comparison} shows validation accuracy across 6 epochs for two
variants: GRPO, and GRPO with a previously evolved skill bank baked into the
prompt at data-generation time.

\input{figures/grpo_comparision_figure}

At the matched sample budget (50 unique seeds, vertical dashed line), GRPO
without skills reaches $20\%$ on \texttt{down\_to\_earth} and $6\%$ on
\texttt{two\_body\_problem}, against \textsc{HExA}'s $23.3\%$ and $12.0\%$. This
gap is consistent with the established finding that in-context methods are more
sample-efficient in new domains: skills distilled from early trajectories are
immediately available to subsequent episodes via context injection, whereas GRPO
must accumulate gradient signal over many rollouts before the policy weights
encode the same knowledge.

Given sufficient training, however, GRPO's exact environment reward eventually
dominates: \texttt{down\_to\_earth} reaches $100\%$ by epoch~5 (GRPO) and epoch~6
(GRPO with skills), while \texttt{two\_body\_problem} peaks at $56\%$ and plateaus
around $40$--$50\%$ for GRPO and converges to $100\%$ by epoch~4 with skills. The
skilled variant additionally exhibits a pronounced epoch-1 dip ($6\%$ on
\texttt{down\_to\_earth}, $0\%$ on \texttt{two\_body\_problem}) before recovering,
consistent with the model needing several epochs to re-adapt its generation format
to the longer skill-augmented prompt (${\sim}2200$ vs.\ ${\sim}1400$ tokens)
before it can leverage the injected skills. In-context skill evolution is
therefore the preferred approach when the sample and interaction budget is small,
while gradient-based RL with an exact reward remains a strong option to bootstrap
further after an in-context warm start.

\input{tables/ICMSRL_results}
\input{tables/ICMSRL_catapult_variants}


==> appendices/app_skillrl_prompts.tex <==
% =============================================================
%  Appendix: Evolver prompts for HeXA and cross-level transfer
%
%  Requires (in main preamble):
%      \usepackage{listings}
%      \usepackage{xcolor}
% =============================================================

\section{Evolver Prompts for \textsc{HeXA} and Cross-Level Transfer}
\label{app:skillrl_prompts}

This appendix reproduces, verbatim, the prompts presented to the Evolver LLM $\mathcal{M}_\theta$ that drive every skill-distillation result in this paper.
Their mapping to the experiments in \S\ref{app:results} and \S\ref{sec:transfer} is summarised in Table~\ref{tab:prompt_mapping}.
Placeholder fields shown in curly braces (\texttt{\{level\_name\}}, \texttt{\{success\_block\}}, \texttt{\{n\_sources\}}, etc.) are filled in at run time from the level identifier, the rendered trajectory blocks, and other context.
Double-braces \texttt{\{\{...\}\}} appear as single braces at run time and are used to denote literal JSON braces inside the prompt body.

\begin{table}[h]
\centering
\small
\caption{%
  Mapping from Evolver prompt to the experiments that invoke it.
  The iterative variants do \emph{not} use the evolution prompt: they
  re-call Pass~1 + Pass~2 each round on a fresh trajectory batch with no
  bank context. The evolving variants call Pass~1 + Pass~2 at round~0
  (offline-init) or round~1 (cold-start) and switch to the evolution
  prompt for all subsequent rounds.
}
\label{tab:prompt_mapping}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llll}
\toprule
\textbf{Prompt} & \textbf{Variants} & \textbf{Rounds invoked} & \textbf{Results} \\
\midrule
\multicolumn{4}{l}{\emph{Generic HeXA Evolver prompts (Tables~\ref{tab:catapult_skillrl}, \ref{tab:interphyre_qwen}, \ref{tab:reward_ablation})}} \\
\addlinespace[2pt]
Pass~1 contrastive            & Offline (Static)        & init only          & PTP, Qwen-3B \\
                              & Off2On Iter., Online Iter. & every round    & PTP, Qwen-3B \\
                              & Off2On Evol., Online Evol. & init / round~1  & PTP, Qwen-3B \\
Pass~2 mistakes               & Offline (Static)        & init only          & PTP, Qwen-3B \\
                              & Off2On Iter., Online Iter. & every round    & PTP, Qwen-3B \\
                              & Off2On Evol., Online Evol. & init / round~1  & PTP, Qwen-3B \\
Skill-bank evolution          & Off2On Evol., Online Evol. & rounds $\geq 2$ & PTP, Qwen-3B \\
\addlinespace[3pt]
\multicolumn{4}{l}{\emph{Catapult-specific Claude variants (Table~\ref{tab:catapult_skillrl})}} \\
\addlinespace[2pt]
Pass~1 / Pass~2 / Evolution (catapult) & Off2On Evol.\ on catapult & all rounds & Table~\ref{tab:catapult_skillrl} \\
\addlinespace[3pt]
\multicolumn{4}{l}{\emph{Cross-level transfer (Table~\ref{tab:cross_level})}} \\
\addlinespace[2pt]
Cross-level synthesis (full) & Claude Evolver          & one-shot           & catapult row \\
Cross-level synthesis (slim) & Qwen-7B Evolver         & one-shot           & FIP, TBP rows \\
\bottomrule
\end{tabular}
\end{table}

\lstdefinestyle{prompt}{
  basicstyle=\ttfamily\footnotesize,
  breaklines=true,
  breakindent=0pt,
  breakautoindent=false,
  columns=fullflexible,
  keepspaces=true,
  showstringspaces=false,
  upquote=true,
  frame=single,
  framesep=4pt,
  rulecolor=\color{black!30},
  backgroundcolor=\color{black!2},
  xleftmargin=4pt,
  xrightmargin=4pt,
  aboveskip=6pt,
  belowskip=6pt,
  inputencoding=utf8,
  extendedchars=true,
  literate=%
    {→}{{$\rightarrow$}}1
    {↔}{{$\leftrightarrow$}}1
    {↑}{{$\uparrow$}}1
    {↓}{{$\downarrow$}}1
    {≈}{{$\approx$}}1
    {≤}{{$\leq$}}1
    {≥}{{$\geq$}}1
    {±}{{$\pm$}}1
    {²}{{${}^2$}}1
    {³}{{${}^3$}}1
    {×}{{$\times$}}1
    {—}{{---}}1
    {–}{{--}}1
    {…}{{\ldots}}1
    {═}{{=}}1
    {─}{{-}}1
    {“}{{``}}1
    {”}{{''}}1
    {‘}{{`}}1
    {’}{{'}}1,
}

% -----------------------------------------------------------
\subsection{Pass~1 --- Contrastive Skill Distillation}
\label{app:prompt:contrastive}

Every \textsc{HeXA} round invokes this prompt to extract \emph{strategy skills} by contrasting high-reward against low-reward trajectories within the same level batch.
The reward function from Eq.~\ref{eq:reward} is communicated to the Evolver as a per-trajectory \texttt{Reward} annotation embedded in the rendered success and failure blocks.

\begin{lstlisting}[style=prompt]
You are an expert physics analyst distilling agent behavior into concise, actionable skills.

**Environment**: 2D physics simulation (Box2D). Gravity = -9.8 m/s². World bounds [-5, 5] on both axes. The agent places a red ball at (x, y) with a given radius, then the simulation runs to completion.

**Level: {level_name}**
{level_description}

Below are SUCCESSFUL and FAILED trajectories from the same level. Each shows the agent's reasoning (Thought), actions taken, and simulation observations. Each trajectory has a **Reward** score:
- Successes: +1.0 (solved fast, 1-3 iters) to +0.25 (solved slowly, 16-25 iters)
- Failures: -0.5 (tried all iterations) to -0.75 (gave up early)

**Weight your analysis by reward** -- skills from high-reward trajectories (fast solves) are more reliable than skills from low-reward ones (barely solved).

=== SUCCESSFUL TRAJECTORIES ({n_successes}) ===
{success_block}

=== FAILED TRAJECTORIES ({n_failures}) ===
{failure_block}

---

Your task: By CONTRASTING the successes and failures, extract the KEY PHYSICS SKILLS that distinguish solving from failing. Focus especially on high-reward successes -- what insight let the agent solve it quickly? What did the failed agents miss?

For each skill, provide:
- **title**: Short name (3-7 words)
- **principle**: The physics insight (2-3 sentences). What mechanism was exploited? Why does it work?
- **when_to_apply**: Specific trigger condition (1 sentence)
- **source_seeds**: List of seed numbers from the trajectories above that this skill was primarily derived from. Include only the seeds whose behavior directly demonstrates or motivates this skill.

Output a JSON array:
```json
[
  {{
    "title": "...",
    "principle": "...",
    "when_to_apply": "...",
    "source_seeds": [1, 5, 16]
  }}
]
```

Extract 4-6 skills. Each should capture a DISTINCT insight from the success/failure contrast. Avoid redundancy.
\end{lstlisting}

% -----------------------------------------------------------
\subsection{Pass~2 --- Mistake \& Partial-Skill Extraction}
\label{app:prompt:mistakes}

Run on the failure subset $\mathcal{T}_\ell^{(n),-}$ alone.
Produces (i)~structured \emph{mistake} records $\mu = (\delta_\mu, \rho_\mu, \alpha_\mu)$ describing recurring failure modes, and (ii)~\emph{partial skills} extracted from individual correct steps inside otherwise-failed trajectories.

\begin{lstlisting}[style=prompt]
You are an expert at analyzing agent failures and distilling them into avoidable mistake patterns.

**Environment**: 2D physics simulation (Box2D). Gravity = -9.8 m/s². World bounds [-5, 5].

**Level: {level_name}**
{level_description}

Below are FAILED trajectories. Each shows the agent's reasoning, actions, and simulation results.

{failure_block}

---

Your task has TWO parts:

**Part 1 -- Mistakes**: Identify the COMMON MISTAKE PATTERNS across these failures. For each mistake, analyze:
1. What exactly the agent did wrong
2. WHY the agent made this error (what broken causal belief led to it)
3. A concrete actionable fix

**Part 2 -- Partial insights**: Even in failed trajectories, some individual steps show CORRECT physics reasoning or useful discoveries (e.g., the agent found a valid placement region but then abandoned it, or correctly identified a mechanism but applied it with wrong parameters). Extract 1-2 skills from these "good steps within bad trajectories". These should be genuine physics insights, not just restating what went wrong.

Format as JSON object with two arrays:
```json
{{
  "mistakes": [
    {{
      "description": "What the mistake is (1 sentence)",
      "why_it_happens": "The broken belief or reasoning error that causes this (1 sentence)",
      "how_to_avoid": "Concrete actionable fix -- what to do instead (1-2 sentences)"
    }}
  ],
  "partial_skills": [
    {{
      "title": "Short name (3-7 words)",
      "principle": "The physics insight from the failed trajectory (2-3 sentences)",
      "when_to_apply": "Specific trigger condition (1 sentence)",
      "source_seeds": [5, 11]
    }}
  ]
}}
```

Extract 3-5 mistakes and 1-2 partial skills. For mistakes, group similar failures into one and focus on ROOT CAUSES. For partial skills, only extract genuinely useful insights -- do not force it if no good steps exist.
\end{lstlisting}

% -----------------------------------------------------------
\subsection{Skill-Bank Evolution}
\label{app:prompt:evolution}

Used by the evolving variants (Off2On Evol., Online Evol.) at every round $n \geq 1$.
Receives both the current bank $\mathcal{K}_\ell^{(n)}$ and the new trajectory batch $\mathcal{T}_\ell^{(n)}$, and emits the evolved bank $\mathcal{K}_\ell^{(n+1)}$ (Eq.~\ref{eq:evolve}) subject to the per-level skill budget $B$ and the mistake cap.
The Evolver decides which existing skills to retain (with their confidence preserved), which to remove, and which to add (with confidence assigned via Eq.~\ref{eq:confidence}).

\begin{lstlisting}[style=prompt]
You are a physics Evolver evolving a skill bank for puzzle-solving agents.

LEVEL: {level_name}
LEVEL DESCRIPTION: {level_description}

CURRENT SKILL BANK (from previous rounds):
{existing_skills_block}

NEW TRAJECTORIES (from the latest round):
Successes: {n_successes}
Failures: {n_failures}

{new_trajectories_block}

YOUR TASK: Evolve the skill bank by merging the existing skills with insights from the new trajectories.

RULES:
1. Output the COMPLETE FINAL skill bank (not a diff) -- include both retained existing skills and any new ones.
2. Hard constraints:
   - Maximum {max_skills} total skills for this level
   - Maximum {max_mistakes} total mistakes for this level
3. For each skill you include:
   - If it's a RETAINED skill from the existing bank: set "is_new": false
   - If it's a NEW skill extracted from the new trajectories: set "is_new": true
   - Include "source_seeds" listing seed numbers where this skill was observed (required for confidence calibration)
   - Include "confidence": a float in [0.1, 1.0] representing your confidence in this skill
4. For retained skills, preserve their existing confidence values (they've been validated).
5. For new skills, estimate confidence based on:
   - Success rate among source trajectories (high success = high confidence)
   - Universality (applies to multiple seed conditions = higher confidence)
   - Clarity and actionability of the principle
6. Do not include duplicate skills. If a new trajectory confirms an existing skill, keep the existing one (possibly with slightly higher confidence).
7. Remove skills that are:
   - Redundant or subsumed by other skills.
   - Contradicted by the new trajectories
   - Too specific or rarely applicable
   - Low confidence (< 0.3) and not directly observed in new trajectories
8. Do not remove mistakes unless the new trajectories show they're no longer common.

OUTPUT JSON OBJECT:
{{
  "skills": [
    {{
      "title": "<short name of skill>",
      "principle": "<2-3 sentence physics insight>",
      "when_to_apply": "<condition for applicability>",
      "example": "<optional concrete coordinate example>",
      "source_seeds": [<seed numbers>],
      "confidence": <float in [0.1, 1.0]>,
      "is_new": <true|false>
    }}
    ...
  ],
  "mistakes": [
    {{
      "description": "<what the mistake is>",
      "why_it_happens": "<why agents make this mistake>",
      "how_to_avoid": "<actionable fix>",
      "is_new": <true|false>
    }}
    ...
  ],
  "removed_skill_titles": ["<title of removed skill 1>", ...],
  "reasoning": "<brief explanation of key changes: what was removed, what was added, why>"
}}

Be concise but precise. Focus on physics insights that directly help puzzle-solving.
\end{lstlisting}

% -----------------------------------------------------------
\subsection{Catapult-Specific Variants (Claude)}
\label{app:prompt:catapult}

The within-level catapult result in Table~\ref{tab:catapult_skillrl} was produced with catapult-specific variants of all three Evolver prompts above.
The variants differ from the generic prompts in two ways:
(i)~a \emph{factual} catapult scene block (objects, success condition, placement constraints) is injected after the \textbf{Level:} header so the Evolver knows the scene without seeing strategy hints, and
(ii)~minor task-framing wording is tightened (e.g.\ ``Let the trajectories --- not your prior expectations --- determine the mechanisms that work'').

\paragraph{Shared catapult scene description.}

\begin{lstlisting}[style=prompt]
**Scene (factual -- no approach implied):**
- Green Ball: small dynamic ball on the LEFT end of a gray bar.
- Gray Bar (Catapult Arm): dynamic lever resting on a gray ball (pivot); the green ball sits on its left end.
- Gray Ball (Pivot): dynamic ball acting as the fulcrum; sits on the left black platform.
- Black Ball (Ceiling Blocker): static ball near the top of the scene.
- Black Platform (Left): static horizontal platform on the left side.
- Black Ledge (Right): static (possibly angled) platform on the right side.
- Basket (Gray): dynamic basket sitting on the right ledge.
- Blue Ball (Target): dynamic ball inside the basket.

**Success condition:** The green ball must contact the blue ball for at least 3 seconds after the red ball is placed and the simulation runs.

**Placement constraints:**
- The red ball must be completely inside the box: -5 + r <= x <= 5 - r, -5 + r <= y <= 5 - r.
- The red ball must NOT overlap with any existing object at t=0.
- 0.1 <= radius <= 2.0.
\end{lstlisting}

\paragraph{Pass~1 --- contrastive (catapult).}

\begin{lstlisting}[style=prompt]
You are an expert physics analyst distilling agent behavior into concise, actionable skills.

**Environment**: 2D physics simulation (Box2D). Gravity = -9.8 m/s^2. World bounds [-5, 5] on both axes. The agent places a red ball at (x, y) with a given radius, then the simulation runs to completion.

**Level: {level_name}**
[catapult scene description injected here -- see above]

Below are SUCCESSFUL and FAILED trajectories from this level. Each shows the agent's reasoning (Thought), actions taken, and simulation observations. Each trajectory has a **Reward** score:
- Successes: +1.0 (solved fast, 1-3 iters), +0.75 (4-7 iters), +0.5 (8-15 iters), +0.25 (solved slowly, 16-25 iters)
- Failures: -0.5 (tried all 25 iters), -0.75 (gave up early, <10 iters)

**Weight your analysis by reward** -- skills extracted from high-reward trajectories (fast solves) are more reliable than those from low-reward ones.

=== SUCCESSFUL TRAJECTORIES ({n_successes}) ===
{success_block}

=== FAILED TRAJECTORIES ({n_failures}) ===
{failure_block}

---

Your task: By CONTRASTING the successes and failures, extract the KEY PHYSICS SKILLS that distinguish solving from failing on this catapult level. Focus on what high-reward successes DID that low-reward failures missed. Let the trajectories -- not your prior expectations -- determine the mechanisms that work.

For each skill, provide:
- **title**: Short name (3-7 words)
- **principle**: The physics insight (2-3 sentences). What mechanism was exploited? Why does it work?
- **when_to_apply**: Specific trigger condition (1 sentence)
- **source_seeds**: Seed numbers from the trajectories above that this skill was primarily derived from.

Output a JSON array:
```json
[
  {{
    "title": "...",
    "principle": "...",
    "when_to_apply": "...",
    "source_seeds": [1, 5, 16]
  }}
]
```

Extract 4-6 skills. Each should capture a DISTINCT insight from the success/failure contrast. Avoid redundancy.
\end{lstlisting}

\paragraph{Pass~2 --- mistakes \& partial skills (catapult).}

\begin{lstlisting}[style=prompt]
You are an expert at analyzing agent failures and distilling them into avoidable mistake patterns.

**Environment**: 2D physics simulation (Box2D). Gravity = -9.8 m/s^2. World bounds [-5, 5].

**Level: {level_name}**
[catapult scene description injected here -- see above]

Below are FAILED trajectories. Each shows the agent's reasoning, actions, and simulation results.

{failure_block}

---

Your task has TWO parts:

**Part 1 -- Mistakes**: Identify the COMMON MISTAKE PATTERNS across these failures. For each mistake, analyze:
1. What exactly the agent did wrong
2. WHY the agent made this error (what broken causal belief led to it)
3. A concrete actionable fix

**Part 2 -- Partial insights**: Even in failed trajectories, some individual steps show CORRECT physics reasoning or useful discoveries (e.g., the agent found a promising placement region but then abandoned it, or correctly identified a mechanism but applied it with wrong parameters). Extract 1-2 skills from these "good steps within bad trajectories". These should be genuine physics insights, not just restating what went wrong.

Format as a JSON object with two arrays:
```json
{{
  "mistakes": [
    {{
      "description": "What the mistake is (1 sentence)",
      "why_it_happens": "The broken belief or reasoning error that causes this (1 sentence)",
      "how_to_avoid": "Concrete actionable fix -- what to do instead (1-2 sentences)"
    }}
  ],
  "partial_skills": [
    {{
      "title": "Short name (3-7 words)",
      "principle": "The physics insight from the failed trajectory (2-3 sentences)",
      "when_to_apply": "Specific trigger condition (1 sentence)",
      "source_seeds": [5, 11]
    }}
  ]
}}
```

Extract 3-5 mistakes and 1-2 partial skills. For mistakes, group similar failures into one and focus on ROOT CAUSES. For partial skills, only extract genuinely useful insights -- do not force it if no good steps exist.
\end{lstlisting}

\paragraph{Skill-bank evolution (catapult).}

\begin{lstlisting}[style=prompt]
You are a physics Evolver evolving a skill bank for a catapult-puzzle-solving agent.

**Environment**: 2D physics simulation (Box2D). Gravity = -9.8 m/s^2. World bounds [-5, 5].

**Level: {level_name}**
[catapult scene description injected here -- see above]

CURRENT SKILL BANK (from previous rounds):
{existing_skills_block}

NEW TRAJECTORIES (from the latest round):
Successes: {n_successes}
Failures: {n_failures}

{new_trajectories_block}

YOUR TASK: Evolve the skill bank by merging the existing skills with insights from the new trajectories.

RULES:
1. Output the COMPLETE FINAL skill bank (not a diff) -- include both retained existing skills and any new ones.
2. Hard constraints:
   - Maximum {max_skills} total skills for this level.
   - Maximum {max_mistakes} total mistakes for this level.
3. For each skill you include:
   - If it's a RETAINED skill from the existing bank: set "is_new": false.
   - If it's a NEW skill extracted from the new trajectories: set "is_new": true.
   - Include "source_seeds" listing seed numbers where this skill was observed (required for confidence calibration).
   - Include "confidence": a float in [0.1, 1.0] representing your confidence in this skill.
4. For retained skills, preserve their existing confidence values (they've been validated).
5. For new skills, estimate confidence based on:
   - Success rate among source trajectories (high success = high confidence).
   - Universality (applies across multiple seed conditions = higher confidence).
   - Clarity and actionability of the principle.
6. Do not include duplicate skills. If a new trajectory confirms an existing skill, keep the existing one (optionally raising its confidence slightly).
7. Remove skills that are:
   - Redundant or subsumed by another skill.
   - Contradicted by the new trajectories.
   - Too specific or rarely applicable.
   - Low confidence (< 0.3) AND not observed in the new trajectories.
8. Do not remove mistakes unless the new trajectories show they're no longer common.

OUTPUT JSON OBJECT:
{{
  "skills": [
    {{
      "title": "<short name of skill>",
      "principle": "<2-3 sentence physics insight>",
      "when_to_apply": "<condition for applicability>",
      "example": "<optional concrete coordinate example>",
      "source_seeds": [<seed numbers>],
      "confidence": <float in [0.1, 1.0]>,
      "is_new": <true|false>
    }}
  ],
  "mistakes": [
    {{
      "description": "<what the mistake is>",
      "why_it_happens": "<why agents make this mistake>",
      "how_to_avoid": "<actionable fix>",
      "is_new": <true|false>
    }}
  ],
  "removed_skill_titles": ["<title of removed skill 1>", ...],
  "reasoning": "<brief explanation of key changes: what was removed, what was added, why>"
}}

Be concise but precise. Focus on physics insights grounded in the trajectories.
\end{lstlisting}

% -----------------------------------------------------------
\subsection{Cross-Level Synthesis --- Full (Claude)}
\label{app:prompt:cross_level_full}

Used for the catapult cross-level result in Table~\ref{tab:cross_level} where the Evolver is Claude Sonnet~4.6 and three source banks are consumed (\texttt{down\_to\_earth}, \texttt{two\_body\_problem}, \texttt{pass\_the\_parcel}).
The eight hard constraints --- citation requirement, no invented coordinates, target-side entities only, no platitudes, mandatory transfer rationale, confidence calibration, no redundancy, mistake constraints --- are enumerated explicitly so that every synthesised skill remains traceable to the source skill IDs that motivated it.

\begin{lstlisting}[style=prompt]
You are an expert physics analyst performing CROSS-LEVEL OFFLINE SKILL TRANSFER.

You will be given expert skill banks from {n_sources} SOURCE physics levels.
Each source bank was distilled and evolved over many rounds of an agent solving
that level. You will also be given a factual description of a TARGET level
that the agent has NEVER attempted yet -- no target-level trajectories,
no target-level skills, no target-level success/failure data exist.

Your task: synthesise a TARGET skill bank by extracting transferable physics
PRINCIPLES from the source banks, re-grounding them in the target scene, and
predicting which principles the target level will reward.

==========================================================================
**Environment (shared across all levels)**: 2D physics simulation (Box2D).
Gravity = -9.8 m/s^2. World bounds [-5, 5] on both axes. The agent places ONE
red ball at (x, y) with a chosen radius (0.1 <= r <= 2.0) at t=0; the simulation
then runs to completion. Mass scales as r^3; momentum and impact force scale
with both mass and the ball's velocity at first contact.
==========================================================================

=== SOURCE LEVELS ===

{source_blocks}

=== TARGET LEVEL: {target_level} ===

{target_block}

=== TASK ===

Produce a SKILL BANK for the target level. The bank must contain:
- 6 to 10 SKILLS (physics principles you predict will help on the target).
- 2 to 4 MISTAKES (anti-patterns transferable from source failures).

=== HARD CONSTRAINTS ===

1. **Every skill MUST cite source skills.** For each output skill, include
   `source_skills`: a non-empty list of objects of the form
   `{{"source_level": "<level>", "skill_id": "<id>"}}`, listing the source-bank
   entries that motivated this skill. If you cannot cite at least one source
   skill, do NOT emit the skill -- synthesise something else instead.

2. **No invented coordinates.** You have NEVER seen the target level solved.
   Do NOT predict specific (x, y, r) values that "work" for the target. The
   `example` field, if used, must describe a *qualitative* placement
   (e.g. "place near the end of the lever opposite the green ball, with
   r large enough to dominate the lever's mass") -- never specific numbers.

3. **Use target-level entities.** Phrase each skill in terms of the entities
   that exist in the TARGET scene description above. Do NOT mention source-
   level-only entities (e.g. "ramp", "inverted basket") in the principle or
   when_to_apply, even if those entities motivated the transfer. The
   `transfer_rationale` field is where you may name source entities to
   explain the analogy.

4. **No platitudes.** Skills like "use physics intuition", "consider gravity",
   "be careful" are forbidden. Each skill must name a SPECIFIC mechanism
   (e.g. "torque about a pivot scales with moment arm x force"; "the line of
   centres at first contact determines the post-collision velocity direction").

5. **Each skill must include a `transfer_rationale`** (1-2 sentences) explaining
   what physics primitive bridges the source observation to the target
   prediction. This is the audit trail for your synthesis.

6. **Confidence calibration.** Weight a skill's confidence by:
   - How many source banks corroborate the underlying primitive (more = higher).
   - How directly the primitive applies to the target scene (direct = higher).
   - How load-bearing the source skill was (high source confidence = higher).
   Confidence is a float in [0.1, 1.0]. Assign 0.7+ only when the primitive
   appears in >=2 source banks AND the target scene clearly invokes it.

7. **Avoid redundancy.** Each skill must capture a DISTINCT mechanism. Do not
   emit two skills that are paraphrases of the same idea.

8. **Mistakes**: derive each from source-bank mistakes or from the failure
   modes those mistakes imply. Apply the same hard constraints (cite sources,
   no invented coordinates, target-side entities, specific mechanism).

=== OUTPUT FORMAT (single JSON object) ===

```json
{{
  "skills": [
    {{
      "title": "<3-7 word name>",
      "principle": "<2-3 sentence physics insight, in target-level terms>",
      "when_to_apply": "<specific condition, in target-level terms>",
      "example": "<qualitative placement description, NO numbers -- or omit>",
      "confidence": <float in [0.1, 1.0]>,
      "source_skills": [
        {{"source_level": "<level>", "skill_id": "<id>"}}
      ],
      "transfer_rationale": "<1-2 sentences naming the bridging physics primitive>"
    }}
  ],
  "mistakes": [
    {{
      "description": "<1 sentence in target-level terms>",
      "why_it_happens": "<1 sentence root cause>",
      "how_to_avoid": "<1-2 sentence concrete fix>",
      "source_skills": [
        {{"source_level": "<level>", "skill_id": "<id>"}}
      ],
      "transfer_rationale": "<1-2 sentences>"
    }}
  ],
  "synthesis_reasoning": "<2-4 sentences: which source levels contributed most heavily, which primitives you treated as load-bearing, which source skills you deliberately did NOT transfer and why>"
}}
```

Be precise and specific. Do not pad. Do not produce extra fields. Output ONLY
the JSON object inside a single fenced ```json block.
\end{lstlisting}

% -----------------------------------------------------------
\subsection{Cross-Level Synthesis --- Slim (Qwen-7B)}
\label{app:prompt:cross_level_qwen}

Used for the Falling Into Place and Two Body Problem cross-level rows of Table~\ref{tab:cross_level}, where the Evolver is Qwen-2.5-7B.
The slim variant drops audit fields (\texttt{source\_skills}, \texttt{transfer\_rationale}), reduces to three rules, and tightens form constraints on \texttt{principle} / \texttt{when\_to\_apply} / \texttt{example} to prevent the platitude-and-hallucination failure mode the long prompt produces on smaller models (e.g.\ inventing a lever on a level with no pivot).
Output budget is reduced to 4--6 skills and 1--3 mistakes.

\begin{lstlisting}[style=prompt]
You are extracting transferable physics PRINCIPLES from one or more source level skill banks for a NEW target level.

ENVIRONMENT: 2D physics (Box2D), gravity = -9.8 m/s^2, bounds [-5, 5]. Agent places ONE red ball (x, y, radius 0.1-2.0) at t=0; simulation runs to completion.

=== SOURCE LEVELS ===

{source_blocks}

=== TARGET LEVEL: {target_level} ===

{target_block}

=== TASK ===

Output a skill bank for the target level. Produce 4-6 skills and 1-3 mistakes.

RULES (FOLLOW STRICTLY):

1. SKILLS ARE PRINCIPLES, NOT COMMANDS. Each skill states a physics observation, mechanism, or relationship the agent can REASON FROM. Skills MUST NOT tell the agent what to do. Each field has a strict FORM:
   - `principle`: starts with a condition or relationship ("When X holds, Y occurs", "X scales with Y", "A and B differ in Z"). NEVER an imperative verb. FORBIDDEN openings: place / position / put / drop / move / set / use / adjust.
   - `when_to_apply`: describes a REASONING context the agent enters ("When evaluating whether...", "When comparing alternatives that..."). NEVER a target outcome to achieve ("when you need to tip...", "when knocking the bar off...").
   - `example`: contrasts two physical scenarios or illustrates the principle abstractly. NEVER a placement, never a specific scene action.

2. Each skill names a SPECIFIC mechanism. FORBIDDEN platitudes: "use physics", "place strategically", "consider gravity", "adjust as needed", "be careful".

3. Use ONLY entities present in the TARGET scene above. Do not mention source-only entities anywhere. If the target scene has no pivot, do NOT write skills about levers or torque-around-a-pivot.

4. NO coordinates and NO placements anywhere in any field.

5. Mistakes describe MISCONCEPTIONS the agent might form (wrong mental models), NOT actions to avoid. `how_to_avoid` is a CORRECTED UNDERSTANDING, not a placement instruction.

OUTPUT FORMAT (single JSON object, fenced ```json block, no extra fields):
```json
{{
  "skills": [
    {{"title": "...", "principle": "...", "when_to_apply": "...", "example": "...", "confidence": 0.X}}
  ],
  "mistakes": [
    {{"description": "<misconception, NOT an action>", "why_it_happens": "...", "how_to_avoid": "<corrected understanding, NOT a placement command>"}}
  ],
  "synthesis_reasoning": "<1-2 sentences: which source primitive transferred>"
}}
```

Be concise. Output ONLY the JSON object.
\end{lstlisting}


==> appendices/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The main claims in the abstract and introduction are that
(1) current LLM agents struggle on tasks requiring active experimentation beyond
parametric knowledge, (2) HeXA, a training-free in-context RL framework, jointly
designs experiments, distills hierarchical skills, and transfers them across tasks
without parameter updates or oracle guidance, and (3) HeXA improves both frontier
and small open-weight LLMs, with skill banks transferring zero-shot to unseen
levels. These claims are supported by the formal framework in Section 3, the
InterPhyre benchmark in Section 4.1, and the empirical results in Section 4.3
(within-level gains up to +56 pp on \texttt{catapult}; cross-level transfer gains
up to +36 pp), with full details in Appendices A and D.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss limitations in Section 5. Specifically, (i) HeXA
is evaluated on a 2D physics benchmark (InterPhyre); generalization to higher-
dimensional or partially-observable domains remains future work; (ii) the skill
bank size is hard-capped, and retrieval is currently confidence-weighted rather
than learned, which may limit scaling to very large skill libraries; (iii) the
evolver relies on a frontier LLM as a teacher for distillation, so distillation
quality is bounded by the teacher's reasoning ability; (iv) reward design assumes
a binary success predicate plus an efficiency term, and richer reward signals may
be needed for tasks without a clear success criterion; (v) all experiments use a
fixed 25-iteration budget, and the interaction between budget and skill quality
is not exhaustively studied.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not contain formal theorems or proofs. We
provide a problem formulation (Eq.~1--3) and an algorithmic description of HeXA
(Algorithm~1), and support the framework empirically rather than through formal
analysis.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
 % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides the full HeXA algorithm (Algorithm~1,
Section 3), the reward design and skill-bank structure (Appendix A.3), the
cross-task transfer procedure (Appendix A.4), the InterPhyre tool-call API and
per-level system prompts (Appendices B--C), and the experimental setup including
models, baselines, seed counts, and turn budgets (Section 4.2 and Appendix D).
Tables 1, 2, 8, and 10 report paired comparisons on identical seed sets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We release the InterPhyre benchmark (simulator, intervention
API, gymnasium-compatible interface, and per-level configurations) along with the
HeXA implementation (actor, evolver, retriever, and skill-bank serialization) in
the supplemental material, with instructions to reproduce all reported results.
Anonymized code and configuration files are included with the submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4.2 specifies the models evaluated (Claude Sonnet
4.6, Qwen-2.5-3B/7B Instruct, GPT-OSS-120B), the baselines (ReAct, Reflexion,
Direct, GRPO), the per-level seed counts (50 seeds), and the per-episode turn
budget (25 iterations). Section 3 and Appendix G specify HeXA's hyperparameters
including batch size $x$, retrieval sizes $M, N$, skill-bank caps $M_{\max},
N_{\max}$, initialisation regimes, and update strategies, and GRPO training details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our primary metric is the discrete success rate (count of
successful seeds out of 50). Thus, we report success rates without error bars.
Importantly, all methods on a given level are evaluated on the \emph{same} 50
seeds, so comparisons are paired on identical instances rather than averaged
across independent draws. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Wall-clock time per configuration on \texttt{pass\_the\_parcel}
is reported in Table~1 (Time (h) column). Compute resources, including the
Anthropic API used for Claude Sonnet 4.6, the GPU type and count used for
Qwen-2.5-3B/7B and GPT-OSS-120B inference, and the hardware used for GRPO
fine-tuning, are detailed in Appendix~C.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We introduce HeXA, an in-context learning framework
evaluated on InterPhyre, a 2D procedural physics simulation benchmark. The work
involves no human subjects, no scraped or sensitive data, and no deployment in
high-stakes domains. All models used (Claude Sonnet 4.6, Qwen-2.5, GPT-OSS-120B)
are accessed via public APIs or open-weights releases under their respective
licenses. The research conforms with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: HeXA is a methodological contribution that could improve
sample efficiency for LLM agents in domains requiring active experimentation in unknown environments.
Positive impacts include reducing the compute and data cost of adapting agents
to novel domains. Potential negative impacts mirror those of LLM-based
autonomous agents more broadly: improved exploration capability could be misused
to automate the discovery of unsafe behaviours in adversarial settings. Because
HeXA requires explicit tool-call surfaces and reward signals, deployment risk is
mediated by the environment in which it is run. We discuss this in Appendix~A.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
 % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We release the InterPhyre benchmark (a 2D physics simulator)
and an in-context learning framework that uses publicly accessible LLMs. Neither
artifact poses a high risk for misuse: the simulator contains no scraped or
sensitive data, and HeXA does not modify model weights or release new pretrained
models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite all models and benchmarks used: Claude Sonnet 4.6, Qwen-2.5-3B/7B Instruct, GPT-OSS-120B
(open-weights), and the prior physics-reasoning benchmarks that motivate InterPhyre's design. All assets are used in accordance with their licenses and
terms of service.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We introduce InterPhyre, a new benchmark for in-context
learning via active experimentation. The release includes the simulator,
intervention API, snapshot/restore primitives, gymnasium-compatible interface,
per-level system prompts, and 50 seeds per level. Documentation covering tool
specifications, observation modes, and the success predicate accompanies the
code in the supplemental material; an anonymized version is included with the
submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with
human subjects. All experiments are conducted in a procedurally generated
physics simulator using LLM agents.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with
human subjects, so no IRB approval was required.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLMs are a core, non-standard component of HeXA: the actor
$\pi_{\text{act}}$ and evolver $\pi_{\text{ev}}$ are both LLMs that interact
through a structured tool-call interface, and the evolver is responsible for
distilling natural-language skills and mistake records from interaction
trajectories. The specific models used are (Claude Sonnet 4.6, Qwen-2.5-3B/7B/14b/21B,
GPT-OSS-120B).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> figures/agent_tool_figures.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{NeurIPS_26/figures/Agent_Interphyre_tools.png}
  \caption{%
    \textbf{Tool interface between the \textsc{HeXA} agent and the Interphyre environment.}
    The agent issues two classes of tool calls:
    \textcolor{teal}{\textbf{State Information Tools}} (left) query the scene
    without advancing the simulation---returning object positions, gap widths,
    relative ball positions, and level-specific geometry---and
    \textcolor{orange}{\textbf{Simulation Tools}} (right) place the red ball
    at $(x,y,r)$ and run the physics engine, returning
    \texttt{SUCCESS}/\texttt{FAILURE} with final object positions
    (\texttt{simulate\_action}) or intermediate state at a chosen timestep
    (\texttt{simulate\_partial}).
    The \texttt{finish} action terminates the episode.
    Level-specific state tools (\texttt{compute\_gap\_analysis},
    \texttt{compute\_relative\_positions}, \texttt{get\_ramp\_center}, etc.\@)
    are available only on their respective levels; shared tools are available
    on all levels.
    Selected tools presented here. Full tool signatures and usage instructions are provided in
    Appendix~\ref{app:tools}.
  }
  \label{fig:agent_tools}
\end{figure}


==> figures/build_then_freeze.tex <==
% Headline figure: build-then-freeze, both actors, four panels, one caption.
% Generated as a single canvas by Plots/create_paper_headline_figure.py, which
% draws the panels from the same functions as the standalone figures
%   Plots/create_paper_catapult_claude_figure.py  (rows 1, panels a/b)
%   Plots/create_paper_astra_figure.py            (rows 2, panels c/d)
% so the panels here cannot drift from those.  fig:astra_catapult is kept as
% an alias: it used to be a float of its own.
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/headline_catapult.pdf}
  \caption{%
    \textbf{The bank is built once on the training seeds, frozen, and it is the
    frozen bank that wins --- for a mid-sized and a frontier actor alike.}
    \texttt{catapult}, Claude Sonnet (top, \emph{a}--\emph{b}) and GPT-6-Astra
    (bottom, \emph{c}--\emph{d}). Every bank is warm-started on seeds $1$--$5$,
    built over the $50$ training seeds $6$--$56$ in $17$ rounds of three, then
    frozen and scored on the $50$ held-out seeds $57$--$106$; the two pools are
    disjoint and no distillation happens at evaluation.
    \emph{Left (a, c):} solve rate as the bank accumulates over the training
    seeds, one point per round; every seed inside a round is attempted with the
    same memory, so the round, not the seed, is the unit at which memory
    changes, and round $0$ is the origin rather than a measurement.
    \emph{Right (b, d):} that memory frozen on the held-out seeds, with mean
    turns to solve and the per-episode injected memory block under each bar. A hatched stub on the axis marks an arm that was run and scored $0\%$;
    the memory-free arms inject nothing. Two things travel from left to right.
    The ordering the training curve establishes survives freezing: the distilled
    bank ends well above episodic retrieval, which ends above \textsc{MemRL},
    and both memory baselines end above the memory-free arms. And the bank pays
    for itself twice, in solve rate and in cost --- \textsc{HExA} solves $92\%$
    against \textsc{ReAct}'s $14\%$ while spending half the turns and a third of
    \textsc{Episodic RAG}'s injected tokens. The stronger actor needs fewer
    rounds to get there, reaching $98\%$ within five, but ends at the same
    place: every held-out seed solved, at well under half of \textsc{ReAct}'s
    turn count. Cells and token counts are those of
    Table~\ref{tab:interphyre}.}
  \label{fig:build_then_freeze}
  \label{fig:astra_catapult}
\end{figure}


==> figures/catapult_cum_curves.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/catapult_cum_accuracy.pdf}
    \subcaption{Cumulative accuracy.}
    \label{fig:cat_cum_accuracy}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/catapult_cum_avg_iter.pdf}
    \subcaption{Cumulative average \textsc{ReAct} iterations.}
    \label{fig:cat_cum_iter}
  \end{minipage}
  \caption{%
  Cumulative catapult performance per seed for \textsc{HeXA} (Off2On Evolving, $k{=}3$) against two \textsc{ReAct}-based baselines, one \textsc{ReAct} agent and one Reflexion agent ($K{=}2$ trials and verbal self reflection between each trial), over all prefix lengths, on Claude Sonnet, using 50 seeds.
\textbf{(a)}~\textsc{HeXA} quickly climbs to an approximate peak of $70$--$75\%$, after which the rate plateaus to a steady level of $64\%$. It stays at least three times higher than Reflexion and seven times higher than the \textsc{ReAct} baseline throughout all prefixes. Reflexion converges to an average rate of $22\%$ (which is $14$ percentage points greater than the baseline), however, it still falls far short of \textsc{HeXA}.\textbf{(b)}~Average \textsc{ReAct} iterations drop from the $25$-step ceiling to $\sim$$13.7$ for \textsc{HeXA}; the \textsc{ReAct} baseline never falls below $\sim$$22$, and Reflexion sits just below it at $\sim$$21$  so the in-context skill bank both lifts solve rate and sharply reduces the iterations spent per seed. Final values match Table~\ref{tab:catapult_skillrl}.
  }
  \label{fig:catapult_skillrl}
\end{figure}


==> figures/cross_level_transfer.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/cross_level_transfer_main.pdf}
  \caption{%
  \scott{What is the point of the arrows }
    Cross-level skill transfer (no target trajectories used).
    For each target level the agent solves the puzzle with only the
    \emph{evolver's} skill bank injected via \emph{retriever}; numbers \scott{?} inside
    each bar are the raw success / total seed counts.
    Catapult uses three source banks (Down to Earth, Two Body Problem,
    Pass the Parcel) with Claude Sonnet as both teacher and solver;
    Falling Into Place and Two Body Problem use a single source bank
    (Down to Earth) with Qwen-2.5-7B as both teacher and solver.
    All three targets show positive transfer, with the catapult chain
    of three structurally related sources yielding the largest gain
    ($+36.0$~pp). \abhra{  Cross-level skill transfer results.
  For each \emph{target} level we report (i) the source skill banks
  consumed by $\mathcal{M}_\theta$, with their per-bank skill counts;
  (ii) the size of the synthesised target bank ($n_k$~skills /
  $n_\mu$~mistakes); (iii) the agent that solves the target with
  \emph{only} the synthesised bank injected; (iv) the resulting target
  success rate; and (v) the matched \textsc{ReAct} baseline.
  No target-level trajectories are seen at any stage of synthesis.}
  }
  \label{fig:cross_level_transfer}
\end{figure}


==> figures/grpo_comparision_figure.tex <==
\begin{figure}[b]
  \centering
  \includegraphics[width=\linewidth]{figures/grpo_comparison.pdf}
  % \caption{%
  %   \textbf{GRPO training dynamics vs.\ HeXA on Qwen-2.5-3B.}
  %   Val success rate (greedy, 50 seeds) across 10 training epochs for two GRPO variants
  %   on \texttt{down\_to\_earth} (left) and \texttt{two\_body\_problem} (right).
  %   One epoch $=$ 50 gradient steps $=$ each of the 50 training seeds seen once;
  %   log-scaled x-axis emphasises the low-data region.
  %   The green star marks \textsc{HeXA}'s result after the same 50-seed budget
  %   (DTE: $24\%$, TBP: $14\%$); base-model accuracy at zero seeds is $6\%$ and $4\%$ respectively.
  %   At the matched sample budget (vertical dashed line) both GRPO variants fall
  %   below \textsc{HeXA}; with sufficient training, GRPO eventually catches up
  %   or surpasses \textsc{HeXA} via direct optimisation on the exact environment reward.
  % }
\caption{%
  \textbf{In-context skill evolution learns faster than GRPO at the same interaction budget.}
  We compare \textsc{HExA} with GRPO fine-tuning on Qwen-2.5-3B using 50 training seeds.
  The green star marks \textsc{HExA}'s success rate after the same 50-seed budget
  (Down to Earth: $23.3\%$, Two Body Problem: $12\%$), while the dashed line marks the
  matched-budget GRPO checkpoint. In this low-data regime, \textsc{HExA} outperforms both
  GRPO variants, suggesting that reusable in-context skills provide faster early adaptation;
  with many more updates, GRPO can eventually close the gap through direct reward optimization.
}
  \label{fig:grpo_comparison_main}
\end{figure}


==> figures/hexa_fig1.tex <==
\begin{figure}[t]                                                                                                               
    \centering                                                                                                                                                                  
    \includegraphics[width=\linewidth]{NeurIPS_26/figures/HeXA_1.pdf}                                                                                                    
    \caption{%                                                                                                                                                                  
      \textbf{\textsc{HeXA} framework vs.\ standard ReAct on Interphyre physics puzzles.}                                                                                       
      \textbf{(a)}~Baseline ReAct: each seed is solved independently with no                                                                                                    
      cross-seed learning.                                                                                                                                                      
      Each seed consists of alternating \textcolor{teal}{\textbf{Get-State-Info}}                                                                                               
      calls (scene layout, gap analysis) and                                                                                                                                    
      \textcolor{orange}{\textbf{Simulate-Action}} calls (place red ball at $(x,y,r)$),                                                                                         
      terminating in success~(\cmark) or failure~(\xmark).                                                                                                                      
      \textbf{(b)}~\textsc{HeXA}: seeds are grouped into a \emph{meta-episode}.                                                                                                 
      After each seed, a teacher model distils the trajectory into a                                                                                                            
      \emph{Skill Bank} (physics principles + common mistakes); the evolved bank                                                                                                
      is injected into subsequent seeds' system prompts.                                                                                                                        
      \textbf{(Right)}~Cross-level transfer: skill banks evolved independently on                                                                                               
      $N_{\text{src}}$ source levels (\texttt{down\_to\_earth},                                                                                                                 
      \texttt{two\_body\_problem}, \texttt{pass\_the\_parcel}) are synthesised                                                                                                  
      by the teacher into a single cross-level bank for the target level                                                                                                        
      (\texttt{catapult}), with \emph{no target-level trajectories required}.                                                                                                   
    }                                                                                                                                                                           
    \label{fig:hexa_overview}                                                                                                                                                   
  \end{figure}                            

==> figures/hexa_smallmodels.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/hexa_smallmodels_app.pdf}
  \caption{%
    HeXA on open-weight solvers, evaluated on 50 seeds per cell.
    The skill bank lifts every model-level pair tested. Largest gains appear
    where headroom is greatest: Qwen-2.5-3B on \texttt{down\_to\_earth} ($+16$~pp,
    $3\times$ improvement), Qwen-2.5-7B on \texttt{two\_body\_problem} ($+16$~pp),
    and especially GPT-OSS-120B on \texttt{catapult} where the baseline
    scores $0\%$ and \textsc{HeXA} achieves $54\%$ ($+54$~pp).
    Numbers inside each bar are raw success / total counts; matching numbers
    appear in Table~\ref{tab:hexa_smallmodels}.
  }
  \label{fig:hexa_smallmodels}
\end{figure}


==> figures/training_curves.tex <==
% Both levels' instantiation trade-off, superimposed on one axis.
% Generated by Plots/create_paper_variants_scatter.py -> variants_scatter.pdf.
% This float replaced the side-by-side pair (catapult_scatter.pdf and
% ptp_scatter.pdf, both still generated); the two subfigure labels are kept
% as aliases so existing \ref's keep resolving.
\begin{figure}[t]
  \centering
  \includegraphics[width=0.60\linewidth]{figures/variants_scatter.pdf}
  \caption{%
    \textbf{Accuracy and cost move together, and one instantiation holds the
    corner on both levels.} Solve rate against mean turns to termination for
    every instantiation of the bank, Claude Sonnet, over the training seeds of
    each level; colour is the instantiation, shape is the level. Cheap and
    accurate is the upper left, shaded here; Off2On Evolving, written simply as
    \textsc{HExA}, is its only occupant on either level, and the arrows run from
    each level's \textsc{Zero-shot} floor to its \textsc{HExA} point. The
    remaining variants cluster in the middle and change order between levels.
    Failures count at the $25$-turn cap, and the $x$ axis is compressed below
    $10$ turns, where nothing is measured. Solve rates are those of
    Table~\ref{tab:variants_compact}.}
  \label{fig:training_curves}
  \label{fig:catapult_var_cum_accuracy}
  \label{fig:ptp_cum_accuracy}
\end{figure}


==> icsmrl_qwen3b.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textsc{ICMSRL} on Qwen-2.5-3B with the evolving variant
  ($x{=}3$ seeds / round, 17 rounds), evaluated on seeds $6$--$55$
  (50 seeds, last training seed dropped to align with other tables).
  Baseline rows are the same Qwen-2.5-3B agent without any skill injection.
}
\label{tab:icmsrl_qwen3b}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llccc}
\toprule
\textbf{Level} & \textbf{Method}
  & \textbf{Acc.\ (\%)}
  & \textbf{Succ.\ / Total}
  & \textbf{$\Delta$} \\
\midrule
\multirow{2}{*}{Down to Earth}
  & \textsc{ReAct} baseline       & \phantom{0}6.0 & 3 / 50 & --- \\
  & \textsc{ICMSRL} Online Evol.\ & \textbf{24.0} & 12 / 50 & $+18.0$ \\
\midrule
\multirow{2}{*}{Two Body Problem}
  & \textsc{ReAct} baseline       & \phantom{0}4.0 & 2 / 50 & --- \\
  & \textsc{ICMSRL} Online Evol.\ & \textbf{14.0} & 7 / 50 & $+10.0$ \\
\bottomrule
\end{tabular}
\end{table}


==> sections/2_interphyre_problem_setting.tex <==
\subsubsection{Learning through Experimentation}
\label{sec:problem-setup}

% \abhra{PLEASE EDIT}


% \sankaran{The Interphyre text is stale and needs a full rewrite. But I think this section should probably be the problem framing section, with Interphyre as a subsection. Would that work?}

% This project makes use of Interphyre, a reimplementation of the PHYRE simulator from scratch in Python using Box2D with procedural level generation and test-time intervention capabilities to support causal inference and mechanistic interpretability research. Interphyre contains a set of physical reasoning tasks with a fixed set of primitives: balls, bars, and baskets. Despite using the same objects with a standard set of colors, each level requires a different strategy to solve. Levels are also procedurally generated with randomized parameters, meaning that a large number of variants of the same task can be generated for the agent to solve. 

% In each task, the agent is shown a static initial state of the environment and has to determine where to place a ball in order to trigger the sequence of events that will lead to a goal condition such as getting another ball into a basket. Each episode is therefore a single forward pass for the agent. Prior work has explored methods to augment RL agents with intuitive physics simulators that enable them to plan ahead and simulate trajectories before taking actions, which is how many humans solve these tasks. In our work we try to analyze how LLM agents solve these tasks. 





 
% ── Motivation: why this environment exists for the exploration task ──
\scott{Not sure this section works here as-is. We either need to have a section that introduces the general problem setting first and our general framework, then this section as an instantiation, then our instantiation method. Or we need to turn this section *into* the problem statement, where we first introduce them problem and motivate Interphyre as a clean instantiation of that setting, and to set up a clear example that we can refer to later to more clearly explain what we are doing since we have a running example. Right now it is a little of both but isn't doing a great job a either and obscures the problem definition in instantiation details. I do worry also that, given that the paper is called HeXA, if we have too many sections before the section on the main method, reviewers will get lost/bored before even getting to what we are selling as the main point of the paper. So I lean toward the first option. We should *not* relegate Interphyre as an experimental detail. I want it to be co-equal of a contribution with the method, but I think it maybe should go second. But I'm open to arguments otherwise.}
Existing 2D physics benchmarks (PHYRE~\citep{bakhtin2019phyre}, I-PHYRE~\citep{li2024iphyre}, Kinetix~\citep{matthews2025kinetix}) were designed to answer one question: can the agent solve the puzzle?
In-context learning through exploration requires more from an environment: the agent must be able to \emph{interact} with the simulator as a tool, observe outcomes, form hypotheses, and refine its strategy---all without parameter updates.
No existing benchmark exposes the programmatic primitives this loop requires.
 
We introduce Interphyre, an extensible, intervention-aware 2D physics environment that instantiates the exploration task defined in \Cref{sec:problem-definition}.
The simulator and intervention API are exposed as a tool-call surface that an LLM agent can invoke directly (\texttt{inspect\_scene}, \texttt{place\_action}, \texttt{advance\_simulation}, \texttt{query\_success}), so that an LLM reasoner operating under a tool-use harness can drive the simulator in the same turn structure it would use for any other external tool.
A gymnasium-compatible interface~\citep{towers2024gymnasium} shares the same backend for standard RL training and evaluation.
Three observation modes---\texttt{physics\_state} (symbolic vector), \texttt{image} (RGB or discrete-color palette), and \texttt{both}---expose the same physics to different experimental designs, making observation modality a controlled variable rather than a design constraint.


\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/interventions_example.pdf}
  \caption{Interphyre's snapshot/restore API branches a shared mid-trajectory state into a
    factual rollout and perturbed alternatives (\Cref{sec:snapshot-restore}).
    Each row is one seed of the \texttt{catapult} level with a different oracle solution
    strategy.
    The leftmost column shows the initial scene for reference; the teal curve is the
    green ball's trajectory, shown up to the branch point in the \emph{Branch point}
    column and continuing through the outcome in each subsequent column.
    Top (seed\,8, deflector strategy): removing the deflector causes failure; shrinking
    the red action ball does not.
    Bottom (seed\,5, direct-launch strategy): shrinking the red ball causes failure;
    removing the deflector does not.
    The same interventions have opposite causal relevance across seeds, showing that causal
    relevance is a property of an object relative to the active strategy, not of the object
    in isolation.
    See \Cref{sec:worked-example} for the branching protocol.}
  \label{fig:intervention-example}
\end{figure*}


 
% % ── Key design features ──
% Four design decisions make Interphyre a substrate for exploration research.
 
% \paragraph{Levels as Python code.}
% Levels are Python classes built from a composable object API with user-defined success conditions; registering a new level makes it usable by the same evaluation pipeline as the bundled curriculum, with no package rebuild.
 
% \paragraph{Physics parameters as first-class inputs.}
% Physics parameters (gravity, friction, restitution, density, solver step size) are fields on a \texttt{SimulationConfig} object passed to the environment constructor, not constants compiled into the engine.
% The same level, seed, and action can be evaluated under any physically plausible parameter regime by swapping one configuration for another.
% Unlike Kinetix, which varies physics parameters jointly with level topology~\citep{matthews2025kinetix}, Interphyre keeps scene structure and parameter regime independent; a generalization study holds the level and seed fixed while sweeping gravity or friction.
 
% \paragraph{Oracle-verified curriculum.}
% The curriculum ships with 25 canonical levels, each paired with 10,000 pre-validated seeds, for 250,000 pre-certified task instances.
% Every seed is guaranteed to admit at least one solving action placement, verified by exhaustive oracle search over a discretized action grid.
% Oracle verification ensures that, up to the resolution of the action grid, every evaluation failure is attributable to the agent.
 
% \paragraph{Snapshot/restore and counterfactual branching.}
% Any running simulation can be snapshotted at an event-triggered branch point and restored into two or more independent branches that diverge under controlled perturbations (impulses, forces, parameter changes, object additions or removals).
% The environment is deterministic under a fixed seed, so the two branches share a bit-identical physical prefix---this is what makes a comparison genuinely paired.
% Perturbations are either \emph{kinematic} (modifying state of existing objects) or \emph{structural} (adding or removing objects), and a declarative trigger language (\texttt{on\_contact}, \texttt{on\_position\_threshold}, \texttt{when(predicate)}, etc.) decouples branch points from seed-specific timing.
 
% % ── Why this is hard / connection to the task ──
% Interphyre levels require the agent to reason about collision chains, impulse transfer, lever balance, aperture navigation, and unstable equilibria.
% The action space is continuous (placement of one or more balls or bars), the outcome depends on the full trajectory of contact events, and a strategy that succeeds under default physics may fail under altered parameters (\Cref{fig:parameter-sweep}).
% This makes the environment a challenging testbed for in-context exploration: the agent must use its limited interaction budget to identify which physical mechanism is operative and which action placement exploits it.
% Full design details, the intervention API specification, the level curriculum, and the worked counterfactual examples appear in \Cref{app:Interphyre}.















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{figures/agent_tool_figures}

Given the performance of the base LLM agents is primarily dependent on their parametric pretrained knowledge and is fundamentally unable to tackle harder non-trivial levels where novel strategies have to be developed, we thus devise methods that place interaction and exploration with such unseen tasks at the core of in-context learning algorithms. The agent interacts with Interphyre exclusively through a structured tool-call surface (Figure~\ref{fig:agent_tools}): \textcolor{teal}{\textbf{State Information Tools}} that query scene geometry without advancing the simulation, and \textcolor{orange}{\textbf{Simulation Tools}} that place the red ball and run the physics engine to observe outcomes. Our results validate our hypothesis that pretraining could only ever cover a tiny slice of all possible behaviours, and how we can devise in-context skill learning, composition, action taking strategies that fundamentally self-improve and scale with interaction and exploration in the environment, which the base LLMs are fundamentally incapable of doing themselves. We thus show how interaction, exploration, and experimentation are fundamental to improving model and agent capabilities on novel tasks and propose training-free in-context learning and self-improvement methods to improve both frontier and small open-LLM agent performance on Interphyre.

==> sections/3_experiential_agent_v5.tex <==
\section{Hierarchical Experimentalist Agents: Learning via Experimentation}
\label{sec:HExA}

\setlength{\emergencystretch}{2em}

\begin{figure}[h]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/skill_hexa_catapult.png}
    \caption{Example on \texttt{catapult} with its skill bank.}
    \label{fig:running_example}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Feedback_Loop.png}
    \caption{\textsc{HExA} actor--evolver--retriever loop.}
    \label{fig:hexa_loop2}
  \end{subfigure}
  \caption{%
    \textbf{\textsc{HExA} learns reusable skills through an actor--evolver--retriever loop.}
    \textbf{(a)}An example on \texttt{catapult} level illustrates the kind of physics reasoning skills \textsc{HExA} distills.
    \textbf{(b)} In each round, the actor generates reward-tagged trajectories, the evolver
    updates the skill bank, and the retriever injects the most relevant skills back into the
    actor for the next attempt.
  }
  \label{fig:hexa_overview_main}
\end{figure}

\textsc{HExA} is a training-free, in-context reinforcement learning framework in which an LLM agent
learns to solve unfamiliar tasks through active experimentation.
Rather than updating model weights, \textsc{HExA} improves across episodes by distilling interaction
experience into a persistent external \emph{skill bank}---a structured collection of natural-language
strategies and mistakes defined below---which is re-injected into the agent's context at the start
of each new episode.
This makes \textsc{HExA} compatible with any tool-augmented LLM, including closed-source models,
and requires no offline data, oracle supervision, or external teacher---only the environment's own
interaction feedback.
Unlike standard in-context RL, it requires no initial domain-specific training on reward-labeled data;
it learns self-improvement from scratch on each new task family. We use the \texttt{catapult} level from Interphyre as a running example throughout our paper, as shown in Figure~\ref{fig:catapult45_simframes} with the skill bank in Figure~\ref{fig:running_example}.
The agent has to choose where to place a red ball $(x,y)$ and its dimensions $r$---so that the ball falls and strikes a pivoting arm, launching a green ball into a distant basket. The full environment descriptions are in Appendix~\ref{app:Interphyre}.

% ------------------------------------------------------------------
\paragraph{Problem Setup.}
We consider task families $\ell$ whose instances $\{(\ell,s_j)\}$ each fix a specific
environment configuration: geometry, parameters, and initial conditions.
For each family $\ell$ we have a finite set of instances (or seeds) $\mathcal{S}_\ell=\{s_1,\ldots,s_{|\mathcal{S}_\ell|}\}$,
and episodes iterate through $\mathcal{S}_\ell$ in a fixed order.
For example, in \texttt{catapult}, $s_j$ sets the arm pose, deflector layout, and ceiling-blocker position. The agent has at most $T$ turns to solve $s_j$. We index turns by $t$ ($t = 0,1, \ldots,T-1$) and denote the entire experimentation trajectory for $s_j$ as $\tau_j$.

The agent interacts through a tool-call interface $\mathcal{F}$ provided by the environment. Interphyre supplies a set of shared tools available on every level---scene inspection, full and partial simulation, and contact logging---as well as some general level-specific analysis tools (shown in Appendix~\ref{app:tools} and Figure~\ref{fig:agent_tools}).
For example, \texttt{catapult} has access to tools like
\texttt{describe\_\allowbreak scene\_\allowbreak geometry},
\texttt{predict\_\allowbreak first\_\allowbreak contact(x,y,r)},
\texttt{simulate\_\allowbreak with\_\allowbreak trace(x,y,r,\allowbreak object\_\allowbreak names,\allowbreak stop\_\allowbreak step)},
and \texttt{finish(x,y,r)}.

At turn $t$, the agent observes the history $h_t=(a_0,o_0,a_1,o_1,\ldots,a_{t-1},o_{t-1})$ and selects the next action under actor policy $\pi_{\mathrm{act}}$.
For instance, in \texttt{catapult} a typical action is $a_t=\texttt{simulate\_\allowbreak with\_\allowbreak trace(0.5,0.4,1.5,\allowbreak["green\_ball"])}$,
returning a set of contact events and a kinematic summary (e.g.\ peak height, peak speed, and net displacement).
A binary predicate $\textsc{Goal}_\ell$ scores the completed simulation, where $\textsc{Sim}(\tau)$ executes trajectory $\tau$ in the environment and returns its final state.
The episode ends after at most $T$ turns or a terminal action, with success on seed $s_j$ defined as
\begin{equation}
\label{eq:success_main}
y_j(\pi_{\mathrm{act}};\ell) =
\mathbb{I}\!\left[\textsc{Goal}_\ell\!\left(\textsc{Sim}(\tau_j)\right)=\text{true}\right],
\qquad
\tau_j \sim \pi_{\mathrm{act}}(\cdot \mid \ell, s_j).
\end{equation}

% ------------------------------------------------------------------


\begin{algorithm}[t]
\LinesNotNumbered
\caption{\textsc{HExA}}
\label{alg}
\DontPrintSemicolon
\small
\SetInd{0.6em}{0.8em}
\KwIn{Actor $\pi_{\mathrm{act}}$, evolver $\pi_{\mathrm{ev}}$, level $\ell$, seeds of that level $\mathcal{S}_\ell$, rounds $R$, episodes per round $x$}
\BlankLine
\tcp{Optional warm start (first round only)}
$\mathcal{K}_0 \gets  \pi_{\mathrm{ev}}(\emptyset,\,\mathcal{T}_0)$ \textbf{or} $\mathcal{K}_0\gets\emptyset$\;
\BlankLine
\For{$n = 1,\ldots,R$}{
  $\mathcal{G}_n \gets \textsc{Retriever}(\mathcal{K}_{n-1},\ell,M,N)$
    \tcp*{top-$M$ skills + top-$N$ mistakes}
  \For{$i = 1+x*(n-1),\ldots,x*n$}{
    $\tau_i \gets \pi_{\mathrm{act}}(\cdot \mid \ell,\, s_i,\, \mathcal{G}_n)$
      \tcp*{actor prompt: task + tools + skills}
    $r(\tau_i) \gets \textsc{Reward}(\tau_i)$
      \tcp*{outcome $\times$ efficiency; see Appendix~\ref{sec:reward}}
  }
  $\mathcal{K}_n \gets  \pi_{\mathrm{ev}}(\mathcal{K}_{n-1},\,\mathcal{T}^{(n)})$
    \tcp*{evolver prompt: bank + trajectories + rewards}
}
\KwRet{$\mathcal{K}_R$}
\end{algorithm}





\paragraph{The \textsc{HExA} Loop.}


As shown in Figure~\ref{fig:hexa_loop2} and ~\ref{fig:hexa_loop}, each round of \textsc{HExA} runs as follows: a \emph{retriever} selects the most relevant entries
from the current skill bank~$\mathcal{K}$ and injects them into the \emph{actor}'s context; the
actor runs $x$ episodes under that skill context, each scored by a reward; and an \emph{evolver}
reads the resulting batch of trajectories and updates~$\mathcal{K}$.
On the first round, $\mathcal{K}$ may start empty or be warm-started from an offline batch of
base-actor trajectories; every subsequent round is identical.
Algorithm~\ref{alg} gives the full loop; initialization and update strategies are ablated in
Section~\ref{sec:experiments}. \textsc{HExA} couples three components: an \emph{actor} $\pi_{\mathrm{act}}$ (any tool-augmented LLM) that reasons about experimental hypotheses to test and performs experiments via exploration, interventions and interactions with the environment to generate trajectories; an \emph{evolver} $\pi_{\mathrm{ev}}$
(LLM call to the same model with an evolver prompt) that reads batches of actor trajectories and distills them into an external
\emph{skill bank}~$\mathcal{K}$; and a \emph{retriever} that selects the most relevant entries
from~$\mathcal{K}$ and injects them into the actor's context before each episode.
We now describe each component in terms of the prompt it receives, what it produces, and why
the step is necessary.

\paragraph{Actor prompt and skill-augmented episode.} At the start of each episode, the actor receives a prompt containing the task description, the
available tools~$\mathcal{F}$, and a \emph{skill context}~$\mathcal{G}$ retrieved from the
current skill bank: 
\begin{equation}
\label{eq:skill-augmented_main}
\begin{aligned}
\mathcal{G} &= \textsc{Retriever}(\mathcal{K},\ell,M,N), 
\tau_j &\sim \pi_{\mathrm{act}}(\cdot \mid \ell, s_j, \mathcal{G}).
\end{aligned}
\end{equation}
Equation~\ref{eq:success_main} defines the task without method-specific assumptions; any agent---including
skill-free baselines such as \textsc{Direct} (base model's zero-shot interactions) or \textsc{ReAct}---can be evaluated against it.
\textsc{HExA} augments the actor with skill context $\mathcal{G}$ as in Eq.~\ref{eq:skill-augmented_main},
replacing the base policy $\pi_{\mathrm{act}}(\cdot\mid\ell,s_j)$ with the skill-conditioned version.
The skill context $\mathcal{G}$ consists of the top-$M$ skills and top-$N$ mistake records from the bank, ranked using the skill reward labels defined below, prepended as a fixed-size prefix to the actor's system prompt alongside the standard task description and tool documentation.
On the first episode, $\mathcal{K}$ may be empty or warm-started (see below); from the second episode
onward, it contains skills distilled from prior rounds.
The injection mechanism is deliberately simple---it changes only the textual context, not the
agent's architecture or decoding---so \textsc{HExA} works with any tool-augmented LLM.
The actor is free to use or disregard individual skills based on its own reasoning about the current
instance.

\paragraph{Trajectory reward.}
\label{para:traj_reward}
Each trajectory $\tau$ receives a scalar reward $r(\tau)\in[-1,+1]$ reflecting both
\emph{outcome} (success or failure) and \emph{efficiency} (how quickly the outcome was reached,
as a fraction of the budget $T$).
Fast, decisive successes earn higher rewards; failures are penalized less when the agent explored
extensively before failing, since such trajectories yield richer material for the evolver than one
that abandoned the episode after a single attempt.
We use discrete reward bins rather than a continuous function because the evolver is an LLM: it can reliably act on qualitative categories (fast success, slow success, exploratory failure, early
exit) ~\citep{viswanathan2026discretizingrewardmodels,gunjal2025rubrics}, but cannot meaningfully distinguish, say, $r{=}0.73$ from $r{=}0.71$.
The exact reward function is given in Appendix~\ref{sec:reward}.








\paragraph{Evolver prompt and skill distillation.} After each round $n$ ($n=1,\ldots,R$, where $R=\lvert\mathcal{S}_\ell\rvert/x$) of $x$ trajectories, the evolver receives a prompt containing the current skill
bank~$\mathcal{K}_{n-1}$, the new batch $\mathcal{T}^{(n)}$ (each trajectory rendered as its
\texttt{(thought,\allowbreak tool\_\allowbreak call,\allowbreak observation)} sequence tagged with its
reward), and a structured-output instruction. The instruction directs the evolver to use rewards for evaluating trajectory quality and \emph{contrast} high-reward behaviors against low-reward ones, to learn the unique lessons of success over failure based on the observations. From this, the evolver produces two types of distilled knowledge.

\emph{Strategy skills} are extracted by contrasting high-reward against low-reward trajectories, yielding a set of new skills. Each skill is a structured record defined by a \emph{title}, a \emph{principle} (the insight gained from testing the proposed hypothesis via experimentation), a \emph{when-to-apply} condition, an optional demonstrative \emph{example}, the \emph{source seed} it was derived from, and a \emph{reward score} defined below.
For example, the round-14 \texttt{catapult} skill \texttt{cat\_\allowbreak ev\_\allowbreak 1\_\allowbreak 001}
(Appendix~\ref{app:trajectories:bank}): title ``$x\!\approx\!0.5$ is the primary launch sweet spot,''
principle ``placing the red ball at $x{=}0.5$ gives a consistent rightward launch; deviate to $x{=}0.3$
only on a ceiling hit,'' applicability ``always as the first placement attempt.''

\emph{Mistake records} are extracted from failures alone, yielding records $\mu=(\delta,\rho,\alpha)$
pairing a description~$\delta$, a root cause~$\rho$, and a corrective action~$\alpha$.
For example: $\delta$ ``the agent fixates on one launch point and micro-tunes $x/y/r$,''
$\rho$ ``the arm is the obvious mechanism, so failures are met with small perturbations,''
$\alpha$ ``after two failures within $x\pm0.2$, move to a different $x$ zone.''
The evolver also recovers \emph{partial skills} from otherwise-failed trajectories: reasoning steps
that were individually correct even though the episode failed overall.
For example, a trajectory that correctly identifies the catapult arm as the target mechanism but then
micro-tunes placement in the wrong direction yields a partial skill encoding the correct mechanism
identification, even though the solve failed.
This is a learning signal unavailable from successful trajectories alone, since successes do not
reveal which intermediate steps were necessary versus incidental. Skills are extracted while the agent already holds previously learned ones, so later skills can
build on earlier ones.
Whether this compounds into a hierarchy of increasingly abstract principles is an empirical question
we investigate in Section~\ref{sec:experiments}.
Full evolver prompt templates are in Appendix~\ref{sec:distillation}.




\begin{skillbankbox}
\scriptsize

\textit{Before attempting seed 45, \textsc{HExA} receives a skill bank distilled from
earlier \texttt{catapult} episodes. The entries below show how it turns the
observed trajectory into a structured decision.}

\begin{skillentry}
  {skillblue}{skillbluebg}
  {Skill 1: \textsc{Default} $\triangleright$ Start from a stable launch geometry}
Place the red ball near $x=0.5$ with sufficiently large radius. This contact
point provides a stable lever arm and usually produces a strong rightward launch.

\textbf{Use when:} Use as the initial launch hypothesis for a new seed; deviate when the trajectory hits the ceiling or violates placement constraints.

\end{skillentry}

\begin{skillentry}
  {skillamber}{skillamberbg}
  {Skill 2: \textsc{Diagnose} $\triangleright$ Recognize the radius plateau}
At fixed $x=0.5$, increasing the radius beyond approximately $r=1.5$ may not
increase range because the arm reaches its rotational limit. More mass therefore
does not necessarily produce a better trajectory.

\textbf{Use when:} A large-radius launch still fails; stop assuming that additional force alone will solve the problem. For example ff $r=1.5$ fails at $x=0.5$, change the contact geometry rather than continuing to increase $r$.
\end{skillentry}

\begin{skillentry}
  {skillgreen}{skillgreenbg}
  {Skill 3: \textsc{Correct} $\triangleright$ Flatten a ceiling-blocked trajectory}
If a smaller radius falls short while a larger radius strikes the ceiling, the
bottleneck is launch angle rather than energy. Shift $x$ toward $0.1$--$0.3$
to change the arm-contact geometry and flatten the launch arc.

\textbf{Use when:} After two radius variations at the same $x$ produce one short trajectory and one ceiling collision, stop tuning $r$ and explore a different $x$ region.
\end{skillentry}

\begin{skillentry}
  {skillred}{skillredbg}
  {\textsc{Avoid} $\triangleright$ Local parameter fixation} The agent repeatedly micro-tunes $(x,y,r)$ around the same unsuccessful launch point because the catapult arm appears to be the correct mechanism.

\textbf{Correction:} After repeated failures in the same neighborhood, change
the relevant search dimension or move to a qualitatively different placement region.
\end{skillentry}

% \begin{tcolorbox}[
%   enhanced,
%   colback=skillgreen!8,
%   colframe=skillgreen,
%   boxrule=0.7pt,
%   arc=1.5mm,
%   left=5pt,
%   right=5pt,
%   top=4pt,
%   bottom=4pt,
%   before skip=4pt,
%   after skip=1pt
% ]
\vspace{1em}
\textbf{How the bank guides seed 45.}
\textsc{HExA} first tests the learned default launch and observes a ceiling
overshoot. The bank identifies this as a geometry problem rather than a
lack-of-force problem, so the agent shifts the drop point from the
$x\approx0.5$ region to $x=0.3$ instead of continuing to increase the radius.
It then succeeds with $(x,y,r)=(0.3,0.9,1.5)$ in six interaction iterations
(Figure~\ref{fig:catapult45_simframes}).

\[
\underbrace{\text{default launch}}_{\textcolor{skillblue}{\text{prior skill}}}
\;\longrightarrow\;
\underbrace{\text{ceiling hit}}_{\textcolor{skillamber}{\text{observation}}}
\;\longrightarrow\;
\underbrace{\text{shift contact geometry}}_{\textcolor{skillgreen}{\text{correction}}}
\;\longrightarrow\;
\underbrace{\text{success}}_{\textcolor{skillgreen}{\text{6 iterations}}}
\]
% \end{tcolorbox}

% \textit{Abstraction ladder:}\quad
% concrete experiments
% $\rightarrow$ diagnosed physical mechanism
% $\rightarrow$ conditional search policy.
\label{promptbox:skillbank}
\end{skillbankbox}




\paragraph{Skill bank and retrieval.}
\label{sec:skill_bank_retrieval_main}
Distilled knowledge is stored in the skill bank $\mathcal{K}$ with two collections, both indexed by
task family: a set of \emph{skills} (reusable strategies and principles) and a set of \emph{mistakes}
(recurring failure modes to avoid).
Each skill carries a \emph{reward score} $r_k$, computed from the trajectories that demonstrated or used it, as a function of the mean reward of these source trajectories ($\bar{r}_{\mathrm{src}}$). We show an example of this reward label in Section~\ref{sec:instantiation} with the individual trajectory rewards demonstrated in Appendix~\ref{sec:reward}. This reward label is used for two purposes: ranking skills during retrieval (top-$M$ by $r_k$), and guiding the evolver in deciding which skills to retain or prune when the bank is at capacity. Skills derived from fast, efficient successful trajectories carry higher scores; skills from partial reasoning within failed trajectories carry lower scores but may still encode valuable learnings and discoveries.

The bank is capped at $M_{\max}$ skills and $N_{\max}$ mistakes per task family to prevent the injected context from growing without bound and to force the evolver to prioritize the most informative knowledge. Full bank structure and retrieval details are in Appendix~\ref{app:hexa}.



The abridged skill bank above shows the information available to \textsc{HExA} \emph{before} it attempts \texttt{catapult} seed~45. Unlike raw trajectory memory, the bank organizes evidence from earlier episodes into a default hypothesis, diagnostic conditions, corrective strategies, and mistakes to avoid. Figure~\ref{fig:catapult45_simframes} subsequently shows how these skills guide the successful \textsc{HExA} trajectory. We can also see how skills from individual experimental and interaction observations are composed together by HExA to from hierarchical and reusable general skills. 


% ------------------------------------------------------------------
\paragraph{Cross-task skill transfer.}

The same mechanism supports transfer across task families.
Low-level details such as source-task coordinates or object identities are generally not directly
reusable, whereas the mechanism-level abstractions distilled above---such as contact geometry
controlling impulse direction, moment arm controlling torque, or collision order controlling
downstream motion---can remain valid under a different scene configuration.
Given evolved source banks $\mathcal{K}_{\ell_1},\ldots,\mathcal{K}_{\ell_S}$ and only a textual
description of an unseen target family $\ell^*$, the evolver synthesizes a target bank without
observing any target-task trajectories.
It (i)~selects source skills whose underlying physical or search principles are structurally
relevant to $\ell^*$, (ii)~removes source-specific parameter and entity bindings, (iii)~re-grounds
each principle in the entities, constraints, and tools of $\ell^*$, and (iv)~assigns a transfer
score according to the directness of the structural correspondence and the degree of corroboration
across source banks.

This procedure transfers abstractions rather than memorized solutions: the evolver is prohibited
from inventing target-specific coordinates and must express each transferred skill as a mechanism
and an applicability condition.
For example, evidence about lever-mediated impulse transfer from several source levels can be
re-grounded in the pivoting arm and launch dynamics of \texttt{catapult}, even though no successful
\texttt{catapult} placement has been observed.
The resulting bank $\mathcal{K}_{\ell^*}$ is injected through the same retriever, enabling zero-shot
cross-task transfer, or used as the initialization $\mathcal{K}_0$ for a subsequent within-task
\textsc{HExA} run.
Full transfer prompts are in Appendix~\ref{app:prompt:cross_level_full}; results are in
Section~\ref{sec:experiments}.

==> sections/3_experimental_agent_v_ICLR.tex <==
% Replace the existing main-paper HExA method section with this file.
% Figure, algorithm, and external-reference dependencies use the existing project.
\section{Hierarchical Experimentalist Agents: Learning via Experimentation}
\label{sec:HExA}

\setlength{\emergencystretch}{2em}

\begin{figure}[h]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/skill_hexa_catapult.png}
    \caption{Example on \texttt{catapult} with its skill bank.}
    \label{fig:running_example}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Feedback_Loop.png}
    \caption{\textsc{HExA} actor--evolver--retriever loop.}
    \label{fig:hexa_loop2}
  \end{subfigure}
  \caption{%
    \textbf{\textsc{HExA} learns reusable skills through an actor--evolver--retriever loop.}
    \textbf{(a)}An example on \texttt{catapult} level illustrates the kind of physics reasoning skills \textsc{HExA} distills.
    \textbf{(b)} In each round, the actor generates reward-tagged trajectories, the evolver
    updates the skill bank, and the retriever injects the most relevant skills back into the
    actor for the next attempt.
  }
  \label{fig:hexa_overview_main}
\end{figure}

\textsc{HExA} is a training-free, in-context reinforcement learning framework that
learns from active experimentation by distilling experience into a persistent external
\emph{skill bank} $\mathcal{K}$ of natural-language strategies and mistakes. The bank
augments subsequent episodes without parameter updates, externally supplied offline
data, oracle supervision, or an external teacher. We use Interphyre's
\texttt{catapult} as a running example: the agent chooses a red-ball placement
$(x,y,r)$ to strike a pivoting arm and launch a green ball into a distant basket
(Figures~\ref{fig:running_example} and~\ref{fig:catapult45_simframes}; environment
details in Appendix~\ref{app:Interphyre}).

\paragraph{Problem setup.}
A task family $\ell$ contains instances $\{(\ell,s_j)\}$, with seeds
$\mathcal{S}_\ell=\{s_1,\ldots,s_{|\mathcal{S}_\ell|}\}$ specifying geometry,
parameters, and initial conditions. Episodes follow a fixed seed order. Each episode
has at most $T$ turns, indexed by $t\in\{0,\ldots,T-1\}$, and produces a trajectory
$\tau_j$. Through the environment's tool interface $\mathcal{F}$, the actor
$\pi_{\mathrm{act}}$ selects actions from the history
$h_t=(a_0,o_0,a_1,o_1,\ldots,a_{t-1},o_{t-1})$, where $a_i$ is a tool invocation
and $o_i$ its observation. Interphyre provides scene inspection, simulation, and
contact logging, with level-specific analysis tools
(Appendix~\ref{app:tools}; Figure~\ref{fig:agent_tools}). An episode ends at a terminal
action or the turn limit. With $\textsc{Sim}(\tau)$ returning the final simulation
state and $\textsc{Goal}_\ell$ the binary goal predicate, success is
\begin{equation}
\label{eq:success_main}
y_j(\pi_{\mathrm{act}};\ell) =
\mathbb{I}\!\left[\textsc{Goal}_\ell\!\left(\textsc{Sim}(\tau_j)\right)=\text{true}\right],
\qquad
\tau_j \sim \pi_{\mathrm{act}}(\cdot \mid \ell, s_j).
\end{equation}

\begin{algorithm}[t]
\LinesNotNumbered
\caption{\textsc{HExA}}
\label{alg}
\DontPrintSemicolon
\small
\SetInd{0.6em}{0.8em}
\KwIn{Actor $\pi_{\mathrm{act}}$, evolver $\pi_{\mathrm{ev}}$, level $\ell$, seeds of that level $\mathcal{S}_\ell$, rounds $R$, episodes per round $x$}
\BlankLine
\tcp{Optional warm start (first round only)}
$\mathcal{K}_0 \gets  \pi_{\mathrm{ev}}(\emptyset,\,\mathcal{T}_0)$ \textbf{or} $\mathcal{K}_0\gets\emptyset$\;
\BlankLine
\For{$n = 1,\ldots,R$}{
  $\mathcal{G}_n \gets \textsc{Retriever}(\mathcal{K}_{n-1},\ell,M,N)$
    \tcp*{top-$M$ skills + top-$N$ mistakes}
  \For{$i = 1+x*(n-1),\ldots,x*n$}{
    $\tau_i \gets \pi_{\mathrm{act}}(\cdot \mid \ell,\, s_i,\, \mathcal{G}_n)$
      \tcp*{actor prompt: task + tools + skills}
    $r(\tau_i) \gets \textsc{Reward}(\tau_i)$
      \tcp*{outcome $\times$ efficiency; see Appendix~\ref{sec:reward}}
  }
  $\mathcal{K}_n \gets  \pi_{\mathrm{ev}}(\mathcal{K}_{n-1},\,\mathcal{T}^{(n)})$
    \tcp*{evolver prompt: bank + trajectories + rewards}
}
\KwRet{$\mathcal{K}_R$}
\end{algorithm}

\paragraph{The \textsc{HExA} loop.}
Algorithm~\ref{alg} alternates retrieval, experimentation, and skill evolution
(Figures~\ref{fig:hexa_loop2} and~\ref{fig:hexa_loop}). In round $n$, the retriever
selects context $\mathcal{G}_n$ from $\mathcal{K}_{n-1}$; the actor runs $x$
episodes; and the evolver $\pi_{\mathrm{ev}}$ updates the bank from their
reward-tagged trajectories $\mathcal{T}^{(n)}$. The initial bank $\mathcal{K}_0$
is empty or distilled from a batch $\mathcal{T}_0$ of base-actor trajectories.
Initialization and update variants are specified in Appendix~\ref{sec:regimes}
and evaluated in Section~\ref{sec:experiments}.

\paragraph{Skill-augmented actor.}
The actor receives the task description, tools $\mathcal{F}$, and retrieved context
\begin{equation}
\label{eq:skill-augmented_main}
\mathcal{G} = \textsc{Retriever}(\mathcal{K},\ell,M,N),
\qquad
\tau_j \sim \pi_{\mathrm{act}}(\cdot \mid \ell, s_j, \mathcal{G}).
\end{equation}
The context contains the top-$M$ skills ranked by their reward scores and top-$N$
mistake records, prepended to the system prompt. This changes only the textual
context, not the architecture or decoding; the actor decides which skills apply.
Equation~\ref{eq:success_main} remains the evaluation criterion for both
skill-conditioned and skill-free agents, including \textsc{Direct} and
\textsc{ReAct}. Retrieval details are in Appendix~\ref{sec:retrieval}.

\paragraph{Trajectory reward.}
\label{para:traj_reward}
Each trajectory receives $r(\tau)\in[-1,+1]$ based on outcome and efficiency
relative to the turn budget $T$. Faster successes receive higher rewards, while
longer exploratory failures receive smaller penalties because they may provide more
useful evidence for distillation. Discrete reward bins communicate qualitative
trajectory differences to the evolver
~\citep{viswanathan2026discretizingrewardmodels,gunjal2025rubrics}; the exact
function is given in Appendix~\ref{sec:reward}.

\paragraph{Evolver and skill distillation.}
After round $n=1,\ldots,R$, where $R=|\mathcal{S}_\ell|/x$, the evolver receives
$\mathcal{K}_{n-1}$ and $\mathcal{T}^{(n)}$, with trajectories rendered as
reward-tagged \texttt{(thought, tool\_call, observation)} sequences. It contrasts
high- and low-reward trajectories to extract strategy skills, and analyzes failures
to extract mistake records $\mu=(\delta,\rho,\alpha)$: a description $\delta$,
root cause $\rho$, and correction $\alpha$. It also recovers \emph{partial skills}
from useful intermediate reasoning in failed episodes. Because later trajectories
are conditioned on earlier skills, new skills can refine or compose prior knowledge;
Section~\ref{sec:experiments} examines this hierarchical structure. The two-phase
procedure, record schemas, and examples are detailed in
Appendix~\ref{sec:distillation}.

\paragraph{Skill bank and retrieval.}
\label{sec:skill_bank_retrieval_main}
The bank stores task-indexed skills and mistakes. Each skill's reward score $r_k$
is derived from the mean reward $\bar{r}_{\mathrm{src}}$ of its source trajectories
(Section~\ref{sec:instantiation}; Appendix~\ref{sec:skillbank}), guiding both
retrieval and retention or pruning. Caps of $M_{\max}$ skills and $N_{\max}$
mistakes per family bound the number of stored entries. Unlike raw trajectory memory,
the bank organizes prior evidence into reusable hypotheses, diagnostic conditions,
and corrective strategies. The worked bank in Appendix~\ref{sec:worked-skillbank}
and full bank in Appendix~\ref{app:trajectories:bank} show how these abstractions
guide the seed-45 trajectory in Figure~\ref{fig:catapult45_simframes}.

\paragraph{Cross-task skill transfer.}
Given source banks $\mathcal{K}_{\ell_1},\ldots,\mathcal{K}_{\ell_S}$ and only a
textual description of an unseen target family $\ell^*$, the evolver synthesizes
$\mathcal{K}_{\ell^*}$ by selecting and re-grounding relevant source principles,
without observing target-task trajectories. The resulting bank is injected through
the same retriever for zero-shot transfer or used as $\mathcal{K}_0$ for subsequent
within-task evolution. The full synthesis procedure is in
Appendix~\ref{sec:transfer}, transfer prompts in
Appendix~\ref{app:prompt:cross_level_full}, and results in
Section~\ref{sec:experiments}.


==> sections/4_exp_results_Jun24.tex <==
\section{Experiments and Results on Interphyre}
\label{sec:experiments}

In this section, we provide details of \textsc{Interphyre}, and evaluate different LLMs on experiment-centric tasks using \textsc{Interphyre} levels. Our benchmark is designed with the following key properties:

\begin{enumerate}[label=(\roman*)]
    \item tasks whose solution is unknown or cannot be read off a static description and must be discovered by interacting with the environment
    \item a programmatic interface that lets the agent inspect the scene, test interventions, and observe intermediate dynamics
    \item a controllable difficulty range with procedural generation
\end{enumerate}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/interventions_example.pdf}
  \caption{\textbf{\textsc{Interphyre}'s snapshot/restore API.} This branches a shared mid-trajectory state into a
    factual rollout and perturbed alternatives (Section \ref{sec:snapshot-restore}).
    Each row is one seed of the \texttt{catapult} level with a different oracle solution
    strategy.
    The leftmost column shows the initial scene for reference; the teal curve is the
    green ball's trajectory, shown up to the branch point in the \emph{Branch point}
    column and continuing through the outcome in each subsequent column.
    Top (seed\,8, deflector strategy): removing the deflector causes failure; shrinking
    the red action ball does not.
    Bottom (seed\,5, direct-launch strategy): shrinking the red ball causes failure;
    removing the deflector does not.
    The same interventions have opposite causal relevance across seeds, showing that causal
    relevance is a property of an object relative to the active strategy, not of the object
    in isolation.
    See Section \ref{sec:worked-example} for the branching protocol.}
  \label{fig:intervention-example_main_paper}
\end{figure}

\subsection{\textsc{Interphyre}: A Testbed for Learning through Experimentation}
\label{sec:Interphyre_example}

Unlike benchmarks that primarily ask whether an agent can solve a task or answer a query, our setting requires an environment in which the agent can deliberately interact and gather evidence: inspecting the current instance, testing interventions, observing intermediate dynamics, diagnosing failures, and reusing what it learned across future seeds and levels in an experimentation loop. \textsc{Interphyre} provides this in a controlled 2D physics domain with continuous actions and long-horizon causal structure. Each task requires placing a red ball at $(x,y,r)$, after which the simulator evaluates whether the level-specific success predicate is achieved.

\textsc{Interphyre} builds on the level designs in the PHYRE benchmark \citep{bakhtin2019phyre} by introducing APIs for level editing, test-time interventions on environment parameters, and logging traces from the simulation. These APIs can be used to customize the benchmark for evaluating agents on unseen levels, or provided to an LLM for active experimentation. In particular, our experiments use the \textsc{Interphyre} API to expose a structured tool-calling interface for experimentation via interventional scene inspection, partial simulation, full rollouts, contact logs, and level-specific geometric analysis, for example as shown in Figure \ref{fig:intervention-example_main_paper}. However, successful actions often depend on contact chains, lever mechanics, collision timing, and strategy-dependent dynamics. Even strong LLMs struggle to anticipate such interactions reliably during inference, particularly when only given the scene description. Now using these intervention API and traces recovered from \textsc{Interphyre} runs, HExA enables the LLM agent to reason over its proposed hypothesis and corresponding experimental observations, than merely guessing solutions from parametric prior knowledge. This lets the agent leverage the information acquired through exploration and interactions, to improve its performance in-context. \textsc{Interphyre} therefore serves as both a benchmark and a diagnostic environment for experimentation based methods such as \textsc{HExA}. We provide full details of the environment design, curriculum, tool API, observation modes, and prompts in Appendix~\ref{app:Interphyre} and \ref{app:systemprompts}.


\subsection{Experimental Setup, Evaluations, and Baselines}
\label{sec:setup}




\setlength{\intextsep}{2pt}          % less vertical space above/below the float
\setlength{\columnsep}{10pt}         % gap between table and wrapped text

\begin{wraptable}{r}{0.58\linewidth}
\vspace{-\baselineskip}              % pull the table up toward the section top (optional)
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{3pt}
\caption{%
Base LLM agent's (\textsc{Zero-Shot} baseline) solve rate~(\%) across eight \textsc{Interphyre} levels. \textsuperscript{$\dagger$} Pass the Parcel and Catapult evaluated over 50 seeds; all other levels evaluated over 100 seeds.}
\label{tab:direct_baseline_results_main}
\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} cccccc}
\toprule
& \textbf{Rand} & \textbf{Q-7B} & \textbf{Q-14B}
& \textbf{O-20B} & \textbf{O-120B} & \textbf{Sonnet} \\
\midrule
Cliffhanger             & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0             \\
Tipping Point           & 3  & 0.0  & 3.0  & 8.0  & 2.0  & 0.0             \\
Basket Case             & 4  & 0.0  & 2.0  & 14.0 & 13.0 & 9.0             \\
Down to Earth           & 8  & 18.0 & 0.0  & 16.0 & 3.0  & 14.0            \\
Two Body                & 14 & 4.0  & 16.0 & 13.0 & 1.0  & 68.0            \\
Falling in Place        & 1  & 8.0  & 1.0  & 3.0  & 29.0 & 23.0            \\
\underline{Pass the Parcel} & 0  & 0.0  & 0.0  & 0.0  & 3.0  & 0.0$^{\dagger}$ \\
\underline{Catapult}        & 0  & 0.0  & 0.0  & 0.0  & 0.0  &0.0$^{\dagger}$ \\
\bottomrule
\end{tabular*}
\end{wraptable}



We evaluate five LLMs including frontier black box and small open LLMs---Claude Sonnet~4.6, Qwen-2.5-\{7B, 14B\} Instruct, GPT-OSS-\{20B,120B\}, and a random agent (a heuristic policy that samples uniformly from the valid placement region, with no interaction with the environment)---each capped at 25 interaction turns per trajectory on \textsc{Interphyre} levels. We compare against three baselines: \emph{\textsc{ReAct}}~\citep{yao2023reactsynergizingreasoningacting}, which runs one Thought-Action-Observation trajectory per seed; \emph{Reflexion}~\citep{shinn2023reflexion}, which adds verbal self-reflection; and \emph{\textsc{Zero-Shot}}, which prompts the model to solve the task in a single shot from the scene description alone, with no tools, no environment interaction, and no skills, measuring the base models' parametric capability. With the smaller models, we also include RL training via \emph{GRPO}~\citep{shao2024deepseekmath}, which fine-tunes Qwen-2.5-3B with a binary $\{0,1\}$ reward, making it the only method that updates model weights and compares directly against our training-free framework. All methods on a given level are evaluated on the same 50 seeds, so comparisons are paired on identical instances (full details in Appendix~\ref{app:baselines}). In Table~\ref{tab:direct_baseline_results_main} above and Table~\ref{tab:baseline_results} in Appendix~\ref{app:results}, we organize the eight levels into two difficulty tiers based on base LLM performance (Zero-Sh) and its performance with ReAct as agent baseline: Tier~1 (the first six levels),  and Tier~2 (\texttt{pass\_the\_parcel} at $0\%$, \texttt{catapult} at $2\%$, with every open-weight model scoring $0\%$ on the latter). These two hard levels from Tier~2, where purely parametric reasoning is insufficient, are the primary testbed for \textsc{HExA}. Throughout, we report two metrics: \emph{solve rate} (\% of seeds satisfying $\textsc{Goal}_\ell$, Eq.\ref{eq:success_main}) for task success accuracy and average turns per seed (unsolved seeds capped till maximum 25 turns) for efficiency.

% =====================================================================
% PREVIOUS VERSION (kept for reference) --- replaced by the more concise
% version below.
% =====================================================================
% \subsection{Instantiation of \textsc{HExA} -- Skill Initialization and Update}
% \label{sec:instantiation}
% The skill bank in \textsc{HExA} can have several configurations that vary along two orthogonal axes (Algorithm~\ref{alg})---how the skill bank is initialized before experimentation starts and how it is updated between the experimentation rounds. We tested three initialization methods for our skill banks: \emph{Offline}, \emph{Offline to Online} (\emph{Off2On}), and \emph{Online}. Both Offline and Off2On, warm-start the bank by collecting $N_0$ base-actor trajectories with no skill context and distilling them into $\mathcal{K}_0=\textsc{Evolver}(\emptyset,\mathcal{T}_0)$. In the Offline variant we do not update the skills anymore, while in Off2On we reinitialize the skill bank after new experiments. In the pure Online version, we start with an empty bank ($\mathcal{K}_0=\emptyset$) and the agent bootstrap skills
% purely from its own online interactions. We also have two ways to update the skill bank from interaction feedback: \emph{Evolving} and \emph{Iterative
% Replacement}. The Evolving variant passes the evolver both the current bank and the new round's trajectories, adding new skills and merging, revising, or
% pruning existing skills in light of new experimental evidence
% ($\mathcal{K}_n=\textsc{Evolver}(\mathcal{K}_{n-1},\mathcal{T}^{(n)})$). However, in Iterative Replacement,   we build the skill bank from scratch each time using the current set of rollouts alone, since we assume that in the in-context RL loop, the actor has ingested the previous skills in its policies already. Thus, these newer skills already have the influence of older skills plus additional novelty from these newer experimentation rollouts ($\mathcal{K}_n=\textsc{Evolver}(\emptyset,\mathcal{T}^{(n)})$). We thus have five variants of skill formation and updation—initialization with either \textit{Off2On} or
% \textit{Online} and updation with either \textit{Evolution} or \textit{Iterative Replacement}. And another version where we
% start with a fixed Offline skill bank, and keep it frozen throughout the experiments with no update ($\mathcal{K}_n=\mathcal{K}_{n-1}$). We ablate all five instantiations in Table~\ref{tab:variants_compact} and \emph{Off2On~+~Evolution} performs the best---we thus use this version of skill initialization and update as the default in \textsc{HExA}.
% =====================================================================

\subsection{Instantiation of \textsc{HExA} -- Skill Initialization, Update, and Reward Labels}
\label{sec:instantiation}
The skill bank in \textsc{HExA} has three orthogonal axes of instantiation (Algorithm~\ref{alg}): how it is \emph{initialized} before experimentation, how it is \emph{updated} between rounds and if we use interaction reward labels with the skills. We test three initializations---\emph{Offline}, \emph{Offline-to-Online} (\emph{Off2On}), and \emph{Online}. Both Offline and Off2On warm-start the bank from $N_0$ base-actor trajectories collected with no skill context, distilled into a fixed skill bank $\mathcal{K}_0=\textsc{Evolver}(\emptyset,\mathcal{T}_0)$; Offline then freezes the bank, whereas Off2On keeps updating it after new experiments. Online instead starts empty ($\mathcal{K}_0=\emptyset$) and bootstraps skills purely from the agent's own interactions. For updates, we use two strategies---\emph{Evolving} and \emph{Iterative Replacement}. In Evolving, we pass the evolver both the current bank and the new rounds trajectories, adding, merging, revising, or pruning skills in light of these new evidence ($\mathcal{K}_n=\textsc{Evolver}(\mathcal{K}_{n-1},\mathcal{T}^{(n)})$). \emph{Iterative Replacement} instead rebuilds the bank from the current rollouts alone ($\mathcal{K}_n=\textsc{Evolver}(\emptyset,\mathcal{T}^{(n)})$), since in the in-context RL loop the actor has already ingested prior skills, so the new skills carry their influence plus the novelty of the latest rollouts. We thus have five variants of skill bank initialization and update---\textit{Off2On} or \textit{Online} initialization $\times$ \textit{Evolution} or \textit{Iterative Replacement} update---plus the frozen Offline bank ($\mathcal{K}_n=\mathcal{K}_{n-1}$). We ablate these settings in Table~\ref{tab:variants_compact} and \emph{Off2On~+~Evolution} performs the best. 

HExA is also flexible to effectively ingest and use additional experimental evidence and data like trajectory rewards which are a function of outcome reward and efficiency, as shown in Appendix~\ref{sec:reward}, to further guide skill evolution and retrieval. The skill reward labels $r_k$ are again a function of these individual trajectory rewards that invoked the skill,  
\begin{equation}
\label{eq:weight}
r_k = \operatorname{clamp}\!\left(\frac{\bar{r}_{\mathrm{src}}+1}{2},\,0.1,\,1.0\right),
\end{equation}






\begin{figure}[h]
\centering
\setlength{\tabcolsep}{1.2pt}
\renewcommand{\arraystretch}{0.85}
% --- ReAct row ----------------------------------------------------------
{\footnotesize\itshape \textsc{ReAct} (25 iterations, FAILURE)}\\[1pt]
\begin{tabular}{@{}ccccccc@{}}
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step0.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step30.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step57.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step70.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step91.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step151.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step193.png} \\[-1pt]
  {\scriptsize } & {\scriptsize } & {\scriptsize } &
  {\scriptsize } & {\scriptsize } &
  {\scriptsize } & {\scriptsize } \\
\end{tabular}\\[2pt]
% --- HExA row -----------------------------------------------------------
{\footnotesize\itshape \textsc{HExA} (6 iterations, SUCCESS)}\\[1pt]
\begin{tabular}{@{}ccccccc@{}}
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step0.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step25.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step57.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step74.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step119.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step140.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step172.png} \\[-1pt]
  {\scriptsize } & {\scriptsize } & {\scriptsize } &
  {\scriptsize } & {\scriptsize } &
  {\scriptsize } & {\scriptsize } \\
\end{tabular}
\caption{%
\textbf{How the evolved skill bank of HExA guides the agent to solve \texttt{catapult}.}
Top: \textsc{ReAct}, which has no cross-episode memory, exhausts its
25-iteration budget while repeatedly exploring ineffective placements.
Bottom: \textsc{HExA} begins with the evolved bank summarized above. After
observing that its initial launch strikes the ceiling, it applies the bank's
diagnosis that the limiting factor is launch geometry rather than insufficient
force. It therefore shifts the drop point toward $x=0.3$ instead of further
increasing the radius, and succeeds with
$(x,y,r)=(0.3,0.9,1.5)$ in six interaction iterations. Frames are sampled from
the final simulations; full prompts, bank entries, and trajectories are
provided in Appendix~\ref{app:trajectories:bank}.}
\label{fig:catapult45_simframes}
\end{figure}








where $\bar{r}_{\mathrm{src}}$ is the mean reward of the source trajectories. Depending on experimental settings, users can define any trajectory reward and skill reward; HExA as a framework is agnostic of these choices. We also tried skill evolution without rewards, using the evolver LLM's prior knowledge itself to guide skill bank update, ignoring the useful environment grounded rewards. Our ablations in Table~\ref{tab:reward_ablation} show that reward labeled skill banks perform the best. Thus, our default experimental setting for \textsc{HExA} is Off2On~+~Evolution with reward labeled skills.








\begin{figure}[t]
\centering
\begin{minipage}[c]{0.56\linewidth}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{lccr}
  \toprule
  \textbf{Method} & \textbf{Acc.\ (\%)} & \textbf{Avg Iter} & \textbf{Tok./ep.} \\
  \midrule
  \multicolumn{4}{l}{\emph{No persistent memory}}\\
  \textsc{Claude}               & \phantom{0}0.0& \phantom{0}1.0          & 0 \\
  \textsc{ReAct}                & \phantom{0}$11.0{\pm}3.0$           &$23.1{\pm}0.2$                    & 0 \\
  Reflexion ($K{=}2$)           &$21.3{\pm}2.5$           & $21.2{\pm}0.7$          & \phantom{0}\phantom{,}287 \\
  \midrule
  \multicolumn{4}{l}{\emph{External memory}}\\
  MemRL          & $33.3{\pm}7.8$                     & $20.4{\pm}3.1$                    & 8{,}135 \\
  Episodic RAG                  & $60.8{\pm}8.9$                     & $14.9{\pm}2.8$                    & 6{,}706 \\
  \midrule
  \multicolumn{4}{l}{\emph{\textsc{HExA}}}\\
  \textsc{HExA} (no reward)     & $50.7{\pm}9.4$           & $16.5{\pm}2.7$          & 2{,}082 \\
  \textsc{HExA} (frozen bank)   & $\mathbf{82.7{\pm}11.4}$ & $\mathbf{12.5{\pm}0.9}$ & \textbf{2{,}392} \\
  \bottomrule
  \end{tabular}
\end{minipage}\hfill
\begin{minipage}[c]{0.42\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/catapult_three_methods_50seeds.pdf}
\end{minipage}
\caption{%
  \textbf{Reward-guided skill accumulation makes \textsc{HExA} much stronger on
  \texttt{catapult}, the hardest level.}
  This experiment tests whether an agent can improve by turning past attempts
  into reusable, reward-guided skills, and how that compares to simply carrying
  the past experience itself forward. On \texttt{catapult}, Claude Sonnet solves
  only $8.0\%$ of seeds with a standard \textsc{ReAct} loop, while \textsc{HExA}
  reaches $82.7\%$ with its bank frozen, using fewer iterations per solve.
  \textbf{Left:} solve rate, average iterations, and the memory block injected
  into the actor's prompt each episode (\emph{Tok./ep.}). The external memory
  methods store past experience directly---Episodic RAG retrieves rollouts
  verbatim, MemRL keeps (intent, experience, utility) triplets---and both are
  beaten by the distilled bank at roughly $3\times$ their context cost, which
  stays constant because the bank is fixed at 10 skills and 5 mistakes.
  \textbf{Right:} cumulative success over $50$ seeds; curves show mean over
  $3$ runs with shaded $\pm 1$ std.
  Removing the reward signal drops \textsc{HExA} to $50.7\%$, and Reflexion reaches
  only $21.3\%$, showing that the main gain comes from scoring and reusing skills,
  not merely from extra interaction or verbal self-reflection.
  Full protocol in Appendix~\ref{app:baselines}.
}
\label{tab:catapult_skillrl}
\label{fig:catapult_three_methods_50seeds}
\end{figure}






\subsection{Results, Analysis, and Ablations}

% =====================================================================
% PREVIOUS VERSION (question-by-question, Q1--Q7) --- kept for reference.
% The float environments (figures/tables) that were interleaved here have
% been pulled out below and are kept ACTIVE; only the prose is commented.
% =====================================================================
% We organize our analysis around seven questions about \textsc{HExA}'s efficacy and generality in
% learning-by-experimentation settings, comparing it to base models and agent-side baselines. We ask
% whether converting interaction into an evolving skill bank lets a frontier agent solve levels that
% single-episode agents cannot (\textbf{Q1}) and whether any gain reflects more efficient search
% rather than additional attempts (\textbf{Q2}); whether the benefit extends to smaller open-weight
% models (\textbf{Q3}); which design ingredients---reward guidance, cross-episode evolution, or
% initialization---drive the improvement (\textbf{Q4}); whether the distilled skills are hierarchical
% and build on one another across rounds (\textbf{Q5}); whether they transfer to unseen levels
% (\textbf{Q6}); and whether in-context skill learning is more sample-efficient than gradient-based RL
% at a matched interaction budget (\textbf{Q7}). Unless noted otherwise, all methods on a level are
% evaluated on the same seeds under an identical $25$-iteration \textsc{ReAct} harness, and
% \textsc{HExA} uses its default Off2On Evolving configuration ($x{=}3$ seeds per round).
%
% \paragraph{Q1: Can distilling interaction into an evolving skill bank solve hard levels that defeat single-episode agents?}
% On the two Tier-2 levels---\texttt{catapult} ($8\%$ \textsc{ReAct}) and \texttt{pass\_the\_parcel}
% ($24\%$ \textsc{ReAct})---a frontier model fails under a single \textsc{ReAct} trajectory, so we
% hypothesize that turning interaction traces into an evolving skill bank should yield substantially
% higher solve rates than agent-side baselines that accumulate no reusable skills (\textsc{Direct},
% \textsc{ReAct}, Reflexion). We test this with Claude Sonnet, running every method on the same $50$
% seeds per level; \textsc{HExA} and Reflexion are repeated over $3$ independent runs
% (mean~$\pm$~std), while \textsc{Direct} and \textsc{ReAct} are deterministic single runs.
% \textsc{HExA} turns both levels from mostly-unsolved one-episode problems into substantially
% solvable in-context learning tasks. On \texttt{catapult} it reaches $67.3 \pm 9.3\%$, against
% $2.0\%$ (\textsc{Direct}), $8.0\%$ (\textsc{ReAct}), and $21.3 \pm 2.5\%$ (Reflexion)
% (Table~\ref{tab:catapult_skillrl}); on \texttt{pass\_the\_parcel} it reaches $60.0\%$, against
% $24.0\%$ (\textsc{ReAct}), $16.0\%$ (Reflexion), and $0.0\%$ (\textsc{Direct})
% (Table~\ref{tab:ptp_variants}). Because \texttt{pass\_the\_parcel} requires discovering the
% ramp-and-basket mechanism rather than a direct collision, the gain indicates that distilling past
% interactions into reusable strategies---not merely retrying---is what makes the level solvable.
% Figure~\ref{fig:catapult45_simframes} shows a representative \texttt{catapult} seed where
% \textsc{HExA} solves the task in a handful of iterations by reusing previously distilled placement
% heuristics, while \textsc{ReAct} exhausts its budget without finding a working launch.
%
% \paragraph{Q2: Is \textsc{HExA}'s advantage more efficient search, or just more attempts?}
% A higher solve rate alone could arise from spending more interaction per seed or from occasional
% lucky placements, rather than from genuinely easier episodes. We therefore record, on the same runs
% as Q1, the average number of \textsc{ReAct} iterations per seed as an efficiency proxy, and track
% the cumulative success and cumulative iteration curves across the seed sweep. \textsc{HExA} lowers
% the average iterations from $22.9$ (\textsc{ReAct}) and $21.2 \pm 0.7$ (Reflexion) to
% $14.4 \pm 1.8$, roughly $37\%$ fewer, so each episode becomes genuinely easier rather than merely
% more numerous (Figure~\ref{fig:catapult_three_methods_50seeds}). The cumulative curves stay
% separated throughout the sweep---\textsc{HExA}'s success curve remains above the baselines while its
% iteration curve converges below them (Figures~\ref{fig:catapult_three_methods_50seeds}
% and~\ref{fig:cum_iter_both})---so the ranking is not an artifact of a few lucky seeds, and the extra
% accuracy comes with less, not more, computation per instance; the same per-seed efficiency pattern
% holds on \texttt{pass\_the\_parcel}. Reflexion, which adds verbal self-reflection but keeps no
% persistent bank, trails \textsc{HExA} by $46$~percentage points (pp) on \texttt{catapult} and
% $29$~pp even after the reward signal is removed, evidence that the gain comes from reusing distilled
% skills rather than from extra trials or in-context verbalization alone.
%
% \paragraph{Q3: Does the benefit extend to smaller open-weight models, not just a frontier solver?}
% If \textsc{HExA}'s gains depended on a frontier model's reasoning, they would not appear with weaker
% actors. We therefore run the same skill-injection loop on open-weight solvers---Qwen-2.5-\{3B,7B\}
% and GPT-OSS-120B---against a matched baseline that is the identical agent with no skill injection
% (Qwen runs use Online Evolving with $k{=}3$ seeds per round; GPT-OSS-120B uses Off2On Evolving).
% Across every level and model, \textsc{HExA} improves over its baseline
% (Table~\ref{tab:hexa_smallmodels_main_paper}): on \texttt{down\_to\_earth}, Qwen-2.5-3B rises
% $8.0\to24.0\%$ and Qwen-2.5-7B $62.0\to72.0\%$; on \texttt{two\_body\_problem}, $6.0\to14.0\%$ and
% $18.0\to34.0\%$; and on \texttt{catapult}, GPT-OSS-120B rises from $0.0\%$ to $54.0\%$. Gains range
% from $+8$ to $+54$~pp, so the mechanism is not specific to a frontier model. Per-seed cumulative
% trajectories and the full sweep are in Figure~\ref{fig:hexa_smallmodels} and Appendix~\ref{sec:h2}.
%
% \paragraph{Q4: Which ingredients drive the improvement---reward guidance, cross-episode evolution, or initialization?}
% Given the configuration axes defined in Section~\ref{sec:setup} (initialization: Offline / Off2On /
% Online; update: Evolving / Iterative Replacement), we now isolate which ingredients are responsible
% for \textsc{HExA}'s gains. We probe three candidate drivers in turn: the reward signal supplied to
% the evolver, evolving the bank across rounds versus rebuilding it each round, and warm-starting the
% bank versus starting cold.
% \emph{Reward guidance.} We first ablate the reward signal in the evolver so that every success and
% failure is treated identically, regardless of how efficiently it was reached. (The reward enters as
% a priority label the evolver acts on when retaining or pruning skills, not as a numeric weight in a
% learned sum.) On Qwen-2.5-7B this calibration accounts for most of the gain: on
% \texttt{down\_to\_earth} the unguided variant reaches only $64\%$ ($+2$~pp over \textsc{ReAct})
% versus $72\%$ for full \textsc{HExA} ($+10$~pp), and on \texttt{two\_body\_problem} it reaches $26\%$
% versus $34\%$ (Table~\ref{tab:reward_ablation}). The same effect appears with a frontier solver: on
% \texttt{catapult}, removing the reward signal lowers Claude Sonnet from $67.3 \pm 9.3\%$ to
% $50.7 \pm 9.4\%$ (Figure~\ref{fig:catapult_three_methods_50seeds}). Reward calibration thus lets the
% evolver separate efficiently-solved trajectories from merely-successful ones, so the skills it keeps
% and refines are the more reusable ones.
% \emph{Cross-episode evolution.} We next sweep the update rule with initialization held fixed.
% Evolving the bank across rounds consistently beats distilling it once: on \texttt{pass\_the\_parcel}
% the evolving variants reach $58$--$60\%$ versus $48\%$ for a frozen offline bank and $24\%$ for
% \textsc{ReAct} (Table~\ref{tab:ptp_variants}), and on \texttt{catapult} Off2On Evolving reaches
% $76\%$ versus $56\%$ and $36\%$ for the two iterative variants and $60\%$ for the frozen offline bank
% (Table~\ref{tab:variants_compact}; full per-configuration breakdown in Appendix
% Table~\ref{tab:catapult_variants}). The cumulative-accuracy curves on both levels
% (Figure~\ref{fig:cum_accuracy_both}) make the mechanism visible: the evolving variants pull steadily
% away from the others as each round adds evidence, instead of plateauing like a one-shot
% distillation, because re-distilling from scratch discards accumulated skills and amplifies drift.
% \emph{Initialization.} Holding the update rule at Evolving, the warm start helps but matters less:
% Off2On reaches $76\%/60\%$ on \texttt{catapult}/\texttt{pass\_the\_parcel} versus $44\%/58\%$ for a
% cold Online start, with the gap sharpest on \texttt{catapult} because a cold start spends its early
% rounds rediscovering basic strategies from a few correlated trajectories, an advantage that shrinks
% once online evolution takes over. Combining a broad offline prior with cumulative refinement,
% \emph{Off2On Evolving} is best on both levels and is the configuration we refer to as \textsc{HExA}
% throughout.
%
% \paragraph{Q5: Does \textsc{HExA} learn hierarchical skills that build on one another across rounds?}
% A central claim is that \textsc{HExA} accumulates not only per-seed recipes but skills that compose
% into increasingly abstract principles. Because each round's trajectories are generated while the
% actor is already conditioned on the previous round's retrieved skills, a new skill can refine,
% bound, merge with, or overturn an earlier one---so we ask whether the evolved bank shows such
% layering rather than a flat list of placements. We examine this qualitatively through the evolved
% \texttt{catapult} bank (Appendix~\ref{app:trajectories:bank}). Within a round, the evolver abstracts
% trajectory-level evidence into general principles: experiments at $x{=}0.5$ showed that $r{=}1.0$
% fell short, $r{=}1.5$ struck the ceiling, and intermediate radii $r\in[1.1,1.4]$ did not resolve the
% tradeoff; rather than store these as separate parameter prescriptions, the evolver inferred that
% ceiling clearance is governed by launch angle and contact geometry, not impact energy alone, and
% consolidated them into a higher-level rule---when radius tuning at fixed $x$ alternates between
% insufficient range and ceiling collisions, stop interpolating $r$ and shift $x$ toward $0.1$--$0.3$
% to flatten the launch arc. This compresses many $(x,y,r)$ trials into both a reusable physical
% principle and a policy for \emph{when to abandon local parameter search}. The hierarchy also
% develops across rounds: the seed-45 solve in Figure~\ref{fig:catapult45_simframes} applies exactly
% this layered structure---a learned default launch, a diagnosed ceiling failure, and the corrective
% geometry shift---to succeed in six iterations. We read these as evidence of compositional,
% hierarchical skill formation rather than proof, and provide the full bank and trajectories in
% Appendix~\ref{app:trajectories:bank}.
%
% \paragraph{Q6: Are the learned skills reusable on unseen levels?}
% If \textsc{HExA} distills genuinely reusable physics primitives rather than level-specific recipes,
% skills from source levels should help on an unseen target with no target-level experience. We test
% this by synthesising a target bank from source-level banks plus a textual description of the target
% alone---no target-level trajectories are generated at any stage---and injecting it with no further
% evolution. Combining fully-evolved banks from three source levels (\texttt{down\_to\_earth},
% \texttt{two\_body\_problem}, \texttt{pass\_the\_parcel}), the evolver synthesises a \texttt{catapult}
% bank that raises Claude Sonnet from $8.0\%$ to $44.0\%$ ($+36$~pp), closing roughly $60\%$ of the
% gap to the within-level \textsc{HExA} result of $64\%$ (Table~\ref{tab:cross_level},
% Figure~\ref{fig:cross_level_transfer}); this is consistent with \texttt{catapult}'s lever-launch
% dynamics sharing structural primitives (collision normals, energy thresholds, directional impulse)
% with the source levels. Transfer also helps with a single source bank and a smaller teacher:
% on a structurally similar pair (\texttt{down\_to\_earth}~$\to$~\texttt{falling\_into\_place}) it
% gains $+12$~pp, and on a dissimilar pair (\texttt{down\_to\_earth}~$\to$~\texttt{two\_body\_problem})
% it still gains $+16$~pp (Table~\ref{tab:cross_level}). That transfer succeeds even across dissimilar
% levels suggests the evolver extracts abstract principles---momentum transfer, contact
% geometry---rather than narrow placement heuristics.
%
% \paragraph{Q7: At a matched interaction budget, is in-context \textsc{HExA} more sample-efficient than gradient-based RL?}
% Finally we ask whether in-context skill evolution is more sample-efficient than updating model
% weights from the same experience. We compare against GRPO~\citep{shao2024deepseekmath} fine-tuning
% Qwen-2.5-3B on the same levels, matched on the number of model updates and on $50$ unique
% environment seeds. At this budget GRPO reaches $20\%$ on \texttt{down\_to\_earth} and $6\%$ on
% \texttt{two\_body\_problem}, versus \textsc{HExA}'s $24\%$ and $14\%$
% (Figure~\ref{fig:grpo_comparison_main}). The gap reflects the core advantage of in-context skill
% evolution: strategies distilled from early trajectories are immediately available to later episodes
% through context, whereas gradient-based methods must accumulate signal over many rollouts before the
% weights encode equivalent knowledge---so in harder domains where early successes are rare,
% \textsc{HExA} can still bootstrap learning from failure and partial-success trajectories. With many
% more updates, GRPO can eventually close the gap through direct optimization on the environment
% reward. We present more details of these ablations in Appendix~\ref{sec:h5}.
% =====================================================================
% END PREVIOUS VERSION
% =====================================================================







\begin{table}[t]
\centering
\small
\caption{%
  \textsc{HExA} on open-weight solvers, 50 training/evaluation seeds per cell
  (max 25 iterations). Qwen-2.5 runs use the Online-Evolving configuration ($k{=}3$ seeds
  per round, 17 rounds); GPT-OSS-120B uses Off2On Evolving. Baselines are the same agent with
  no skill injection. Per-seed cumulative trajectories in Figure~\ref{fig:hexa_smallmodels}.
}
\label{tab:hexa_smallmodels_main_paper}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{llcc}
\toprule
\textbf{Level} & \textbf{Method} & \textbf{Acc.\ (\%)} & \textbf{Avg Iters} \\
\midrule
\multirow{4}{*}{Down to Earth}
  & Qwen-2.5-3B \textsc{ReAct} & \phantom{0}8.0 & 23.8 \\
  & Qwen-2.5-3B \textsc{HExA}  & \textbf{24.0}  & 18.6 \\
  \cmidrule(lr){2-4}
  & Qwen-2.5-7B \textsc{ReAct} & 62.0           & 12.5 \\
  & Qwen-2.5-7B \textsc{HExA}  & \textbf{72.0}  & 12.6 \\
\midrule
\multirow{4}{*}{Two Body Problem}
  & Qwen-2.5-3B \textsc{ReAct} & \phantom{0}6.0 & 24.0 \\
  & Qwen-2.5-3B \textsc{HExA}  & \textbf{14.0}  & 21.1 \\
  \cmidrule(lr){2-4}
  & Qwen-2.5-7B \textsc{ReAct} & 18.0           & 22.2 \\
  & Qwen-2.5-7B \textsc{HExA}  & \textbf{34.0}  & 18.9 \\
\midrule
\multirow{2}{*}{Catapult}
  & GPT-OSS-120B \textsc{ReAct} & \phantom{0}0.0 & 25.0 \\
  & GPT-OSS-120B \textsc{HExA}  & \textbf{54.0}  & 16.2 \\
\bottomrule
\end{tabular}
\end{table}







\paragraph{Does active experimentation and skill creation help agents solve complex tasks?}
On levels where a single \textsc{ReAct} trajectory fails, we hypothesize that distilling interaction traces into an evolving skill bank should raise solve rates over base model and non-experimental agent baselines that accumulate
no reusable skills (\textsc{Direct}, \textsc{ReAct}, Reflexion). We test this with frontier model Claude Sonnet, as well as open-weight models like Qwen-2.5-3B and 7B and GPT-OSS-120B against the same non-experimental baselines. On the harder levels where even the base Clause Sonnet model could barely make progress, \textsc{HExA} learns consistently via in-context experimentation: on \texttt{catapult} it reaches
$82.7 \pm 11.4\%$ against $2.0\%$ (\textsc{Direct}), $8.0\%$ (\textsc{ReAct}), and $21.3 \pm 2.5\%$
(Reflexion) (Figure~\ref{fig:catapult_three_methods_50seeds} and Table~\ref{tab:catapult_skillrl}), and on \texttt{pass\_the\_parcel}---which requires
discovering the ramp-and-basket mechanism rather than a direct collision---it reaches $60.0\%$
against $24.0\%$, $16.0\%$, and $0.0\%$ respectively (Table~\ref{tab:ptp_variants}). In
Figure~\ref{fig:catapult45_simframes} we show a representative \texttt{catapult} seed solved in a
handful of iterations by reusing distilled placement skills while \textsc{ReAct} exhausts its
budget. The same pattern holds for weaker open models: \textsc{HExA} improves every open-weight model we tested on every level (Table~\ref{tab:hexa_smallmodels_main_paper}), raising Qwen-2.5-3B from $8.0\to24.0\%$
and Qwen-2.5-7B from $62.0\to72.0\%$ on \texttt{down\_to\_earth}, $6.0\to14.0\%$ and $18.0\to34.0\%$
on \texttt{two\_body\_problem}, and GPT-OSS-120B from $0.0\to54.0\%$ on \texttt{catapult}. The improvement therefore comes from distilling past
interactions into reusable strategies rather than from extra retries, and also helps solve the tasks more efficiently and in lesser number of turns (full sweep in Figure~\ref{fig:hexa_smallmodels} and Appendix~\ref{sec:h2}).

\paragraph{Does a distilled skill bank beat storing the experience itself?}
The baselines above keep no memory at all, so they leave open whether the gain
comes from \emph{distillation} or merely from having past experience available
in context. We therefore compare \textsc{HExA} against two external memory
methods on \texttt{catapult} with the same Claude Sonnet~4.6 actor: Episodic
RAG, which retrieves past rollouts verbatim, and MemRL, which maintains
(intent, experience, utility) triplets. Every arm's memory is \emph{frozen}
after it is built---no further distillation or updating---and scored on the
same held-out pool of $50$ seeds, so each method is judged on reuse rather than
on refitting to the instances it is scored on, and the comparison is paired on
identical instances. Under this protocol \textsc{HExA} reaches
$82.7 \pm 11.4\%$ against $60.8\%$ for Episodic RAG and $33.3\%$ for MemRL
(Table~\ref{tab:catapult_skillrl}). The separation is sharper in context
cost: \textsc{HExA} injects $2{,}392$ tokens per episode against $6{,}706$ and
$8{,}135$, and because the bank is fixed at 10 skills and 5 mistakes, that cost
does not grow as more episodes are played. The episodic methods inject whole
rollouts, so their context scales with the rollout cap rather than with
anything learned. Distilling interaction into compact, reusable skills is thus
both more effective and roughly $3\times$ cheaper in context than carrying the
raw experience forward.











\begin{figure}[h]
  \centering
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/catapult_var_cum_avg_iter.pdf}
    \subcaption{Catapult}
    \label{fig:catapult_var_cum_iter}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/ptp_cum_avg_iter.pdf}
    \subcaption{Pass the Parcel}
    \label{fig:ptp_cum_iter}
  \end{minipage}
  \caption{%
    \textbf{Cumulative average turns per seed} for every \textsc{HExA}
    variant against the baseline (Claude Sonnet); lower is more efficient. On both levels the
    Off2On Evolving configuration converges to the lowest cost per seed, while the iterative and
    pure-online variants remain higher, indicating that \textsc{HExA}'s gains come from guiding
    search more efficiently with accumulated experience rather than from spending more
    computation per instance.
  }
  \label{fig:cum_iter_both_main}
\end{figure}









\paragraph{Can \textsc{HExA} leverage learned skills for more efficient exploration and experimentation?} In our task settings, simply spending more compute on interactions does not ensure higher task success. The agents benefits from active skill acquisition and reuse~\citep{a-skills-1}, helping it with more successes as well as doing so efficiently. These compact skills in turn makes learning more efficient in these complex tasks with lesser interactions. We record the average number of iterations or turns per seed as an efficiency proxy, and track the cumulative success and cumulative iteration curves across our experiments. \textsc{HExA} lowers
the average iterations from $22.9$ (\textsc{ReAct}) and $21.2 \pm 0.7$ (Reflexion) to
$12.5 \pm 0.9$, roughly $45\%$ fewer, so each future episode becomes easier to tackle using the accumulated skills (Figure~\ref{fig:catapult_three_methods_50seeds} and Figure~\ref{fig:cum_iter_both_main}). So the get much more gains in accuracy from HExA at equivalent inference compute. Similar efficiency gains also hold on \texttt{pass\_the\_parcel}. Reflexion, which adds verbal self-reflection but keeps no persistent skill bank to retrieve and reuse from, takes more trails than \textsc{HExA}. Thus self-reflection between trials help far less than converting past experiences into an explicit, reusable skill bank, and this holds even when the reward labels are removed from the bank. The evolving skill bank in HExA thus helps with structured exploration and amortizes the cost of future experimentation, helping both improve performance and efficiency.


% even when the reward signal is removed, evidence that the gain comes from reusing distilled skills rather than from extra trials or in-context verbalization alone.







\paragraph{Which ingredients drive improvements in HExA?}
Using the instantiation axes defined in Section~\ref{sec:instantiation}, we study how these aid learning from experimentation. 

\emph{How do reward labels help learning via experimentation?} We try using HExA with and without the reward labels in the skill bank. In our ablations without the reward labels, every success and failure trajectory and skills formed out of them are treated equally and the LLM evolver implicitly updates the skill bank using its existing knowledge. On Qwen-2.5-7B the unguided reward-free skill variant reaches $64\%$ versus $72\%$ with rewards
on \texttt{down\_to\_earth} and $26\%$ versus $34\%$ on \texttt{two\_body\_problem}
(Table~\ref{tab:reward_ablation_main}). On \texttt{catapult} it drops Claude Sonnet from $67.3 \pm 9.3\%$ to $50.7 \pm 9.4\%$ (Figure~\ref{fig:catapult_three_methods_50seeds}). Thus the reward labels provide valuable environment feedback grounded in actual explorations and interactions of the LLM actor that better helps assign credit for effective and efficient skill acquisition as well as better guide the LLM evolver to compose, retain or prune skills.



\begin{table}[h]
\centering

\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{3pt}
\caption{%
  Reward-signal ablation on Qwen-2.5-7B, 50 seeds per cell.
  Full \textsc{HExA} uses reward-guided, two-pass distillation;
  the no-reward variant treats successful trajectories equally.
}
\label{tab:reward_ablation_main}
\begin{tabular*}{\linewidth}{@{}l l @{\extracolsep{\fill}} c c@{}}
\toprule
\textbf{Level} & \textbf{Method}
  & \textbf{Acc.\ (\%)}
  & \textbf{Iters} \\
\midrule
\multirow{3}{*}{Down to Earth}
  & \textsc{ReAct}              & 62.0          & 12.5 \\
  & \textsc{HExA} no reward     & 64.0          & 14.8 \\
  & \textsc{HExA} reward        & \textbf{72.0} & 12.6 \\
\midrule
\multirow{3}{*}{Two Body}
  & \textsc{ReAct}              & 18.0          & 22.2 \\
  & \textsc{HExA} no reward     & 26.0          & 22.2 \\
  & \textsc{HExA} reward        & \textbf{34.0} & 18.9 \\
\bottomrule
\end{tabular*}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{3pt}
\caption{%
  \textsc{HExA} variant accuracy (\%) on the two hard levels
  Claude Sonnet; \textbf{Cat.}~=~\texttt{catapult};
  \textbf{PtP}~=~\texttt{pass\_the\_parcel}.
  Off2On Evolving ($x{=}3$), referred to simply as \textsc{HExA},
  is best on both.
}
\label{tab:variants_compact}
\begin{tabular*}{\linewidth}{@{}l @{\extracolsep{\fill}} c c@{}}
\toprule
\textbf{Configuration} & \textbf{Catapult} & \textbf{Pass the Parcel} \\
\midrule
Off2On Evolving (HExA) & \textbf{76.0} & \textbf{60.0} \\
Off2On Iterative       & 56.0          & 48.0          \\
Online Evolving        & 44.0          & 58.0          \\
Online Iterative       & 36.0          & 56.0          \\
Offline Static         & 60.0          & 48.0          \\
\bottomrule
\end{tabular*}
\end{minipage}

\end{table}



% \begin{table}[h]
% \centering

% \begin{minipage}[t]{0.48\linewidth}
% \vspace{0pt}
% \centering
% \scriptsize
% \caption{%
%   Reward-signal ablation on Qwen-2.5-7B, 50 seeds per cell.
%   Full \textsc{HExA} uses reward-guided, two-pass distillation;
%   the no-reward variant treats successful trajectories equally.
% }
% \label{tab:reward_ablation_main}
% \begin{tabular}{@{}llcc@{}}
% \toprule
% \textbf{Level} & \textbf{Method}
%   & \textbf{Acc.\ (\%)}
%   & \textbf{Iters} \\
% \midrule
% \multirow{3}{*}{Down to Earth}
%   & \textsc{ReAct}              & 62.0          & 12.5 \\
%   & \textsc{HExA} no reward     & 64.0          & 14.8 \\
%   & \textsc{HExA} reward        & \textbf{72.0} & 12.6 \\
% \midrule
% \multirow{3}{*}{Two Body}
%   & \textsc{ReAct}              & 18.0          & 22.2 \\
%   & \textsc{HExA} no reward     & 26.0          & 22.2 \\
%   & \textsc{HExA} reward        & \textbf{34.0} & 18.9 \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.48\linewidth}
% \vspace{0pt}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \caption{%
%   \textsc{HExA} variant accuracy (\%) on the two hard levels
%   Claude Sonnet; \textbf{Cat.}~=~\texttt{catapult};
%   \textbf{PtP}~=~\texttt{pass\_the\_parcel}.
%   Off2On Evolving ($x{=}3$), referred to simply as \textsc{HExA},
%   is best on both.
% }
% \label{tab:variants_compact}
% \begin{tabular}{@{}lcc@{}}
% \toprule
% \textbf{Configuration} & \textbf{Cat.} & \textbf{PtP} \\
% \midrule
% Off2On Evolving (HExA) & \textbf{76.0} & \textbf{60.0} \\
% Off2On Iterative       & 56.0          & 48.0          \\
% Online Evolving        & 44.0          & 58.0          \\
% Online Iterative       & 36.0          & 56.0          \\
% Offline Static         & 60.0          & 48.0          \\
% \bottomrule
% \end{tabular}
% \end{minipage}

% \end{table}










\emph{Does skill bank initialization matter?} With the update rule fixed, a skill bank initialized with some initial offline bank helps warm-start learning faster, but matters less as more rounds of interaction happens (Section \ref{sec:instantiation}). As we can see in Table \ref{tab:variants_compact}, Off2On reaches $76\%$ and $60\%$ on \texttt{catapult} and \texttt{pass\_the\_parcel} versus $44\%$ and $58\%$ for a pure Online start. The gap on \texttt{catapult} happens where a cold start wastes early rounds rediscovering basic dynamics of the level, an advantage that shrinks once enough enough online experimentation has been done.









\emph{What helps skill update more, evolving over the existing bank or rebuilding from scratch?} We ablate over the two skill update variants, Evolving and Iterative Replacement (Section \ref{sec:instantiation}) with the same initialization. Evolving the previous skill bank with new experimentation trajectories across seeds, beats Iterative Replacement where we rebuild the skill bank from scratch every time with new trajectories from the updated LLM actor. On \texttt{pass\_the\_parcel} the evolving variants reaches $60\%$ accuracy on solving the level
versus $48\%$ for skill update from scratch (Table~\ref{tab:variants_compact}). Similarly on \texttt{catapult} Evolving skill update helps achieve $76\%$ versus $56\%$ for the iterative variant (Table~\ref{tab:variants_compact}). We also show the cumulative-accuracy curves for these ablations in (Appendix figure~\ref{fig:cum_accuracy_both}). We can thus see how gradually evolving the existing skill banks with evidence from new experimentation rounds helps build better skill bank, since re-distilling from scratch discards accumulated skills and amplifies overfitting. A key risk in any iterative skill-update loop is skill overfitting, the skill bank may accumulate increasingly narrow strategies that overfit to the particular instances seen so far, while discarding general principles that would transfer to new instances. Thus the Evolving update strategy works better, because trajectories in round $n$ are generated while conditioned on $\mathcal{G}_n=\textsc{Retriever}(\mathcal{K}_{n-1},\ell,M,N)$, they explicitly reflect the influence of previously learned skills. The evolutionary update $\mathcal{K}_n= \pi_{\mathrm{ev}}(\mathcal{K}_{n-1},\mathcal{T}^{(n)})$ can
therefore refine an earlier rule, identify its boundary conditions, merge it with corroborating evidence, or replace it when contradicted by subsequent experience.












\paragraph{Does \textsc{HExA} learn hierarchical skills that build on one another, and do those skills transfer to unseen levels?} \textsc{HExA} accumulates skills that compose into increasingly abstract principles, because each round's trajectories are generated while the actor is conditioned
on previously retrieved skills, letting a new skill refine, bound, merge with, or overturn an earlier one. 
\begin{wrapfigure}[15]{l}{0.60\linewidth}
  \vspace{-1pt}
  \centering
  \includegraphics[width=\linewidth]{figures/cross_level_transfer_main.pdf}
  \caption{%
    Cross-level skill transfer with no target trajectories. Each target is solved using only skills synthesized from source-level banks; labels report target success and matched \textsc{ReAct} baselines. Multi-source transfer to \texttt{catapult} yields the largest gain
    ($+36$~pp).
  }
  \label{fig:cross_level_transfer_main}
  \vspace{-12pt}
\end{wrapfigure}
Qualitatively, the evolved \texttt{catapult} bank shows this hierarchical nature
(Appendix~\ref{app:trajectories:bank}): experiments at $x{=}0.5$ where $r{=}1.0$ fell short and
$r{=}1.5$ struck the ceiling are not stored as separate parameter settings but consolidated into a
higher-level rule---"when radius tuning at fixed $x$ alternates between falling short and hitting the
ceiling, stop tuning $r$ and shift $x$ toward $0.1$--$0.3$ to flatten the launch arc"---compressing the
many $(x,y,r)$ trials into a physical principle plus a policy for when to abandon local search. The example in Figure~\ref{fig:catapult45_simframes} applies exactly these hierarchical skills (default launch $\to$ diagnosed ceiling failure $\to$ corrective geometry shift) to succeed in just six
iterations. If the skill banks encode not only level-specific recipes but also abstract principles, those principles should transfer to unseen levels and help experimentation there as well. So we test transfer by synthesizing a target skill bank from easier level banks plus only a textual description of the unseen harder target. No target-level trajectories are used at any stage---and injecting it with no further evolution. Combining evolved banks from three source
levels (\texttt{down\_to\_earth}, \texttt{two\_body\_problem}, \texttt{pass\_the\_parcel}) helps improve
Claude Sonnet on \texttt{catapult} from $2.0\%$ solve rate with the base model and $8.0\%$ with active level interaction via REACT to $44.0\%$ with HExA on the transferred skill bank(Figure~\ref{fig:cross_level_transfer_main} and Table~\ref{tab:cross_level}). Transfer also helps with a single source bank and a smaller actor model like Qwen 7B---transfer on a structurally similar pair (\texttt{down\_to\_earth}~$\to$~\texttt{falling\_into\_place})
leads to gains of $+12\%$ in success rate and the dissimilar pair (\texttt{down\_to\_earth}~$\to$~\texttt{two\_body\_problem})
still gains $+16\%$. These transfers across dissimilar levels without any online interactions in the held-out test levels indicates that the evolver extracts generalizable abstract principles---momentum transfer, contact geometry, directional impulse---rather than narrow level-specific heuristics. Thus \textsc{HExA}'s hierarchical skills and evolution methods help learn and acquire reusable and transferable knowledge that even generalize to unseen complex domains via learning from exploration and experimentation.




\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/grpo_comparison.pdf}

\caption{%
  \textbf{In-context skill evolution learns faster than GRPO at the same interaction budget.}
  We compare \textsc{HExA} with GRPO fine-tuning on Qwen-2.5-3B using 50 training seeds.
  The green star marks \textsc{HExA}'s success rate after the same 50-seed budget
  (Down to Earth: $24\%$, Two Body Problem: $14\%$), while the dashed line marks the
  matched-budget GRPO checkpoint. In this low-data regime, \textsc{HExA} outperforms both
  GRPO variants, suggesting that reusable in-context skills provide faster early adaptation;
  with many more updates, GRPO can eventually close the gap through direct reward optimization.
}
  \label{fig:grpo_comparison_main}
\end{figure}









\paragraph{How does performance of \textsc{HExA} compare to RL finetuning with weight updates?}
Finally we ask how learning via experimentation in-context with skill evolution compares to model training with RL in terms of sample-efficient and performance. We compare against GRPO~\citep{shao2024deepseekmath} fine-tuning
Qwen-2.5-3B on the same levels, matched on the number of model updates and on $50$ unique
environment seeds. At this budget GRPO reaches $20\%$ on \texttt{down\_to\_earth} and $6\%$ on
\texttt{two\_body\_problem}, versus \textsc{HExA}'s $24\%$ and $14\%$
(Figure~\ref{fig:grpo_comparison_main}). The gap reflects the core advantage of in-context skill evolution: strategies distilled from early trajectories are immediately available to later episodes
through context, whereas gradient-based methods must accumulate signal over many rollouts before the
weights encode equivalent knowledge---so in harder domains where early successes are rare,
\textsc{HExA} can still enable experimentation guided learning from failure and partial-success trajectories. With many more updates, GRPO can eventually close the gap through direct optimization on the environment
reward. But combining learning from experimentation in-context to bootstrap initial progress on complex domains with later stages of gradient based RL post-training can be a robust learning method. We present more details of these ablations in Appendix~\ref{sec:h5}.



























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Experiments and Results on Interphyre}
% \label{sec:experiments}

% In this section, we provide details of \textsc{Interphyre}, and evaluate different LLMs on experiment-centric tasks using \textsc{Interphyre} levels. Our benchmark is designed with the following key properties:

% \begin{enumerate}[label=(\roman*)]
%     \item tasks whose solution is unknown or cannot be read off a static description and must be discovered by interacting with the environment.
%     \item a programmatic interface that lets the agent autonomously inspect the scene, test interventions, and observe intermediate dynamics.
%     \item a controllable difficulty range with procedural generation.
% \end{enumerate}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figures/interventions_example.pdf}
%   \caption{\textbf{\textsc{Interphyre}'s snapshot/restore API.} This branches a shared mid-trajectory state into a
%     factual rollout and perturbed alternatives (Section \ref{sec:snapshot-restore}).
%     Each row is one seed of the \texttt{catapult} level with a different oracle solution
%     strategy.
%     The leftmost column shows the initial scene for reference; the teal curve is the
%     green ball's trajectory, shown up to the branch point in the \emph{Branch point}
%     column and continuing through the outcome in each subsequent column.
%     Top (seed\,8, deflector strategy): removing the deflector causes failure; shrinking
%     the red action ball does not.
%     Bottom (seed\,5, direct-launch strategy): shrinking the red ball causes failure;
%     removing the deflector does not.
%     The same interventions have opposite causal relevance across seeds, showing that causal
%     relevance is a property of an object relative to the active strategy, not of the object
%     in isolation.
%     See Section \ref{sec:worked-example} for the branching protocol.}
%   \label{fig:intervention-example_main_paper}
% \end{figure}

% \subsection{\textsc{Interphyre}: A Testbed for Learning through Experimentation}
% \label{sec:Interphyre_example}

% Unlike benchmarks that primarily ask whether an agent can solve a task or answer a query, our setting requires an environment in which the agent can deliberately interact and gather evidence: inspecting the current instance, testing interventions, observing intermediate dynamics, diagnosing failures, and reusing what it learned across future seeds and levels in an experimentation loop. \textsc{Interphyre} provides this in a controlled 2D physics domain with continuous actions and long-horizon causal structure. Each task requires placing a red ball at $(x,y,r)$, after which the simulator evaluates whether the level-specific success predicate is achieved.

% \textsc{Interphyre} builds on the level designs in the PHYRE benchmark \citep{bakhtin2019phyre} by introducing APIs for level editing, test-time interventions on environment parameters, and logging traces from the simulation. These APIs can be used to customize the benchmark for evaluating agents on unseen levels, or provided to an LLM for active experimentation. In particular, our experiments use the \textsc{Interphyre} API to expose a structured tool-calling interface for hypothesis testing via interventional scene inspection, partial simulation, full rollouts, contact logs, and level-specific geometric analysis, for example as shown in Figure \ref{fig:intervention-example_main_paper}. However, successful actions often depend on contact chains, lever mechanics, collision timing, and strategy-dependent dynamics. Even strong LLMs struggle to anticipate such interactions reliably during inference, particularly when only given the scene description.

% The traces recovered from \textsc{Interphyre} runs let us measure precisely whether an LLM agent merely guesses from parametric prior knowledge, or leverages the information provided through interactions and exploration to improve its performance in-context. \textsc{Interphyre} therefore serves as both a benchmark and a diagnostic environment for experimentation based methods such as \textsc{HExA}. We provide full details of the environment design, curriculum, tool API, observation modes, and prompts in Appendix~\ref{app:Interphyre} and \ref{app:systemprompts}.


% \subsection{Experimental Setup, Evaluations, and Baselines}
% \label{sec:setup}

% \setlength{\intextsep}{2pt}          % less vertical space above/below the float
% \setlength{\columnsep}{10pt}         % gap between table and wrapped text

% \begin{wraptable}{r}{0.58\linewidth}
% \vspace{-\baselineskip}              % pull the table up toward the section top (optional)
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{3pt}
% \caption{%
%   \textsc{ReAct} baseline solve rate~(\%) across eight
%   \textsc{Interphyre} levels.
%   Underlined levels (Pass the Parcel, Catapult) form the harder tier,
%   based on Claude Sonnet performance.
%   \textsuperscript{$\dagger$}Evaluated on 50 seeds;
%   \textsuperscript{$\ddagger$}25 seeds;
%   all others 100 seeds.
%   --- = not evaluated.
% }
% \label{tab:baseline_results}
% \begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} cccccc}
% \toprule
% & \textbf{Rand} & \textbf{Q-7B} & \textbf{Q-14B}
% & \textbf{O-20B} & \textbf{O-120B} & \textbf{Son.} \\
% \midrule
% Cliffhanger             & 0  & 2.0  & 6.0  & 30.5 & 64.0 & 100$^{\ddagger}$ \\
% Tipping Point           & 3  & 24.0 & 42.0 & 80.0 & 90.1 & 96$^{\ddagger}$  \\
% Basket Case             & 4  & 8.0  & 10.0 & 14.0 & 33.0 & 100$^{\ddagger}$ \\
% Down to Earth           & 8  & 62.0 & 72.0 & 35.0 & 72.5 & 100             \\
% Two Body                & 14 & 18   & 24.0 & 26.0 & 77.8 & 100             \\
% Falling in Place        & 1  & 20.0 & 52.0 & 58.0 & 100  & 100$^{\dagger}$ \\
% \underline{Pass the Parcel} & 0  & 7.8  & 9.8  & 16   & 22   & 24$^{\dagger}$ \\
% \underline{Catapult}        & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 8$^{\dagger}$  \\
% \bottomrule
% \end{tabular*}
% \end{wraptable}

% We evaluate five LLMs including frontier black box and small open LLMs---Claude Sonnet~4.6, Qwen-2.5-\{7B, 14B\} Instruct, GPT-OSS-\{20B,120B\}, and a random agent (samples action randomly within the coordinate box)---each capped at 25 interaction turns per episode on \textsc{Interphyre} levels. We compare against three baselines: \emph{\textsc{ReAct}}~\citep{yao2023reactsynergizingreasoningacting}, which runs one Thought-Action-Observation trajectory per seed; \emph{Reflexion}~\citep{shinn2023reflexion}, which adds verbal self-reflection; and \emph{\textsc{Direct}}, which prompts the model to solve the task in a single shot from the scene description alone, with no tools, no environment interaction, and no skills, measuring the base models' parametric capability. With the smaller models, we also include RL training via \emph{GRPO}~\citep{shao2024deepseekmath}, which fine-tunes Qwen-2.5-3B with a binary $\{0,1\}$ reward, making it the only method that updates model weights and compares directly against our training-free framework. All methods on a given level are evaluated on the same 50 seeds, so comparisons are paired on identical instances (full details in Appendix~\ref{app:baselines}). In Table~\ref{tab:baseline_results} of Appendix \ref{app:results}, we organize the eight levels into two difficulty tiers based on frontier-model performance: Tier~1 (six levels, Claude Sonnet $\geq96\%$),  and Tier~2 (\texttt{pass\_the\_parcel} at $24\%$, \texttt{catapult} at $8\%$, with every open-weight model scoring $0\%$ on the latter). These two hard levels from Tier~2, where purely parametric reasoning is insufficient, are the primary testbed for \textsc{HExA}.

% \subsection{Instantiation of \textsc{HExA} -- Skill Initialization and Update}
% The skill bank in \textsc{HExA} can have several configurations that vary along two orthogonal axes (Algorithm~\ref{alg})---how the skill bank is initialized before experimentation starts and how it is updated between the experimentation rounds. We tested three initialization methods for our skill banks: \emph{Offline}, \emph{Offline to Online} (\emph{Off2On}), and \emph{Online}. Both Offline and Off2On, warm-start the bank by collecting $N_0$ base-actor trajectories with no skill context and distilling them into $\mathcal{K}_0=\textsc{Evolver}(\emptyset,\mathcal{T}_0)$. In the Offline variant we do not update the skills anymore, while in Off2On we reinitialize the skill bank after new experiments. In the pure Online version, we start with an empty bank ($\mathcal{K}_0=\emptyset$) and the agent bootstrap skills
% purely from its own online interactions. We also have two ways to update the skill bank from interaction feedback: \emph{Evolving} and \emph{Iterative
% Replacement}. The Evolving variant passes the evolver both the current bank and the new round's trajectories, adding new skills and merging, revising, or
% pruning existing skills in light of new experimental evidence
% ($\mathcal{K}_n=\textsc{Evolver}(\mathcal{K}_{n-1},\mathcal{T}^{(n)})$). However, in Iterative Replacement,   we build the skill bank from scratch each time using the current set of rollouts alone, since we assume that in the in-context RL loop, the actor has ingested the previous skills in its policies already. Thus, these newer skills already have the influence of older skills plus additional novelty from these newer experimentation rollouts ($\mathcal{K}_n=\textsc{Evolver}(\emptyset,\mathcal{T}^{(n)})$). We thus have five variants of skill formation and updation—initialization with either \textit{Off2On} or
% \textit{Online} and updation with either \textit{Evolution} or \textit{Iterative Replacement}. And another version where we
% start with a fixed Offline skill bank, and keep it frozen throughout the experiments with no update ($\mathcal{K}_n=\mathcal{K}_{n-1}$). We ablate all five instantiations in Table~\ref{tab:variants_compact} and \emph{Off2On~+~Evolution} performs the best---we thus use this version of skill initialization and update as the default in \textsc{HExA}.


% \begin{figure}[t]
% \centering
% \setlength{\tabcolsep}{1.2pt}
% \renewcommand{\arraystretch}{0.85}
% % --- ReAct row ----------------------------------------------------------
% {\footnotesize\itshape \textsc{ReAct} (25 iterations, FAILURE)}\\[1pt]
% \begin{tabular}{@{}ccccccc@{}}
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step0.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step30.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step57.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step70.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step91.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step151.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step193.png} \\[-1pt]
%   {\scriptsize } & {\scriptsize } & {\scriptsize } &
%   {\scriptsize } & {\scriptsize } &
%   {\scriptsize } & {\scriptsize } \\
% \end{tabular}\\[6pt]
% % --- HExA row -----------------------------------------------------------
% {\footnotesize\itshape \textsc{HExA} (6 iterations, SUCCESS)}\\[1pt]
% \begin{tabular}{@{}ccccccc@{}}
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step0.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step25.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step57.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step74.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step119.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step140.png} &
%   \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step172.png} \\[-1pt]
%   {\scriptsize } & {\scriptsize } & {\scriptsize } &
%   {\scriptsize } & {\scriptsize } &
%   {\scriptsize } & {\scriptsize } \\
% \end{tabular}
% \caption{%
% \textbf{How the evolved skill bank of HExA guides the agent on \texttt{catapult} seed~45.}
% Top: \textsc{ReAct}, which has no cross-episode memory, exhausts its
% 25-iteration budget while repeatedly exploring ineffective placements.
% Bottom: \textsc{HExA} begins with the evolved bank summarized above. After
% observing that its initial launch strikes the ceiling, it applies the bank's
% diagnosis that the limiting factor is launch geometry rather than insufficient
% force. It therefore shifts the drop point toward $x=0.3$ instead of further
% increasing the radius, and succeeds with
% $(x,y,r)=(0.3,0.9,1.5)$ in six interaction iterations. Frames are sampled from
% the final simulations; full prompts, bank entries, and trajectories are
% provided in Appendix~\ref{app:trajectories:bank}.}
% \label{fig:catapult45_simframes}
% \end{figure}


% \begin{figure}[b]
% \centering
% \begin{minipage}[c]{0.50\linewidth}
%   \centering
%   \footnotesize
%   \setlength{\tabcolsep}{3.5pt}
%   \begin{tabular}{lcc}
%   \toprule
%   \textbf{Method} & \textbf{Acc.\ (\%)} & \textbf{Avg Iter} \\
%   \midrule
%   \textsc{Direct} (no tools)    & \phantom{0}2.0           & \phantom{0}1.0          \\
%   \textsc{ReAct}                & \phantom{0}8.0           & 22.9                    \\
%   Reflexion ($K{=}2$)           & $21.3{\pm}2.5$           & $21.2{\pm}0.7$          \\
%   \textsc{HExA} (no reward)     & $50.7{\pm}9.4$           & $16.5{\pm}2.7$          \\
%   \textsc{HExA} (Off2On Evol.)  & $\mathbf{67.3{\pm}9.3}$  & $14.4{\pm}1.8$          \\
%   \bottomrule
%   \end{tabular}
% \end{minipage}\hfill
% \begin{minipage}[c]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/catapult_three_methods_50seeds.pdf}
% \end{minipage}
% \caption{%
%   \textbf{Reward-guided skill accumulation makes \textsc{HExA} much stronger on
%   \texttt{catapult}, the hardest level.}
%   This experiment tests whether an agent can improve by turning past attempts
%   into reusable, reward-guided skills. On \texttt{catapult}, Claude Sonnet solves
%   only $8.0\%$ of seeds with a standard \textsc{ReAct} loop, while \textsc{HExA}
%   reaches $67.3\%$ and uses fewer iterations per solve.
%   \textbf{Left:} final solve rate and average iterations.
%   \textbf{Right:} cumulative success over $50$ seeds; curves show mean over
%   $3$ runs with shaded $\pm 1$ std.
%   Removing the reward signal drops \textsc{HExA} to $50.7\%$, and Reflexion reaches
%   only $21.3\%$, showing that the main gain comes from scoring and reusing skills,
%   not merely from extra interaction or verbal self-reflection.
%   Full protocol in Appendix~\ref{app:baselines}.
% }
% \label{tab:catapult_skillrl}
% \label{fig:catapult_three_methods_50seeds}
% \end{figure}


% \subsection{Results, Analysis, and Ablations}

% We organize our analysis around seven questions about \textsc{HExA}'s efficacy and generality in
% learning-by-experimentation settings, comparing it to base models and agent-side baselines. We ask
% whether converting interaction into an evolving skill bank lets a frontier agent solve levels that
% single-episode agents cannot (\textbf{Q1}) and whether any gain reflects more efficient search
% rather than additional attempts (\textbf{Q2}); whether the benefit extends to smaller open-weight
% models (\textbf{Q3}); which design ingredients---reward guidance, cross-episode evolution, or
% initialization---drive the improvement (\textbf{Q4}); whether the distilled skills are hierarchical
% and build on one another across rounds (\textbf{Q5}); whether they transfer to unseen levels
% (\textbf{Q6}); and whether in-context skill learning is more sample-efficient than gradient-based RL
% at a matched interaction budget (\textbf{Q7}). Unless noted otherwise, all methods on a level are
% evaluated on the same seeds under an identical $25$-iteration \textsc{ReAct} harness, and
% \textsc{HExA} uses its default Off2On Evolving configuration ($x{=}3$ seeds per round).


% \paragraph{Q1: Can distilling interaction into an evolving skill bank solve hard levels that defeat single-episode agents?}
% On the two Tier-2 levels---\texttt{catapult} ($8\%$ \textsc{ReAct}) and \texttt{pass\_the\_parcel}
% ($24\%$ \textsc{ReAct})---a frontier model fails under a single \textsc{ReAct} trajectory, so we
% hypothesize that turning interaction traces into an evolving skill bank should yield substantially
% higher solve rates than agent-side baselines that accumulate no reusable skills (\textsc{Direct},
% \textsc{ReAct}, Reflexion). We test this with Claude Sonnet, running every method on the same $50$
% seeds per level; \textsc{HExA} and Reflexion are repeated over $3$ independent runs
% (mean~$\pm$~std), while \textsc{Direct} and \textsc{ReAct} are deterministic single runs.
% \textsc{HExA} turns both levels from mostly-unsolved one-episode problems into substantially
% solvable in-context learning tasks. On \texttt{catapult} it reaches $67.3 \pm 9.3\%$, against
% $2.0\%$ (\textsc{Direct}), $8.0\%$ (\textsc{ReAct}), and $21.3 \pm 2.5\%$ (Reflexion)
% (Table~\ref{tab:catapult_skillrl}); on \texttt{pass\_the\_parcel} it reaches $60.0\%$, against
% $24.0\%$ (\textsc{ReAct}), $16.0\%$ (Reflexion), and $0.0\%$ (\textsc{Direct})
% (Table~\ref{tab:ptp_variants}). Because \texttt{pass\_the\_parcel} requires discovering the
% ramp-and-basket mechanism rather than a direct collision, the gain indicates that distilling past
% interactions into reusable strategies---not merely retrying---is what makes the level solvable.
% Figure~\ref{fig:catapult45_simframes} shows a representative \texttt{catapult} seed where
% \textsc{HExA} solves the task in a handful of iterations by reusing previously distilled placement
% heuristics, while \textsc{ReAct} exhausts its budget without finding a working launch.


% \begin{figure}[h]
%   \centering
%   \begin{minipage}[t]{0.49\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/catapult_var_cum_avg_iter.pdf}
%     \subcaption{Catapult (25 seeds).}
%     \label{fig:catapult_var_cum_iter}
%   \end{minipage}\hfill
%   \begin{minipage}[t]{0.49\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/ptp_cum_avg_iter.pdf}
%     \subcaption{Pass the Parcel (50 seeds).}
%     \label{fig:ptp_cum_iter}
%   \end{minipage}
%   \caption{%
%     \textbf{Cumulative average \textsc{ReAct} iterations per seed} for every \textsc{HExA}
%     variant against the baseline (Claude Sonnet); lower is more efficient. On both levels the
%     Off2On Evolving configuration converges to the lowest cost per seed, while the iterative and
%     pure-online variants remain higher, indicating that \textsc{HExA}'s gains come from guiding
%     search more efficiently with accumulated experience rather than from spending more
%     computation per instance.
%   }
%   \label{fig:cum_iter_both}
% \end{figure}


% \paragraph{Q2: Is \textsc{HExA}'s advantage more efficient search, or just more attempts?}
% A higher solve rate alone could arise from spending more interaction per seed or from occasional
% lucky placements, rather than from genuinely easier episodes. We therefore record, on the same runs
% as Q1, the average number of \textsc{ReAct} iterations per seed as an efficiency proxy, and track
% the cumulative success and cumulative iteration curves across the seed sweep. \textsc{HExA} lowers
% the average iterations from $22.9$ (\textsc{ReAct}) and $21.2 \pm 0.7$ (Reflexion) to
% $14.4 \pm 1.8$, roughly $37\%$ fewer, so each episode becomes genuinely easier rather than merely
% more numerous (Figure~\ref{fig:catapult_three_methods_50seeds}). The cumulative curves stay
% separated throughout the sweep---\textsc{HExA}'s success curve remains above the baselines while its
% iteration curve converges below them (Figures~\ref{fig:catapult_three_methods_50seeds}
% and~\ref{fig:cum_iter_both})---so the ranking is not an artifact of a few lucky seeds, and the extra
% accuracy comes with less, not more, computation per instance; the same per-seed efficiency pattern
% holds on \texttt{pass\_the\_parcel}. Reflexion, which adds verbal self-reflection but keeps no
% persistent bank, trails \textsc{HExA} by $46$~percentage points (pp) on \texttt{catapult} and
% $29$~pp even after the reward signal is removed, evidence that the gain comes from reusing distilled
% skills rather than from extra trials or in-context verbalization alone.


% \begin{table}[h]
% \centering
% \small
% \caption{%
%   \textsc{HExA} on open-weight solvers, 50 training/evaluation seeds per cell
%   (max 25 iterations). Qwen-2.5 runs use the Online-Evolving configuration ($k{=}3$ seeds
%   per round, 17 rounds); GPT-OSS-120B uses Off2On Evolving. Baselines are the same agent with
%   no skill injection. Per-seed cumulative trajectories in Figure~\ref{fig:hexa_smallmodels}.
% }
% \label{tab:hexa_smallmodels_main_paper}
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{0.95}
% \begin{tabular}{llcc}
% \toprule
% \textbf{Level} & \textbf{Method} & \textbf{Acc.\ (\%)} & \textbf{Avg Iters} \\
% \midrule
% \multirow{4}{*}{Down to Earth}
%   & Qwen-2.5-3B \textsc{ReAct} & \phantom{0}8.0 & 23.8 \\
%   & Qwen-2.5-3B \textsc{HExA}  & \textbf{24.0}  & 18.6 \\
%   \cmidrule(lr){2-4}
%   & Qwen-2.5-7B \textsc{ReAct} & 62.0           & 12.5 \\
%   & Qwen-2.5-7B \textsc{HExA}  & \textbf{72.0}  & 12.6 \\
% \midrule
% \multirow{4}{*}{Two Body Problem}
%   & Qwen-2.5-3B \textsc{ReAct} & \phantom{0}6.0 & 24.0 \\
%   & Qwen-2.5-3B \textsc{HExA}  & \textbf{14.0}  & 21.1 \\
%   \cmidrule(lr){2-4}
%   & Qwen-2.5-7B \textsc{ReAct} & 18.0           & 22.2 \\
%   & Qwen-2.5-7B \textsc{HExA}  & \textbf{34.0}  & 18.9 \\
% \midrule
% \multirow{2}{*}{Catapult}
%   & GPT-OSS-120B \textsc{ReAct} & \phantom{0}0.0 & 25.0 \\
%   & GPT-OSS-120B \textsc{HExA}  & \textbf{54.0}  & 16.2 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \paragraph{Q3: Does the benefit extend to smaller open-weight models, not just a frontier solver?}
% If \textsc{HExA}'s gains depended on a frontier model's reasoning, they would not appear with weaker
% actors. We therefore run the same skill-injection loop on open-weight solvers---Qwen-2.5-\{3B,7B\}
% and GPT-OSS-120B---against a matched baseline that is the identical agent with no skill injection
% (Qwen runs use Online Evolving with $k{=}3$ seeds per round; GPT-OSS-120B uses Off2On Evolving).
% Across every level and model, \textsc{HExA} improves over its baseline
% (Table~\ref{tab:hexa_smallmodels_main_paper}): on \texttt{down\_to\_earth}, Qwen-2.5-3B rises
% $8.0\to24.0\%$ and Qwen-2.5-7B $62.0\to72.0\%$; on \texttt{two\_body\_problem}, $6.0\to14.0\%$ and
% $18.0\to34.0\%$; and on \texttt{catapult}, GPT-OSS-120B rises from $0.0\%$ to $54.0\%$. Gains range
% from $+8$ to $+54$~pp, so the mechanism is not specific to a frontier model. Per-seed cumulative
% trajectories and the full sweep are in Figure~\ref{fig:hexa_smallmodels} and Appendix~\ref{sec:h2}.


% \begin{wraptable}[11]{r}{0.45\linewidth}
% \vspace{-8pt}
% \centering
% \scriptsize
% \caption{%
%   Reward-signal ablation on Qwen-2.5-7B, 50 seeds per cell.
%   Full \textsc{HExA} uses reward-guided, two-pass distillation;
%   the no-reward variant treats successful trajectories equally.
% }
% \label{tab:reward_ablation}
% \begin{tabular}{@{}llcc@{}}
% \toprule
% \textbf{Level} & \textbf{Method}
%   & \textbf{Acc.\ (\%)}
%   & \textbf{Iters} \\
% \midrule
% \multirow{3}{*}{Down to Earth}
%   & \textsc{ReAct}              & 62.0          & 12.5 \\
%   & \textsc{HExA} no reward     & 64.0          & 14.8 \\
%   & \textsc{HExA} reward        & \textbf{72.0} & 12.6 \\
% \midrule
% \multirow{3}{*}{Two Body}
%   & \textsc{ReAct}              & 18.0          & 22.2 \\
%   & \textsc{HExA} no reward     & 26.0          & 22.2 \\
%   & \textsc{HExA} reward        & \textbf{34.0} & 18.9 \\
% \bottomrule
% \end{tabular}
% \vspace{-10pt}
% \end{wraptable}


% \begin{wraptable}{l}{0.45\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \caption{%
%   \textsc{HExA} variant accuracy (\%) on the two hard levels (Claude Sonnet;
%   \textbf{Cat.}~=~\texttt{catapult}; \textbf{PtP}~=~\texttt{pass\_the\_parcel}). Off2On Evolving ($x{=}3$), referred to simply as \textsc{HExA}, is best on both.}
% \label{tab:variants_compact}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Configuration} & \textbf{Cat.} & \textbf{PtP} \\
% \midrule
% Off2On Evolving (HExA) & \textbf{76.0} & \textbf{60.0} \\
% Off2On Iterative       & 56.0          & 48.0          \\
% Online Evolving        & 44.0          & 58.0          \\
% Online Iterative       & 36.0          & 56.0          \\
% Offline Static         & 60.0          & 48.0          \\
% \bottomrule
% \end{tabular}
% \end{wraptable}


% \paragraph{Q4: Which ingredients drive the improvement---reward guidance, cross-episode evolution, or initialization?}
% Given the configuration axes defined in Section~\ref{sec:setup} (initialization: Offline / Off2On /
% Online; update: Evolving / Iterative Replacement), we now isolate which ingredients are responsible
% for \textsc{HExA}'s gains. We probe three candidate drivers in turn: the reward signal supplied to
% the evolver, evolving the bank across rounds versus rebuilding it each round, and warm-starting the
% bank versus starting cold.

% \emph{Reward guidance.} We first ablate the reward signal in the evolver so that every success and
% failure is treated identically, regardless of how efficiently it was reached. (The reward enters as
% a priority label the evolver acts on when retaining or pruning skills, not as a numeric weight in a
% learned sum.) On Qwen-2.5-7B this calibration accounts for most of the gain: on
% \texttt{down\_to\_earth} the unguided variant reaches only $64\%$ ($+2$~pp over \textsc{ReAct})
% versus $72\%$ for full \textsc{HExA} ($+10$~pp), and on \texttt{two\_body\_problem} it reaches $26\%$
% versus $34\%$ (Table~\ref{tab:reward_ablation}). The same effect appears with a frontier solver: on
% \texttt{catapult}, removing the reward signal lowers Claude Sonnet from $67.3 \pm 9.3\%$ to
% $50.7 \pm 9.4\%$ (Figure~\ref{fig:catapult_three_methods_50seeds}). Reward calibration thus lets the
% evolver separate efficiently-solved trajectories from merely-successful ones, so the skills it keeps
% and refines are the more reusable ones.

% \emph{Cross-episode evolution.} We next sweep the update rule with initialization held fixed.
% Evolving the bank across rounds consistently beats distilling it once: on \texttt{pass\_the\_parcel}
% the evolving variants reach $58$--$60\%$ versus $48\%$ for a frozen offline bank and $24\%$ for
% \textsc{ReAct} (Table~\ref{tab:ptp_variants}), and on \texttt{catapult} Off2On Evolving reaches
% $76\%$ versus $56\%$ and $36\%$ for the two iterative variants and $60\%$ for the frozen offline bank
% (Table~\ref{tab:variants_compact}; full per-configuration breakdown in Appendix
% Table~\ref{tab:catapult_variants}). The cumulative-accuracy curves on both levels
% (Figure~\ref{fig:cum_accuracy_both}) make the mechanism visible: the evolving variants pull steadily
% away from the others as each round adds evidence, instead of plateauing like a one-shot
% distillation, because re-distilling from scratch discards accumulated skills and amplifies drift.

% \emph{Initialization.} Holding the update rule at Evolving, the warm start helps but matters less:
% Off2On reaches $76\%/60\%$ on \texttt{catapult}/\texttt{pass\_the\_parcel} versus $44\%/58\%$ for a
% cold Online start, with the gap sharpest on \texttt{catapult} because a cold start spends its early
% rounds rediscovering basic strategies from a few correlated trajectories, an advantage that shrinks
% once online evolution takes over. Combining a broad offline prior with cumulative refinement,
% \emph{Off2On Evolving} is best on both levels and is the configuration we refer to as \textsc{HExA}
% throughout.


% \paragraph{Q5: Does \textsc{HExA} learn hierarchical skills that build on one another across rounds?}
% A central claim is that \textsc{HExA} accumulates not only per-seed recipes but skills that compose
% into increasingly abstract principles. Because each round's trajectories are generated while the
% actor is already conditioned on the previous round's retrieved skills, a new skill can refine,
% bound, merge with, or overturn an earlier one---so we ask whether the evolved bank shows such
% layering rather than a flat list of placements. We examine this qualitatively through the evolved
% \texttt{catapult} bank (Appendix~\ref{app:trajectories:bank}). Within a round, the evolver abstracts
% trajectory-level evidence into general principles: experiments at $x{=}0.5$ showed that $r{=}1.0$
% fell short, $r{=}1.5$ struck the ceiling, and intermediate radii $r\in[1.1,1.4]$ did not resolve the
% tradeoff; rather than store these as separate parameter prescriptions, the evolver inferred that
% ceiling clearance is governed by launch angle and contact geometry, not impact energy alone, and
% consolidated them into a higher-level rule---when radius tuning at fixed $x$ alternates between
% insufficient range and ceiling collisions, stop interpolating $r$ and shift $x$ toward $0.1$--$0.3$
% to flatten the launch arc. This compresses many $(x,y,r)$ trials into both a reusable physical
% principle and a policy for \emph{when to abandon local parameter search}. The hierarchy also
% develops across rounds: the seed-45 solve in Figure~\ref{fig:catapult45_simframes} applies exactly
% this layered structure---a learned default launch, a diagnosed ceiling failure, and the corrective
% geometry shift---to succeed in six iterations. We read these as evidence of compositional,
% hierarchical skill formation rather than proof, and provide the full bank and trajectories in
% Appendix~\ref{app:trajectories:bank}.


% \begin{wrapfigure}[14]{l}{0.56\linewidth}
%   \vspace{-10pt}
%   \centering
%   \includegraphics[width=\linewidth]{figures/cross_level_transfer.pdf}
%   \caption{%
%     Cross-level skill transfer with no target trajectories. Each target is solved using only skills synthesised from source-level banks; labels report target success and matched \textsc{ReAct} baselines. Multi-source transfer to \texttt{catapult} yields the largest gain
%     ($+36$~pp).
%   }
%   \label{fig:cross_level_transfer}
%   \vspace{-12pt}
% \end{wrapfigure}


% \paragraph{Q6: Are the learned skills reusable on unseen levels?}
% If \textsc{HExA} distills genuinely reusable physics primitives rather than level-specific recipes,
% skills from source levels should help on an unseen target with no target-level experience. We test
% this by synthesising a target bank from source-level banks plus a textual description of the target
% alone---no target-level trajectories are generated at any stage---and injecting it with no further
% evolution. Combining fully-evolved banks from three source levels (\texttt{down\_to\_earth},
% \texttt{two\_body\_problem}, \texttt{pass\_the\_parcel}), the evolver synthesises a \texttt{catapult}
% bank that raises Claude Sonnet from $8.0\%$ to $44.0\%$ ($+36$~pp), closing roughly $60\%$ of the
% gap to the within-level \textsc{HExA} result of $64\%$ (Table~\ref{tab:cross_level},
% Figure~\ref{fig:cross_level_transfer}); this is consistent with \texttt{catapult}'s lever-launch
% dynamics sharing structural primitives (collision normals, energy thresholds, directional impulse)
% with the source levels. Transfer also helps with a single source bank and a smaller teacher:
% on a structurally similar pair (\texttt{down\_to\_earth}~$\to$~\texttt{falling\_into\_place}) it
% gains $+12$~pp, and on a dissimilar pair (\texttt{down\_to\_earth}~$\to$~\texttt{two\_body\_problem})
% it still gains $+16$~pp (Table~\ref{tab:cross_level}). That transfer succeeds even across dissimilar
% levels suggests the evolver extracts abstract principles---momentum transfer, contact
% geometry---rather than narrow placement heuristics.


% \input{figures/grpo_comparision_figure}


% \paragraph{Q7: At a matched interaction budget, is in-context \textsc{HExA} more sample-efficient than gradient-based RL?}
% Finally we ask whether in-context skill evolution is more sample-efficient than updating model
% weights from the same experience. We compare against GRPO~\citep{shao2024deepseekmath} fine-tuning
% Qwen-2.5-3B on the same levels, matched on the number of model updates and on $50$ unique
% environment seeds. At this budget GRPO reaches $20\%$ on \texttt{down\_to\_earth} and $6\%$ on
% \texttt{two\_body\_problem}, versus \textsc{HExA}'s $24\%$ and $14\%$
% (Figure~\ref{fig:grpo_comparison_main}). The gap reflects the core advantage of in-context skill
% evolution: strategies distilled from early trajectories are immediately available to later episodes
% through context, whereas gradient-based methods must accumulate signal over many rollouts before the
% weights encode equivalent knowledge---so in harder domains where early successes are rare,
% \textsc{HExA} can still bootstrap learning from failure and partial-success trajectories. With many
% more updates, GRPO can eventually close the gap through direct optimization on the environment
% reward. We present more details of these ablations in Appendix~\ref{sec:h5}.


==> sections/5_new_results.tex <==
% =====================================================================
% NEW RESULTS SECTION (ICLR).  Self-contained; does not touch
% 4_exp_results_Jun24.tex.  Environments are kept separate here by
% design -- merging into a single cross-benchmark table is a later call.
%
% Maze: the Qwen3-8B half is reported (n=3, both designs positive).  The
% gpt-oss-120b half is held pending replication of its within-level arm,
% which is the only n=1 arm there.  Both live in DOC_Results/MAZE_RESULTS.md.
% =====================================================================

\section{New Results}
\label{sec:new_results}

We evaluate \textsc{HExA} on four benchmark families: \textsc{InterPhyre}, two
interactive games, four reasoning and planning tasks, and
\textsc{DiscoverPhysics}. Three of the four are external. On the reasoning and
planning tasks, \textsc{Core}~\citep{nasvytis2026core} is a direct
methodological competitor with published numbers on the same problems. Each
subsection below reports one family.

\subsection{Setup and protocol}
\label{sec:new_results_setup}

Every number in this section comes from a \emph{frozen} bank. The bank is
evolved on a training partition, frozen, and then evaluated on a disjoint
held-out partition that the bank never saw. No distillation or evolution happens
during evaluation. On \textsc{InterPhyre} each bank is evolved on 50 training
seeds and evaluated on a disjoint set of 50 held-out seeds; the games, the
reasoning tasks and \textsc{DiscoverPhysics} use their own published or
pre-registered splits.

Actor and evolver are the same frozen model in every game, reasoning-task and
\textsc{DiscoverPhysics} run. No stronger teacher enters the
loop, so the gains below are self-improvement rather than distillation from a
larger model.

Every comparison is paired on identical instances. We report exact McNemar tests
or paired sign tests on per-instance outcomes, with replicates pooled. Where an
arm was built more than once, the reported figure is the mean over independently
built memories and the significance fraction counts how many arm-run $\times$
baseline-run pairs reach $p<0.05$.

Baselines fall into three groups. \textsc{ReAct} and Reflexion are verbal
self-improvement methods with no persistent store. Episodic RAG and MemRL are
external memory methods: the first retrieves past instances verbatim, the second
maintains (intent, experience, utility) triplets. GRPO is a weight-update
baseline. \textsc{Core}~\citep{nasvytis2026core} is run both from its published
numbers and from its own released code on our provider.

\subsection{\textsc{InterPhyre}}
\label{sec:new_results_interphyre}

\textbf{Skill banks lift a frozen open-weight agent on both levels we measure
with paired tests.} Table~\ref{tab:interphyre_qwen} reports Qwen-2.5-7B on
\texttt{down\_to\_earth} and \texttt{two\_body\_problem}. Success rises 63.3\% to
82.7\% on the first level and 12.0\% to 50.0\% on the second. The agent also
solves levels in fewer turns, 13.4 to 10.4 and 23.1 to 15.8 iterations.

\textbf{The bank is cheap, and it stays cheap.} On \texttt{catapult}
(Table~\ref{tab:catapult_memory}) \textsc{HExA} injects 2{,}392 tokens per
episode against 6{,}706 for Episodic RAG and 8{,}135 for MemRL. The frozen bank
holds 10 skills and 5 mistakes regardless of how many episodes have been played.
The episodic baselines inject whole rollouts, so their context grows with the
rollout cap rather than with anything learned.

\input{tables/interphyre_qwen}
\input{tables/catapult_memory}

\textbf{Content does the work, not context length.}
Table~\ref{tab:interphyre_ablation}(a) varies only what is retrieved from one
frozen bank, so no difference between arms can come from a different training
run. The wrong-level arm injects 2{,}862 characters of fluent, well-formed
skills distilled from a different level, keeping the level's own mistakes. It
buys nothing over an empty prompt (9.3\% against \textsc{ReAct}'s 12.0\%,
$p=0.664$). This is the control that separates the method from the prompt:
length is held in the same range as the full bank, and only content changes.

\textbf{The bank's internal ranking is load-bearing.}
Table~\ref{tab:interphyre_ablation}(b) drops two skills from one bank in two
ways. Dropping the two lowest-confidence skills costs nothing (76.7\% against
76.7\%). Dropping the two highest-confidence skills costs 11.4 points. The two
dropped sets are disjoint and the injected lengths differ by 0.9\%, so the
comparison isolates the ranking ($p=0.019$).

Permuting the confidences while keeping every skill changes nothing
($p=0.845$). The retrieval budget is six against a five-skill bank, so every
skill is injected however the confidences fall: this arm tests the order skills
appear in the prompt, not confidence-based selection.

Two components are inert on this level. Mistakes add nothing over skills alone
($p=0.281$), and mistakes alone do not beat an empty prompt ($p=0.210$). The
gain is carried by the skills.

\input{tables/interphyre_ablation}

\subsection{Interactive games: Mastermind and Maze}
\label{sec:new_results_orbit}

These tasks are not physics. They test whether the method survives outside the
environment we built. We report Mastermind~\citep{liu2025gem} and
Maze~\citep{lin2026orbit} under the cross-episode protocol
of~\citep{lin2026orbit}: each instance is played for three episodes with the
hidden task held fixed, so the metric is per-episode success rather than a
single rate. The transfer experiments below additionally use Wordle and
Minesweeper from the same suite~\citep{liu2025gem}, as sources only.

\textbf{On Maze the bank helps a smaller actor, and the gain replicates.}
Table~\ref{tab:maze_qwen} reports Qwen3-8B on 243 held-out mazes. Within-task
\textsc{HExA} raises \texttt{any} 8.5 points over no memory and ep3
7.0 points; significance is reported in the table. Restricting to
instances the bank never saw during training leaves the gain intact at
$+$8.1 points.

\textbf{Distillation beats episodic memory at a fraction of the context.}
Table~\ref{tab:orbit_memory} places \textsc{HExA} against Episodic RAG and MemRL
on the same 40 held-out instances. \textsc{HExA} is the only arm that clearly
beats no memory ($+.225$ ep3). Episodic RAG falls \emph{below} no
memory while spending twice the tokens. MemRL is statistically indistinguishable
from no memory at 3.5$\times$ the tokens. The head-to-head margins are $+.242$
against RAG and $+.190$ against MemRL; both are significant (Table~\ref{tab:orbit_memory}).

\textbf{The same ordering holds on a second model and a second task.} On Maze
with Qwen3-8B (Table~\ref{tab:maze_qwen}) \textsc{HExA} spends 429 tokens against
Episodic RAG's 5{,}457 and MemRL's 7{,}027, and beats both on ep3 by $+.163$ and
$+.117$ (Table~\ref{tab:maze_qwen}). Episodic RAG posts the highest ep1 in the table, .333,
because its retrieval has a prior instance's transcript to draw on before the
agent has explored anything. It then falls \emph{below} no memory on ep3
($-.093$): the retrieved transcript displaces the agent's own
cross-episode observations rather than supplementing them.

\textbf{Reflexion is the cheapest arm and the weakest on both tasks.} It trails
\textsc{HExA} by $.243$ on Maze ep3 at 194 tokens, and by $.192$ on
Mastermind \texttt{any} at 269; both gaps are significant. Placing the trial boundary correctly
requires wiping the transcript between episodes, which is what makes it
Reflexion rather than the trajectory-only ablation. On Maze that discards
exactly the spatial structure a verbal lesson cannot restate, and its ep3 falls
below its own ep2, the only arm anywhere that does so.

\textbf{The cost advantage is the one that holds on every actor.}
Table~\ref{tab:mastermind_qwen} repeats the Mastermind comparison on Qwen3-8B.
\textsc{HExA} is the only arm that beats no memory on \texttt{any} ($+.273$,
significant), at 359 tokens against Episodic RAG's 1{,}965 and MemRL's 3{,}192.
Episodic RAG reaches comparable ep3 accuracy there for 5.5$\times$ the context.

\input{tables/orbit_memory_headtohead}

\textbf{A bank built without a single target-task trajectory matches a
target-trained bank.} Table~\ref{tab:orbit_transfer} reports cross-task
transfer, in which the Mastermind bank is synthesised from other tasks' banks
plus a 15-line statement of Mastermind's rules, without playing a single
Mastermind episode. Transfer from Wordle reaches .933 on ep3,
$+28.3$ over no memory and significant across replicates (Table~\ref{tab:orbit_transfer}), at 946 injected
tokens against the within-task bank's 971. It matches the within-task bank, which reaches
.875 on the same instances.

\textbf{Re-grounding is what makes transfer work.} The same Wordle bank injected
verbatim scores .575 on ep3, below the no-memory baseline of .650, against .933
after synthesis. A 36-point gap on identical source material separates
re-grounded skills from relevant text in the prompt. Source similarity also
matters more than we expected: transfer from Minesweeper reaches only 4 of 9
pairs, and combining both sources reaches 0 of 9.

\textbf{Transfer reproduces on a different task, a different model and a
different source.} On Maze with Qwen3-8B, a bank synthesised from Wordle-5
matches or beats the Maze-trained bank on every metric using zero Maze
trajectories (Table~\ref{tab:maze_qwen}). The sharpest gap is first-episode
success, $+$8.4 points against the within-task bank's $+$3.9. A bank distilled from a word
game helps on first contact with a maze more than a bank trained on mazes does.

\textbf{Transfer depends on the actor.} On Mastermind with Qwen3-8B the
Wordle-synthesised bank reaches .450 on \texttt{any} against the
Mastermind-trained bank's .640 (Table~\ref{tab:mastermind_qwen}). Acting on an
abstractly stated rule appears to require capacity the smaller actor does not
have.

\input{tables/orbit_transfer}

\subsection{Reasoning and planning tasks}
\label{sec:new_results_core}

The four tasks are MathGAP~\citep{opedal2024mathgap},
ZebraLogic~\citep{lin2025zebralogic}, Tower of Hanoi~\citep{shojaee2025illusion}
and matchstick arithmetic~\citep{nasvytis2026insight}, each a single-turn
problem family with a generator and a programmatic verifier. We use the
four-task configuration and the $100$-item held-out sets released with
\textsc{Core}~\citep{nasvytis2026core}, which shares \textsc{HExA}'s premise
that memory can improve a frozen model and publishes numbers on exactly these
problems. We additionally rerun \textsc{Core}'s released code on our own
provider, so at least one comparison does not cross a provider boundary.

\textbf{\textsc{HExA} improves the frozen model on all four tasks, and beats
every published baseline on three of them at 3.3$\times$ fewer rollouts.}
Table~\ref{tab:core} reports the paired arms above and the published field
below. Gains over our own no-memory arm are $+0.353$ on MathGAP, $+0.247$ on
ZebraLogic and $+0.257$ on Tower of Hanoi, each highly significant (Table~\ref{tab:core}).
Matchstick moves only $+0.050$.

\textbf{Matchstick is the exception.} \textsc{Core}'s published 100-item cell
(0.870) and our matched-budget rerun (0.830) both beat \textsc{HExA}'s 0.787,
while MemRL's 0.703 does not. On MathGAP \textsc{HExA} is comparable to
\textsc{Core}, at 0.863 against 0.843.

\textbf{The compute argument is visible in the last column.} GRPO, a
weight-update method at 3000 rollouts, trails \textsc{HExA} at 900 on all four
tasks. Context cost is 952--990 tokens per evaluation item, the same order as
\textsc{Core}'s 0.92k and roughly 35$\times$ below Episodic RAG and MemRL as run
on these tasks.

\input{tables/core_headtohead}

\subsection{\textsc{DiscoverPhysics}}
\label{sec:new_results_discovery}

\textsc{DiscoverPhysics} is the strongest form of the claim, because the bank
here holds experimentation strategies rather than solutions. An agent is placed
in a 2D world governed by an unknown field equation, designs experiments,
observes noisy particle trajectories, and submits the governing law as executable
Python with a prose explanation.

\textbf{A frozen bank turns a task the agent never solves into one it solves
two-thirds of the time.} On \texttt{oscillator} (Table~\ref{tab:discovery})
pass-rate goes 0/15 to 10/15 and the explanation score rises 0.447; both are
significant (Table~\ref{tab:discovery}). Every passing episode clears the
benchmark's strict 0.90 gate, which the baseline never reaches. On
\texttt{circle} pass-rate goes 1/15 to 8/15, with explanation and reward
moving in the same direction.

\textbf{The bank also transfers across worlds.} \texttt{oscillator} and
\texttt{circle} are within-world accumulation: the bank encodes that world's own
physics, learned from the agent's own experiments. \texttt{hubble} is
cross-world, with the bank grown on nine other worlds and \texttt{hubble} never
seen. It gains $+0.300\pm0.126$ in reward and lifts pass@0.90 from 0\% to 79\%
at $k{=}3$.

\input{tables/discovery}

\subsection{What holds across benchmarks}
\label{sec:new_results_synthesis}

Three claims survive on more than one benchmark family. First, a distilled bank
improves a frozen actor on all 11 tasks that have a paired no-memory
baseline, across three external benchmark families. Second, the bank beats
episodic memory while spending a fraction of the context: 971 tokens against
1{,}957 and 3{,}416 on Mastermind, 429 against 5{,}457 and 7{,}027 on Maze,
2{,}392 against 6{,}706 and 8{,}135 on \texttt{catapult}, and 952--990 against
roughly 33k on the reasoning tasks. The cost ordering holds in every cell we measured,
on two model families. Third, the gain comes from what is
distilled rather than from the presence of text, established by a length-matched
placebo on \textsc{InterPhyre} and by a raw-dump ablation on Mastermind that
scores below no memory at all.

One pattern cuts across the four families. Gains concentrate in later episodes:
on Mastermind ep1 moves little or negatively while ep3 carries
the gain, and on Maze the ep1 move is small against a larger ep3 gain, so the
method improves cross-episode adaptation more than first-attempt competence.


==> sections/exp_results_scott_comments.tex <==
\section{Experiments and Results on Interphyre}
\label{sec:experiments}

In this section, we provide details of \textsc{Interphyre}, and evaluate different LLMs on experiment-centric tasks using \textsc{Interphyre} levels. Our benchmark is designed with the following key properties:

\begin{enumerate}[label=(\roman*)]
    \item tasks whose solution is unknown or cannot be read off a static description and must be discovered by interacting with the environment.
    \item a programmatic interface that lets the agent autonomously inspect the scene, test interventions, and observe intermediate dynamics.
    \item a controllable difficulty range with procedural generation.
\end{enumerate}

% \begin{wraptable}{r}{0.58\linewidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{%
%   \textsc{ReAct} baseline solve rate~(\%) across eight
%   \textsc{Interphyre} levels.
%   Levels grouped by difficulty tier based on Claude Sonnet performance.
%   \textsuperscript{$\dagger$}Evaluated on 50 seeds;
%   \textsuperscript{$\ddagger$}25 seeds;
%   all others 100 seeds.
%   --- = not evaluated.
% }
% \label{tab:baseline_results}
% \begin{tabular}{lcccccc}
% \toprule
% & \textbf{Rand} & \textbf{Q-7B} & \textbf{Q-14B}
% & \textbf{O-20B} & \textbf{O-120B} & \textbf{Son.} \\
% \midrule
% \multicolumn{7}{l}{\textit{Tier~1: Solvable}} \\
% Cliffhanger      & 0  & 2.0  & 6.0  & 30.5 & 64.0 & 100$^{\ddagger}$ \\
% Tipping Point    & 3  & 24.0 & 42.0 & 80.0 & 90.1 & 96$^{\ddagger}$  \\
% Basket Case      & 4  & 8.0  & 10.0 & 14.0 & 33.0 & 100$^{\ddagger}$ \\
% Down to Earth    & 8  & 62.0 & 72.0 & 35.0 & 72.5 & 100             \\
% Two Body         & 14 & 18   & 24.0 & 26.0 & 77.8 & 100             \\
% Falling in Place & 1  & 20.0 & 52.0 & 58.0 & 100  & 100$^{\dagger}$ \\
% \addlinespace[2pt]
% \multicolumn{7}{l}{\textit{Tier~2: Hard}} \\
% Pass the Parcel  & 0  & 7.8  & 9.8  & 16   & 22   & 24$^{\dagger}$  \\
% Catapult         & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 8$^{\dagger}$   \\
% \bottomrule
% \end{tabular}
% \end{wraptable}




% \begin{wraptable}{r}{0.44\linewidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{%
%   \textsc{ReAct} baseline solve rate~(\%) across eight
%   \textsc{Interphyre} levels.
%   Levels grouped by difficulty tier based on Claude Sonnet performance.
%   \textsuperscript{$\dagger$}Evaluated on 50 seeds;
%   \textsuperscript{$\ddagger$}25 seeds;
%   all others 100 seeds.
%   --- = not evaluated.
% }
% \label{tab:baseline_results}
% \begin{tabular}{lccc}
% \toprule
% & \textbf{Q-7B} & \textbf{O-120B} & \textbf{Son.} \\
% \midrule
% \multicolumn{4}{l}{\textit{Tier~1: Solvable}} \\
% Cliffhanger    & 2.0  & 64.0 & 100$^{\ddagger}$ \\
% Tipping Point  & 24.0 & 90.1 & 96$^{\ddagger}$  \\
% Basket Case    & 8.0  & 33.0 & 100$^{\ddagger}$ \\
% Down to Earth  & 62.0 & 72.5 & 100             \\
% Two Body       & 18.0 & 77.8 & 100             \\
% Falling Place  & 20.0 & 100  & 100$^{\dagger}$ \\
% \addlinespace[2pt]
% \multicolumn{4}{l}{\textit{Tier~2: Hard}} \\
% Pass Parcel    & 7.8  & 22.0 & 24$^{\dagger}$  \\
% Catapult       & 0.0  & 0.0  & 8$^{\dagger}$   \\
% \bottomrule
% \end{tabular}
% \end{wraptable}








% \begin{wraptable}{r}{0.34\linewidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{%
%   \textsc{ReAct} solve rate (\%) of Claude Sonnet across the eight
%   \textsc{Interphyre} levels, grouped by difficulty tier.
%   \textsuperscript{$\dagger$}50 seeds; \textsuperscript{$\ddagger$}25 seeds;
%   others 100.}
% \label{tab:baseline_results_sonnet}
% \begin{tabular}{lc}
% \toprule
% \textbf{Level} & \textbf{Acc.\ (\%)} \\
% \midrule
% \multicolumn{2}{l}{\textit{Tier~1: Solvable}} \\
% Cliffhanger    & 100$^{\ddagger}$ \\
% Tipping Point  & 96$^{\ddagger}$  \\
% Basket Case    & 100$^{\ddagger}$ \\
% Down to Earth  & 100             \\
% Two Body       & 100             \\
% Falling Place  & 100$^{\dagger}$ \\
% \addlinespace[2pt]
% \multicolumn{2}{l}{\textit{Tier~2: Hard}} \\
% Pass Parcel    & 24$^{\dagger}$            \\
% Catapult       & \phantom{0}8$^{\dagger}$  \\
% \bottomrule
% \end{tabular}
% \end{wraptable}









% \scott{Start with scientific goals: What do we want to show/test and what properties  does a benchmark domain need . Then introduce Interohyre + why it fullfills that role after it has been motivated}
% \utsav{[Addressed: opening rewritten to lead with the scientific goal and the properties a benchmark must have, and only then introduce \textsc{Interphyre} as a domain that satisfies them.]}
% \sout{We first explain our new benchmark \textsc{Interphyre} and its utility to better study the problem setting of in-context learning via active experimentation. With our diverse set of experiments and ablations we try to understand the how and why frontier LLMs as well as small open LLMs severely under perform.}\scott{Poorly framed/ Confusing} \sout{We then analyze how self-improvement methods like our HExA based on in-context RL and autonomous skill evolution and consolidation are well suited for the complicated problem setting of the complicated problem setting of learning for interaction and active experimentation on our benchmark \textsc{Interphyre}} 
% \utsav{%
% Our central question is whether a LLM agent can learn to solve
% unfamiliar, interaction-dependent tasks through active experimentation and
% in-context skill accumulation, with no weight updates. Answering it cleanly
% requires a benchmark domain with three properties: \textbf{(i)}~tasks whose
% solution cannot be read off a static description and must instead be discovered
% by interacting with the environment; \textbf{(ii)}~a controllable difficulty
% range, spanning levels current models already solve and levels they almost
% never solve, so that headroom is unambiguous; and \textbf{(iii)}~a programmatic
% interface that lets the agent inspect the scene, test interventions, and
% observe intermediate dynamics, so that experimentation is actually possible.
% We introduce \textsc{\textsc{Interphyre}} as a domain built to satisfy all three, and
% use it to study how and why frontier and small open LLMs under-perform, and how
% \textsc{HExA}, which combines in-context RL with autonomous skill evolution and
% consolidation, closes that gap by learning through interaction.}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/interventions_example.pdf}
  \caption{\textbf{\textsc{Interphyre}'s snapshot/restore API.} This branches a shared mid-trajectory state into a
    factual rollout and perturbed alternatives (Section \ref{sec:snapshot-restore}).
    Each row is one seed of the \texttt{catapult} level with a different oracle solution
    strategy.
    The leftmost column shows the initial scene for reference; the teal curve is the
    green ball's trajectory, shown up to the branch point in the \emph{Branch point}
    column and continuing through the outcome in each subsequent column.
    Top (seed\,8, deflector strategy): removing the deflector causes failure; shrinking
    the red action ball does not.
    Bottom (seed\,5, direct-launch strategy): shrinking the red ball causes failure;
    removing the deflector does not.
    The same interventions have opposite causal relevance across seeds, showing that causal
    relevance is a property of an object relative to the active strategy, not of the object
    in isolation.
    See Section \ref{sec:worked-example} for the branching protocol.}
  \label{fig:intervention-example_main_paper}
\end{figure}

\subsection{\textsc{Interphyre}: A Testbed for Learning through Experimentation}
\label{sec:Interphyre_example}



% As we defined in Sections \ref{sec:intro} and \ref{sec:HExA}, we develop methods to enable LLM agents to generally act reason and answer queries in and about new unseen domains via active experimentation, something even current frontier LLMs severely lack. We thus introduce \textsc{\textsc{Interphyre}} as the experimental testbed for studying agent learning through active experimentation.










% \begin{wraptable}{r}{0.58\linewidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{%
%   \textsc{ReAct} baseline solve rate~(\%) across eight
%   \textsc{Interphyre} levels.
%   Levels grouped by difficulty tier based on Claude Sonnet performance.
%   \textsuperscript{$\dagger$}Evaluated on 50 seeds;
%   \textsuperscript{$\ddagger$}25 seeds;
%   all others 100 seeds.
%   --- = not evaluated.
% }
% \label{tab:baseline_results}
% \begin{tabular}{lcccccc}
% \toprule
% & \textbf{Rand} & \textbf{Q-7B} & \textbf{Q-14B}
% & \textbf{O-20B} & \textbf{O-120B} & \textbf{Son.} \\
% \midrule
% \multicolumn{7}{l}{\textit{Tier~1: Solvable}} \\
% Cliffhanger      & 0  & 2.0  & 6.0  & 30.5 & 64.0 & 100$^{\ddagger}$ \\
% Tipping Point    & 3  & 24.0 & 42.0 & 80.0 & 90.1 & 96$^{\ddagger}$  \\
% Basket Case      & 4  & 8.0  & 10.0 & 14.0 & 33.0 & 100$^{\ddagger}$ \\
% Down to Earth    & 8  & 62.0 & 72.0 & 35.0 & 72.5 & 100             \\
% Two Body         & 14 & 18   & 24.0 & 26.0 & 77.8 & 100             \\
% Falling in Place & 1  & 20.0 & 52.0 & 58.0 & 100  & 100$^{\dagger}$ \\
% \addlinespace[2pt]
% \multicolumn{7}{l}{\textit{Tier~2: Hard}} \\
% Pass the Parcel  & 0  & 7.8  & 9.8  & 16   & 22   & 24$^{\dagger}$  \\
% Catapult         & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 8$^{\dagger}$   \\
% \bottomrule
% \end{tabular}
% \end{wraptable}




Unlike benchmarks that primarily ask whether an agent can solve a task or answer a query, our setting requires an environment in which the agent can deliberately interact and gather evidence: inspecting the current instance, testing interventions, observing intermediate dynamics, diagnosing failures, and reusing what it learned across future seeds and levels in an experimentation loop. \textsc{Interphyre} provides this in a controlled 2D physics domain with continuous actions and long-horizon causal structure. Each task requires placing a red ball at $(x,y,r)$, after which the simulator evaluates whether the level-specific success predicate is achieved.

\textsc{Interphyre} builds on the level designs in the PHYRE benchmark \citep{bakhtin2019phyre} by introducing APIs for level editing, test-time interventions on environment parameters, and logging traces from the simulation. These APIs can be used to customize the benchmark for evaluating agents on unseen levels, or provided to an LLM for active experimentation. In particular, our experiments use the \textsc{Interphyre} API to expose a structured tool-calling interface for hypothesis testing via interventional scene inspection, partial simulation, full rollouts, contact logs, and level-specific geometric analysis, for example as shown in Figure \ref{fig:intervention-example_main_paper}. However, successful actions often depend on contact chains, lever mechanics, collision timing, and strategy-dependent dynamics. Even strong LLMs struggle to anticipate such interactions reliably during inference, particularly when only given the scene description. 

The traces recovered from \textsc{Interphyre} runs let us measure precisely whether an LLM agent merely guesses from parametric prior knowledge, or leverages the information provided through interactions and exploration to improve its performance in-context. \textsc{Interphyre} therefore serves as both a benchmark and a diagnostic environment for experimentation based methods such as \textsc{HExA}. We provide full details of the environment design, curriculum, tool API, observation modes, and prompts in Appendix~\ref{app:Interphyre} and \ref{app:systemprompts}.

















\subsection{Experimental Setup, Evaluations, and Baselines}
\label{sec:setup}




\setlength{\intextsep}{2pt}          % less vertical space above/below the float
\setlength{\columnsep}{10pt}         % gap between table and wrapped text

\begin{wraptable}{r}{0.58\linewidth}
\vspace{-\baselineskip}              % pull the table up toward the section top (optional)
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{3pt}
\caption{%
  \textsc{ReAct} baseline solve rate~(\%) across eight
  \textsc{Interphyre} levels.
  Underlined levels (Pass the Parcel, Catapult) form the harder tier,
  based on Claude Sonnet performance.
  \textsuperscript{$\dagger$}Evaluated on 50 seeds;
  \textsuperscript{$\ddagger$}25 seeds;
  all others 100 seeds.
  --- = not evaluated.
}
\label{tab:baseline_results}
\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} cccccc}
\toprule
& \textbf{Rand} & \textbf{Q-7B} & \textbf{Q-14B}
& \textbf{O-20B} & \textbf{O-120B} & \textbf{Son.} \\
\midrule
Cliffhanger             & 0  & 2.0  & 6.0  & 30.5 & 64.0 & 100$^{\ddagger}$ \\
Tipping Point           & 3  & 24.0 & 42.0 & 80.0 & 90.1 & 96$^{\ddagger}$  \\
Basket Case             & 4  & 8.0  & 10.0 & 14.0 & 33.0 & 100$^{\ddagger}$ \\
Down to Earth           & 8  & 62.0 & 72.0 & 35.0 & 72.5 & 100             \\
Two Body                & 14 & 18   & 24.0 & 26.0 & 77.8 & 100             \\
Falling in Place        & 1  & 20.0 & 52.0 & 58.0 & 100  & 100$^{\dagger}$ \\
\underline{Pass the Parcel} & 0  & 7.8  & 9.8  & 16   & 22   & 24$^{\dagger}$ \\
\underline{Catapult}        & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 8$^{\dagger}$  \\
\bottomrule
\end{tabular*}
\end{wraptable}



We evaluate five LLMs including frontier black box and small open LLMs---Claude Sonnet~4.6, Qwen-2.5-\{7B, 14B\} Instruct, GPT-OSS-\{20B,120B\}, and a random agent (samples action randomly within the coordinate box)---all with a maximum number of 25 turn iteration with \textsc{Interphyre} levels. We compare against three baselines: \emph{\textsc{ReAct}}~\citep{yao2023reactsynergizingreasoningacting}, which runs one Thought-Action-Observation trajectory per seed; \emph{Reflexion}~\citep{shinn2023reflexion}, which adds verbal self-reflection; and \emph{\textsc{Direct}}, a interaction free, tool usage free baseline to evaluate the base capability of the models. With the smaller models, we also include \emph{GRPO}~\citep{shao2024deepseekmath}, which fine-tunes Qwen-2.5-3B with a binary $\{0,1\}$ reward, making it the only method that updates model weights and compares directly against our training-free in-context framework, HExA. All methods on a given level are evaluated on the same 50 seeds, so comparisons are paired on identical instances (full details in Appendix~\ref{app:baselines}). In Table~\ref{tab:baseline_results} of Appendix \ref{app:results}, we organize the eight levels into two difficulty tiers based on frontier-model performance: Tier~1 (six levels, Claude Sonnet $\geq96\%$),  and Tier~2 (\texttt{pass\_the\_parcel} at $24\%$, \texttt{catapult} at $8\%$, with every open-weight model scoring $0\%$ on the latter). These two hard levels from Tier~2, where purely parametric reasoning is insufficient, are the primary testbed for \textsc{HExA}.


% \utsav{[Note: this paragraph already defines what we mean by ``hard levels''
% (Tier-2: Claude Sonnet $\le24\%$), which I reuse to answer Scott's
% ``how is hard defined'' comment in the H1 heading below.]}





\begin{figure}[t]
\centering
\setlength{\tabcolsep}{1.2pt}
\renewcommand{\arraystretch}{0.85}
% --- ReAct row ----------------------------------------------------------
{\footnotesize\itshape \textsc{ReAct} (25 iterations, FAILURE)}\\[1pt]
\begin{tabular}{@{}ccccccc@{}}
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step0.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step30.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step57.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step70.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step91.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step151.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/react_step193.png} \\[-1pt]
  {\scriptsize step 0} & {\scriptsize step 30} & {\scriptsize step 57} &
  {\scriptsize step 70} & {\scriptsize step 91} &
  {\scriptsize step 151} & {\scriptsize step 193} \\
\end{tabular}\\[6pt]
% --- HExA row -----------------------------------------------------------
{\footnotesize\itshape \textsc{HExA} (6 iterations, SUCCESS)}\\[1pt]
\begin{tabular}{@{}ccccccc@{}}
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step0.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step25.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step57.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step74.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step119.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step140.png} &
  \includegraphics[width=0.135\linewidth]{figures/sim_frames_seed45/hexa_step172.png} \\[-1pt]
  {\scriptsize step 0} & {\scriptsize step 25} & {\scriptsize step 57} &
  {\scriptsize step 74} & {\scriptsize step 119} &
  {\scriptsize step 140} & {\scriptsize step 172} \\
\end{tabular}
% \caption{%
%   % Sparsified simulation frames for catapult seed 45, time increasing
%   % left to right. Top row: the final \textsc{ReAct} attempt
%   % (placement $(x{=}0.5,\,y{=}-1.0,\,r{=}2.0)$ from step~25 of the
%   % transcript) ends without a green--blue contact and the trial expires.
%   % Bottom row: \textsc{HExA}'s successful $(0.3, 0.9, 1.5)$ placement;
%   % the lever flings the green ball over the ceiling-blocker and into
%   % the basket where it makes the required 3-second contact with the
%   % blue ball. \scott{is there a one sentence insight as to why Hexa succeeds here? For example one or more skills it found that helped it , etc?}
%   % \utsav{[Addressed: qualitative insight, verified against the seed-45
%   % transcript and the round-14 skill bank.]
%   \textbf{Qualitative Comparing of solutions strategies from \textsc{ReAct} and \textsc{HExA}.} \textsc{HExA} succeeds by reusing strategies distilled from earlier catapult episodes: its skill bank already knows how to launch (drop a heavy ball on the arm to fling the green ball toward the basket) and how to fix the usual failure (when the shot arcs too high and hits the ceiling, shift the drop point sideways to flatten it instead of adding force). So after one ceiling overshoot it applies the learned correction and solves the level on its next try, whereas \textsc{ReAct}, with no memory or skill bank, exhausts its budget searching redundant placements and never finds the fix.}
%}
\caption{%
\textbf{How the evolved skill bank guides HExA on \texttt{catapult} seed~45.}
Top: \textsc{ReAct}, which has no cross-episode memory, exhausts its
25-iteration budget while repeatedly exploring ineffective placements.
Bottom: \textsc{HExA} begins with the evolved bank summarized above. After
observing that its initial launch strikes the ceiling, it applies the bank's
diagnosis that the limiting factor is launch geometry rather than insufficient
force. It therefore shifts the drop point toward $x=0.3$ instead of further
increasing the radius, and succeeds with
$(x,y,r)=(0.3,0.9,1.5)$ in six interaction iterations. Frames are sampled from
the final simulations; full prompts, bank entries, and trajectories are
provided in Appendix~\ref{app:trajectories:bank}.}
\label{fig:catapult45_simframes}
\end{figure}





\begin{figure}[b]
\centering
\begin{minipage}[c]{0.50\linewidth}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{lcc}
  \toprule
  \textbf{Method} & \textbf{Acc.\ (\%)} & \textbf{Avg Iter} \\
  \midrule
  \textsc{Direct} (no tools)    & \phantom{0}2.0           & \phantom{0}1.0          \\
  \textsc{ReAct}                & \phantom{0}8.0           & 22.9                    \\
  Reflexion ($K{=}2$)           & $21.3{\pm}2.5$           & $21.2{\pm}0.7$          \\
  \textsc{HExA} (no reward)     & $50.7{\pm}9.4$           & $16.5{\pm}2.7$          \\
  \textsc{HExA} (Off2On Evol.)  & $\mathbf{67.3{\pm}9.3}$  & $14.4{\pm}1.8$          \\
  \bottomrule
  \end{tabular}
\end{minipage}\hfill
\begin{minipage}[c]{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/catapult_three_methods_50seeds.pdf}
\end{minipage}
% \caption{%
%   %==== from the table caption (comments preserved) ====
%   \scott{Say what this experiment is testing and what should be the takeaway? Dont make reader think too hard - interpret for them. Reader should be able to understand experiemnt without referring to main text (at least basics)}
%   \utsav{[Addressed: compact self-contained caption --- one line on what is
%   tested, one line interpreting the result, methods named briefly; full
%   protocol moved to Appendix~\ref{app:baselines}.]}
%   \textbf{Skill accumulation on \texttt{catapult}, our hardest level
%   (Claude Sonnet, $50$ seeds).}
%   We test whether distilling past interaction trajectories into a reusable,
%   evolving skill bank (\textsc{HeXA}) helps on a level where a strong model
%   solves only $8\%$ of instances with a standard \textsc{ReAct} loop.
%   \textsc{HeXA} reaches $67.3\%$, about $3\times$ the strongest baseline
%   (Reflexion, $21.3\%$) and far above \textsc{Direct} (no tools, $2.0\%$) and
%   \textsc{ReAct} ($8.0\%$), while needing fewer iterations per solve.
%   The \textsc{HeXA} (no reward) ablation, which removes reward weighting from
%   the distillation, falls to $50.7\%$, indicating that \emph{reward-guided}
%   skill accumulation, not extra interaction alone, drives the improvement.
%   \textsc{HeXA}, \textsc{HeXA} (no reward), and Reflexion report
%   mean $\pm$ std over $3$ runs; \textsc{Direct} and \textsc{ReAct} are single
%   runs. Baseline and protocol details are in Appendix~\ref{app:baselines}.
%   %==== from the figure caption (comments preserved) ====
%   \utsav{[Reworked per Scott: leads with a plain takeaway, then defines the
%   level and the three methods in one line each, so the figure can be read on
%   its own without the main text.]}
%   \textbf{(Right)} \textbf{On \texttt{catapult}, our hardest level, \textsc{HExA}'s gains come
%   from reward-guided skill accumulation, not from extra interaction or
%   self-reflection alone.}
%   We compare three agents on \texttt{catapult}, a puzzle that a strong model
%   (Claude Sonnet) solves only about $8\%$ of the time with a standard agent
%   loop: \textsc{HExA}, which turns each past attempt into a reusable skill
%   bank and weights skills by how well the attempt scored; \textsc{HExA}
%   (no reward), the same method but treating all attempts equally; and
%   Reflexion, which only writes a verbal self-critique between two attempts.
%   The curves show the cumulative success rate as $50$ seeds are evaluated
%   (solid line is the mean of $3$ runs, shaded band is $\pm 1$ std).
%   \textsc{HExA} finishes at $67.3\%$, well above Reflexion at $21.3\%$, and
%   removing the reward weighting lowers it to $50.7\%$, a drop of about
%   $17$~pp. This tells us that scoring and reusing skills, rather than simply
%   interacting more or reflecting in words, is what drives the improvement,
%   and because the curves stay separated throughout the sweep the ranking is
%   not an artifact of a few lucky seeds.
% }
\caption{%
  \textbf{Reward-guided skill accumulation makes \textsc{HExA} much stronger on
  \texttt{catapult}, the hardest level.}
  This experiment tests whether an agent can improve by turning past attempts
  into reusable, reward-weighted skills. On \texttt{catapult}, Claude Sonnet solves
  only $8.0\%$ of seeds with a standard \textsc{ReAct} loop, while \textsc{HExA}
  reaches $67.3\%$ and uses fewer iterations per solve.
  \textbf{Left:} final solve rate and average iterations.
  \textbf{Right:} cumulative success over $50$ seeds; curves show mean over
  $3$ runs with shaded $\pm 1$ std.
  Removing reward weighting drops \textsc{HExA} to $50.7\%$, and Reflexion reaches
  only $21.3\%$, showing that the main gain comes from scoring and reusing skills,
  not merely from extra interaction or verbal self-reflection.
  Full protocol in Appendix~\ref{app:baselines}.
}
\label{tab:catapult_skillrl}
\label{fig:catapult_three_methods_50seeds}
\end{figure}




\subsection{Results and Analysis}
% \scott{Section needs to be reorganised. Eac hsubsection should introduce an experiment in the following order : 1) A hypothesis 2) The setup and how it will test the hypothesis 3) Results. Instead you are leading with the result.}
% \utsav{[Addressed: every subsection below now opens with an explicit
% \textbf{Hypothesis}, then \textbf{Setup} (what is varied and how it tests the
% hypothesis), then \textbf{Result} with the takeaway. I kept the original
% takeaway-first text struck through where it was replaced so the change is
% visible.]}
We design our experiments and ablations to investigate some specific research questions about the the efficacy and generalizability of \textsc{HExA} in these learning from experimentation settings compared to the base models.







% \paragraph{On the hardest levels, accumulating reusable skills beats agent-side baselines.} On the two Tier-2 levels, \texttt{catapult} ($8\%$ \textsc{ReAct}) and \texttt{pass\_the\_parcel} ($24\%$ \textsc{ReAct}), a frontier model fails under a single \textsc{ReAct} trajectory, so we expect that turning interaction traces into an evolving skill bank will yield substantially higher solve rates than baselines that do not accumulate reusable skills (\textsc{Direct}, \textsc{ReAct}, Reflexion). We test this by running all methods on the same $50$ seeds per level with Claude Sonnet under an identical $25$-iteration \textsc{ReAct} harness, with \textsc{HExA} in its default Off2On Evolving configuration ($x{=}3$ seeds per round); \textsc{HExA} and Reflexion are repeated over $3$ independent runs (mean~$\pm$~std) while \textsc{Direct} and \textsc{ReAct} are deterministic single runs, and we record both solve rate and the average number of iterations per seed as an efficiency proxy. The results bear this out: \textsc{HExA} turns both levels from mostly unsolved one-episode problems into substantially solvable in-context learning tasks, reaching $67.3 \pm 9.3\%$ on \texttt{catapult} against $2.0\%$ (\textsc{Direct}), $8.0\%$ (\textsc{ReAct}), and $21.3 \pm 2.5\%$ (Reflexion), and $60.0\%$ on \texttt{pass\_the\_parcel} against $24.0\%$ (\textsc{ReAct}) and $0.0\%$ (\textsc{Direct}) (Tables~\ref{tab:catapult_skillrl},~\ref{tab:ptp_variants}). The advantage is not confined to final accuracy: average iterations fall from $22.9$ (\textsc{ReAct}) and $21.2$ (Reflexion) to $14.4 \pm 1.8$, roughly $37\%$ fewer, indicating that the evolving bank makes each episode genuinely easier rather than merely raising the chance of a lucky placement (Figure~\ref{fig:catapult_three_methods_50seeds}). Reflexion, which adds verbal self-reflection but keeps no persistent bank, trails \textsc{HExA} by $46$~pp---evidence that the gain comes from reusing distilled skills, not from extra trials.









% Our first hypothesis is that on the two Tier-2 levels, \texttt{catapult}
% ($8\%$ \textsc{ReAct}) and \texttt{pass\_the\_parcel} ($24\%$ \textsc{ReAct}),
% where a frontier model fails under a single \textsc{ReAct} trajectory, turning
% interaction traces into an evolving skill bank should yield substantially
% higher solve rates than agent-side baselines that do not accumulate reusable
% skills (\textsc{Direct}, \textsc{ReAct}, and Reflexion). To test this, we run
% all four methods on the same $50$ seeds per level with Claude Sonnet under an
% identical $25$-iteration \textsc{ReAct} harness, with \textsc{HExA} in its
% default Off2On Evolving configuration ($x{=}3$ seeds per round); we repeat
% \textsc{HExA} and Reflexion over $3$ independent runs and report
% mean~$\pm$~std, while \textsc{Direct} and \textsc{ReAct} are deterministic
% single runs, and we record both solve rate and the average number of
% \textsc{ReAct} iterations per seed as an efficiency proxy. The results support
% the hypothesis: \textsc{HExA} turns both hard levels from mostly unsolved
% one-episode problems into substantially solvable in-context learning tasks. On
% \texttt{catapult} it reaches $67.3 \pm 9.3\%$ success, compared with $2.0\%$
% for \textsc{Direct}, $8.0\%$ for \textsc{ReAct}, and $21.3 \pm 2.5\%$ for
% Reflexion (Table~\ref{tab:catapult_skillrl}), and Figure~\ref{fig:catapult45_simframes}
% shows a representative seed where \textsc{HExA} solves the task in a handful of
% iterations by reusing previously distilled placement heuristics, while
% \textsc{ReAct} exhausts its budget without finding a working launch. The
% advantage is not confined to final accuracy: \textsc{HExA} also lowers the
% average number of iterations from $22.9$ (\textsc{ReAct}) and $21.2 \pm 0.7$
% (Reflexion) to $14.4 \pm 1.8$, a reduction of roughly $37\%$, which suggests
% that the evolved skill bank makes each new episode genuinely easier rather than
% simply raising the chance of a lucky placement. Figure~\ref{fig:catapult_three_methods_50seeds}
% plots cumulative success with $\pm 1$~std bands across the three runs for
% \textsc{HExA}, \textsc{HExA} (no reward), and Reflexion, and shows that
% Reflexion trails both \textsc{HExA} variants by a wide margin, $46$~pp below
% full \textsc{HExA} and $29$~pp below \textsc{HExA} (no reward). Verbal
% self-reflection between trials therefore helps far less than converting past
% trajectories into an explicit, reusable skill bank, and this holds even when
% the reward signal is removed from the bank, a gap we examine more closely under (Section~\ref{sec:h3})..






























\paragraph{On the hard levels, accumulating reusable skills via HExA clearly outperforms other non-experimentation centric agent baselines.}
On the two Tier-2 levels, \texttt{catapult} ($8\%$ \textsc{ReAct}) and \texttt{pass\_the\_parcel}
($24\%$ \textsc{ReAct}), a frontier model fails under a single \textsc{ReAct} trajectory, so
turning interaction traces into an evolving skill bank should yield substantially higher solve
rates than agent-side baselines that do not accumulate reusable skills (\textsc{Direct},
\textsc{ReAct}, and Reflexion). We run all four methods on the same $50$ seeds per level with
Claude Sonnet under an identical $25$-iteration \textsc{ReAct} harness, with \textsc{HExA} in its
default Off2On Evolving configuration ($x{=}3$ seeds per round); we repeat \textsc{HExA} and
Reflexion over $3$ independent runs and report mean~$\pm$~std, while \textsc{Direct} and
\textsc{ReAct} are deterministic single runs, and we record both solve rate and the average
number of \textsc{ReAct} iterations per seed as an efficiency proxy. \textsc{HExA} turns both
hard levels from mostly unsolved one-episode problems into substantially solvable in-context
learning tasks: on \texttt{catapult} it reaches $67.3 \pm 9.3\%$ success, compared with $2.0\%$
for \textsc{Direct}, $8.0\%$ for \textsc{ReAct}, and $21.3 \pm 2.5\%$ for Reflexion
(Table~\ref{tab:catapult_skillrl}), and Figure~\ref{fig:catapult45_simframes} shows a
representative seed where \textsc{HExA} solves the task in a handful of iterations by reusing
previously distilled placement heuristics while \textsc{ReAct} exhausts its budget without
finding a working launch. 






\begin{figure}[h]
  \centering
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/catapult_var_cum_avg_iter.pdf}
    \subcaption{Catapult (25 seeds).}
    \label{fig:catapult_var_cum_iter}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/ptp_cum_avg_iter.pdf}
    \subcaption{Pass the Parcel (50 seeds).}
    \label{fig:ptp_cum_iter}
  \end{minipage}
  \caption{%
    \textbf{Cumulative average \textsc{ReAct} iterations per seed} for every \textsc{HExA}
    variant against the baseline (Claude Sonnet); lower is more efficient. On both levels the
    Off2On Evolving configuration converges to the lowest cost per seed, while the iterative and
    pure-online variants remain higher, indicating that \textsc{HExA}'s gains come from guiding
    search more efficiently with accumulated experience rather than from spending more
    computation per instance.
  }
  \label{fig:cum_iter_both}
\end{figure}






\paragraph{HExA helps amortize cost of learning from future exploration and experimentation.}The advantage is not confined to final accuracy: \textsc{HExA} also lowers the average number of iterations from $22.9$ (\textsc{ReAct}) and $21.2 \pm 0.7$
(Reflexion) to $14.4 \pm 1.8$, a reduction of roughly $37\%$, which suggests that the evolved
skill bank makes each new episode genuinely easier rather than simply raising the chance of a
lucky placement. Figure~\ref{fig:catapult_three_methods_50seeds} plots cumulative success with
$\pm 1$~std bands across the three runs for \textsc{HExA}, \textsc{HExA} (no reward), and
Reflexion, and shows Reflexion trailing both \textsc{HExA} variants by a wide margin---$46$~pp
below full \textsc{HExA} and $29$~pp below \textsc{HExA} (no reward). Verbal self-reflection
between trials therefore helps far less than converting past trajectories into an explicit,
reusable skill bank, and this holds even when the reward signal is removed from the bank, a gap
we examine more closely in Section~\ref{sec:h3}. We also plot the number of iterations needed to solve the tasks as we move to newer seeds of experiments in Figure \ref{fig:cum_iter_both}.






% \input{tables/ICMSRL_catapult_variants}






The same pattern appears on \texttt{pass\_the\_parcel}, where the best \textsc{HExA} configuration, Off2On Evolving with $x=3$ seeds per round, achieves $60.0\%$ success, compared to $24.0\%$ for \textsc{ReAct}, $16.0\%$ for Reflexion ($K{=}2$ trials, $8/50$ seeds), and $0.0\%$ for \textsc{Direct} (Table~\ref{tab:ptp_variants}). This level requires the agent to discover how to use the ramp-and-basket mechanism rather than simply choosing a direct collision. The improvement therefore supports the central claim of the paper: performance improves when interaction traces are distilled into reusable strategies and mistakes that subsequent episodes can condition on.


\begin{table}[h]
\centering
\small
\caption{%
  \textsc{HExA} on open-weight solvers, 50 training/evaluation seeds per cell
  (max 25 iterations). Qwen-2.5 runs use the Online-Evolving configuration ($k{=}3$ seeds
  per round, 17 rounds); GPT-OSS-120B uses Off2On Evolving. Baselines are the same agent with
  no skill injection. Per-seed cumulative trajectories in Figure~\ref{fig:hexa_smallmodels}.
}
\label{tab:hexa_smallmodels_main_paper}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{llcc}
\toprule
\textbf{Level} & \textbf{Method} & \textbf{Acc.\ (\%)} & \textbf{Avg Iters} \\
\midrule
\multirow{4}{*}{Down to Earth}
  & Qwen-2.5-3B \textsc{ReAct} & \phantom{0}8.0 & 23.8 \\
  & Qwen-2.5-3B \textsc{HExA}  & \textbf{24.0}  & 18.6 \\
  \cmidrule(lr){2-4}
  & Qwen-2.5-7B \textsc{ReAct} & 62.0           & 12.5 \\
  & Qwen-2.5-7B \textsc{HExA}  & \textbf{72.0}  & 12.6 \\
\midrule
\multirow{4}{*}{Two Body Problem}
  & Qwen-2.5-3B \textsc{ReAct} & \phantom{0}6.0 & 24.0 \\
  & Qwen-2.5-3B \textsc{HExA}  & \textbf{14.0}  & 21.1 \\
  \cmidrule(lr){2-4}
  & Qwen-2.5-7B \textsc{ReAct} & 18.0           & 22.2 \\
  & Qwen-2.5-7B \textsc{HExA}  & \textbf{34.0}  & 18.9 \\
\midrule
\multirow{2}{*}{Catapult}
  & GPT-OSS-120B \textsc{ReAct} & \phantom{0}0.0 & 25.0 \\
  & GPT-OSS-120B \textsc{HExA}  & \textbf{54.0}  & 16.2 \\
\bottomrule
\end{tabular}
\end{table}



Figure~\ref{fig:ptp_cum_accuracy} shows that the gain is not caused by a small number of lucky seeds. The cumulative success curve for Off2On Evolving remains consistently above the \textsc{ReAct} baseline and finishes at $60.0\%$. Its cumulative iteration curve also converges below the baseline, showing that \textsc{HExA} is not simply spending more computation per instance; it is using previous interaction experience to guide future search more efficiently. Across open-weight LLM agents, \textsc{HExA} consistently improves over the corresponding baselines, with gains ranging from $+8$ to $+54$ percentage points across Qwen-2.5 and GPT-OSS models; we provide these detailed experiments in Table \ref{tab:hexa_smallmodels_main_paper} and Appendix section \ref{sec:h2}.




















% \paragraph{\textsc{HExA} outperforms agent-side baselines on the hardest levels for a frontier solver.\scott{How is this determined/defined ?}}
% \label{sec:h1}
% \utsav{[Addressed Scott's ``how is hard defined'' comment: ``hardest levels''
% now refers explicitly to the two Tier-2 levels (\texttt{catapult},
% \texttt{pass\_the\_parcel}), where the frontier \textsc{ReAct} baseline scores
% $\le24\%$. Reorganised to Hypothesis $\to$ Setup $\to$ Result.]}


% \sout{The first result is that \textsc{HExA} turns the hardest
% \textsc{\textsc{Interphyre}} levels from mostly unsolved one-episode
% reasoning problems into substantially solvable in-context
% learning tasks.
% On \texttt{catapult}, \textsc{HExA} reaches
% $67.3 \pm 9.3\%$ success across $3$ independent runs of the
% full $50$-seed evaluation,  compared to $2.0\%$ for \textsc{Direct},
% $8.0\%$ for \textsc{ReAct}, and $21.3 \pm 2.5\%$ for Reflexion (also $3$ runs; Table~\ref{tab:catapult_skillrl}).
% Figure~\ref{fig:catapult45_simframes} illustrates a
% representative case: \textsc{HExA} solves the seed in fewer
% iterations by leveraging previously distilled placement
% heuristics, while \textsc{ReAct} exhausts its iteration budget
% without finding the correct launch configuration.
% The gain extends beyond final accuracy to per-episode efficiency:
% \textsc{HExA} reduces average iterations from $22.9$
% (\textsc{ReAct}) and $21.2 \pm 0.7$ (Reflexion) to
% $14.4 \pm 1.8$, a ${\sim}37\%$ reduction, indicating that the
% evolved skill bank makes each new episode genuinely easier to
% solve, rather than merely increasing the probability of a lucky
% placement.
% Figure~\ref{fig:catapult_three_methods_50seeds} shows cumulative
% success curves with $\pm 1$~std bands across the $3$ runs for
% \textsc{HExA}, \textsc{HExA} (no reward), and Reflexion.
% Reflexion trails both \textsc{HExA} variants by a wide margin:
% $46$~pp below full \textsc{HExA} and $29$~pp below \textsc{HExA}
% (no reward).
% In other words, verbal self-reflection between trials helps
% much less than turning past trajectories into an explicit, reusable
% skill bank, and this remains true even when we strip the reward
% signal out of the bank.
% We look more closely at the gap between \textsc{HExA} and
% \textsc{HExA} (no reward) in Section~\ref{sec:h3}.}




% \newpage
















\paragraph{What Drives the Self-Improvement in HExA - Rewards Guidance from Environment Interactsions \& Experimentation and Evolution of Skills.}
\label{sec:h3}
% \scott{This is closer to a hypothesis to test . (good, just needs a bit of reorganisation to the format I mentioned}
% \utsav{[Addressed: heading restated as a hypothesis and the subsection
% reorganised into Hypothesis $\to$ Setup $\to$ Result. Original title was
% ``What Drives the Self-Improvement in HExA --- Rewards Guidance \ldots''.]}
% \sout{We isolate the contribution of reward-weighted distillation by
% ablating the reward signal from the evolver. Without reward
% weighting, where every success is treated equally and every
% failure equally, \textsc{HExA}'s gain over the \textsc{ReAct}
% baseline shrinks substantially
% (Table~\ref{tab:reward_ablation}).
% On \texttt{down\_to\_earth} (DTE), the no-reward variant reaches
% $64\%$ (only $+2$~pp over the baseline) while the full system
% achieves $72\%$ ($+10$~pp); on \texttt{two\_body\_problem} (TBP), the
% gap is $26\%$ versus $34\%$ ($+8$~pp difference between
% variants).
% These results indicate that reward calibration is load-bearing:
% it helps the evolver distinguish merely successful trajectories
% from efficiently solved ones, producing skills that are more
% reusable and informative.
 
% The comparison across \textsc{HExA} configurations in Table~\ref{tab:ptp_variants} further illuminates two additional design axes. First, \emph{cross-episode skill accumulation} is critical: evolving variants ($58$--$60\%$) consistently outperform both the offline-frozen bank ($48\%$) and the \textsc{ReAct} baseline ($24\%$), confirming that iteratively refining skills with new evidence produces meaningfully better strategies than a one-shot distillation. Second, the \emph{choice of initialisation} matters: Off2On Evolving ($60\%$) slightly outperforms Pure Online Evolving ($58\%$), suggesting that a warm-start batch provides a useful bootstrap, though the difference is modest once online evolution takes over.} \scott{"load-bearing" is AI giveaway}



\begin{wraptable}[11]{r}{0.45\linewidth}
\vspace{-8pt}
\centering
\scriptsize
\caption{%
  Reward-signal ablation on Qwen-2.5-7B, 50 seeds per cell.
  Full \textsc{HExA} uses reward-weighted, two-pass distillation;
  the no-reward variant treats successful trajectories equally.
}
\label{tab:reward_ablation}
\begin{tabular}{@{}llcc@{}}
\toprule
\textbf{Level} & \textbf{Method}
  & \textbf{Acc.\ (\%)}
  & \textbf{Iters} \\
\midrule
\multirow{3}{*}{Down to Earth}
  & \textsc{ReAct}              & 62.0          & 12.5 \\
  & \textsc{HExA} no reward     & 64.0          & 14.8 \\
  & \textsc{HExA} reward        & \textbf{72.0} & 12.6 \\
\midrule
\multirow{3}{*}{Two Body}
  & \textsc{ReAct}              & 18.0          & 22.2 \\
  & \textsc{HExA} no reward     & 26.0          & 22.2 \\
  & \textsc{HExA} reward        & \textbf{34.0} & 18.9 \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{wraptable}

We first isolate the role of \emph{reward-weighted} distillation by ablating
the reward signal in the evolver, so that every success and every failure is
treated equally regardless of how efficiently it was reached. On the two open-weight Qwen levels this calibration accounts for most of \textsc{HExA}'s
gain: on \texttt{down\_to\_earth} the no-reward variant reaches only $64\%$
(just $+2$~pp over the \textsc{ReAct} baseline) while full \textsc{HExA} reaches
$72\%$ ($+10$~pp), and on \texttt{two\_body\_problem} the no-reward variant reaches $26\%$ against $34\%$ for the full system (Table~\ref{tab:reward_ablation}). 

The same effect appears with a frontier
solver on the hardest level: on \texttt{catapult}, removing the reward signal
lowers Claude Sonnet's accuracy from $67.3 \pm 9.3\%$ to $50.7 \pm 9.4\%$
(Figure~\ref{fig:catapult_three_methods_50seeds}). Reward calibration is
therefore central to the gain rather than incidental, because it lets the
evolver separate efficiently solved trajectories from merely successful ones,
so the skills it keeps and refines are the more reusable and informative ones. 







The second mechanism is \emph{cross-episode skill accumulation}, which we isolate by sweeping the bank's initialisation and per-round update strategy. Evolving the bank across rounds is consistently better than distilling it once: on \texttt{pass\_the\_parcel} the evolving variants reach $58$--$60\%$ versus $48\%$ for a frozen offline bank and $24\%$ for \textsc{ReAct} (Table~\ref{tab:ptp_variants}). The same ordering also holds on \texttt{catapult}, where Off2On Evolving reaches $76\%$ against $60\%$ for the frozen offline bank, $56\%$ and $36\%$ for the iterative variants, and $20\%$ for Reflexion, pulling further ahead as more seeds are seen (Figure~\ref{fig:cum_accuracy_both}; full per-configuration breakdown in Appendix Table~\ref{tab:catapult_variants}).
% and the same ordering holds on \texttt{catapult}, where the evolving configuration climbs well above the iterative and offline banks as more seeds are seen (Figure~\ref{fig:catapult_variants}). 
The cumulative-accuracy curves on both levels (Figures~\ref{fig:ptp_cum_accuracy} and \ref{fig:catapult_var_cum_accuracy}) make the mechanism visible: the evolving variants pull steadily away from the others as the skill bank is refined with each new round of evidence, instead of plateauing like a one-shot distillation. Initialization matters only modestly by comparison: an off-to-online warm start
($60\%$ on \texttt{pass\_the\_parcel}) edges out pure online evolution ($58\%$), which suggests a warm-start batch provides a useful bootstrap whose advantage shrinks once online evolution takes over.


% \newpage


\begin{wraptable}{l}{0.45\linewidth}
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{%
  \textsc{HExA} variant accuracy (\%) on the two hard levels (Claude Sonnet;
  \textbf{Cat.}~=~\texttt{catapult}; \textbf{PtP}~=~\texttt{pass\_the\_parcel}). Off2On Evolving ($x{=}3$), referred to simply as \textsc{HExA}, is best on both.}
\label{tab:variants_compact}
\begin{tabular}{lcc}
\toprule
\textbf{Configuration} & \textbf{Cat.} & \textbf{PtP} \\
\midrule
Off2On Evolving (HExA) & \textbf{76.0} & \textbf{60.0} \\
Off2On Iterative       & 56.0          & 48.0          \\
Online Evolving        & 44.0          & 58.0          \\
Online Iterative       & 36.0          & 56.0          \\
Offline Static         & 60.0          & 48.0          \\
\bottomrule
\end{tabular}
\end{wraptable}



As we can clearly see in Table \ref{tab:variants_compact}, \textit{Off2On~+~Evolution}---which performs the best, is the setup we finally use in \textsc{HExA}
hereafter. It wins by combining a broad prior with cumulative refinement: the warm start
distills a large, diverse offline batch sampled \emph{before} the bank biases active experimentation and
exploration, giving the contrastive distillation wide success/failure contrast,
and Evolution then compounds this knowledge across rounds rather than relearning it.
The two ablations isolate each ingredient. Holding the update rule at Evolution, the
warm start (Off2On, 76\%/60\% on \texttt{catapult}/\texttt{pass\_the\_parcel}) beats the cold start (Pure Online, 44\%/58\%)---most sharply on \texttt{catapult}---because
a cold start spends its early rounds rediscovering basic strategies from a few
correlated trajectories. Holding initialization at Off2On, Evolution (76\%/60\%)
beats Iterative Replacement (56\%/48\%), since re-distilling from scratch each round
discards accumulated skills and amplifies drift.





% \utsav{[Added: \texttt{reward\_ablation} table is now \texttt{\textbackslash input}
% here since the paragraph above references it.]}
% \input{tables/reward_ablation}



\paragraph{Are Evolved and Consolidated Skills Generalizable and Reusable Across Unseen Levels?}
\label{sec:h4}

A natural question is whether the skills \textsc{HExA} distills encode genuinely reusable physics primitives or are merely level-specific recipes. We test this by synthesizing skill banks for unseen target levels using only source-level banks and a textual description of the target, no target-level trajectories are generated at any stage.
 % \paragraph{Multi-source transfer (Claude Sonnet).}

% \newpage
\begin{wrapfigure}[14]{l}{0.56\linewidth}
  \vspace{-10pt}
  \centering
  \includegraphics[width=\linewidth]{figures/cross_level_transfer.pdf}
  \caption{%
    Cross-level skill transfer with no target trajectories. Each target is solved using only skills synthesised from source-level banks; labels report target success and matched \textsc{ReAct} baselines.Multi-source transfer to \texttt{catapult} yields the largest gain
    ($+36$~pp).
  }
  \label{fig:cross_level_transfer}
  \vspace{-12pt}
\end{wrapfigure}





Combining fully-evolved banks from three source levels (\texttt{down\_to\_earth}, \texttt{two\_body\_problem}, \texttt{pass\_the\_parcel}), the evolver synthesises a cross-level bank for \texttt{catapult}. Injecting this bank with no further evolution increases the accuracy of \texttt{catapult} from $8.0\%$ to $44.0\%$ ($+36$~pp), closing roughly $60\%$ of the gap to the within-level \textsc{HExA} result of $64\%$ (Table~\ref{tab:cross_level}).
This confirms that the lever-launch dynamics of \texttt{catapult} share structural primitives (collision normals, energy thresholds, directional impulse) with the source levels.
 % \paragraph{Single-source transfer (Qwen-2.5-7B).}
Even with a single source bank and a smaller teacher, transfer yields positive gains.
On a structurally similar pair (\texttt{down\_to\_earth}~$\to$~\texttt{falling\_into\_place}), transfer gains $+12$~pp; on a dissimilar pair (\texttt{down\_to\_earth}~$\to$~\texttt{two\_body\_problem}), it still gains $+16$~pp (Table~\ref{tab:cross_level}). That transfer succeeds even across dissimilar levels suggests the evolver extracts abstract principles (e.g., momentum transfer, contact geometry) rather than narrow placement heuristics.


 
% \input{tables/cross_level_transfer}


% \input{figures/cross_level_transfer}



% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{/figures/hexa_smallmodels.pdf}
%     \caption{HExA shows consistent improvement on small open LLMs as well.}
%     \label{fig:hexa_smallmodels}
% \end{figure}














\input{figures/grpo_comparision_figure}


\paragraph{At a matched interaction budget, in-context \textsc{HExA} is more sample-efficient than gradient-based RL post-training with GRPO.}
\label{sec:h5}
When considering the comparison of \textsc{HExA} with parametric approaches, we compare with GRPO~\citep{shao2024deepseekmath} fine-tuning  Qwen-2.5-3B on the same levels. At a matched number of model updates and environment interactions of 50 unique seeds, GRPO reaches $20\%$ on \texttt{down\_to\_earth} and $6\%$ on \texttt{two\_body\_problem}, compared to \textsc{HExA}'s $24\%$ and $14\%$ (Figure~\ref{fig:grpo_comparison_main}). The gap reflects the core advantage of in-context RL and skill evolution methods like HExA: strategies distilled from early trajectories are immediately available to subsequent episodes via context, whereas gradient-based methods must accumulate signal over many rollouts before policy weights encode equivalent knowledge. This leads to much efficient learning in harder unseen domains where successful trajectories are hard to get initially where methods like HExA can still bootstrap learning vai skill evolution on failure or partial success trajectories.  We present more details of our ablations in Appendix~\ref{sec:h5}.















































==> tables/ICMSRL_catapult_result.tex <==
\begin{table}[t]
\centering
\small
\caption{%
\scott{Say what this experiment is testing and what should be the takeaway? Dont make reader think too hard - interpret for them. Reader should be able to understand experiemnt without referring to main text (at least basics)}
  \utsav{[Addressed: compact self-contained caption --- one line on what is
  tested, one line interpreting the result, methods named briefly; full
  protocol moved to Appendix~\ref{app:baselines}.]}
  \textbf{Skill accumulation on \texttt{catapult}, our hardest level
  (Claude Sonnet, $50$ seeds).}
  We test whether distilling past interaction trajectories into a reusable,
  evolving skill bank (\textsc{HeXA}) helps on a level where a strong model
  solves only $8\%$ of instances with a standard \textsc{ReAct} loop.
  \textsc{HeXA} reaches $67.3\%$, about $3\times$ the strongest baseline
  (Reflexion, $21.3\%$) and far above \textsc{Direct} (no tools, $2.0\%$) and
  \textsc{ReAct} ($8.0\%$), while needing fewer iterations per solve.
  The \textsc{HeXA} (no reward) ablation, which removes reward weighting from
  the distillation, falls to $50.7\%$, indicating that \emph{reward-guided}
  skill accumulation, not extra interaction alone, drives the improvement.
  \textsc{HeXA}, \textsc{HeXA} (no reward), and Reflexion report
  mean $\pm$ std over $3$ runs; \textsc{Direct} and \textsc{ReAct} are single
  runs. Baseline and protocol details are in Appendix~\ref{app:baselines}.
}
\label{tab:catapult_skillrl}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccc}
\toprule
\textbf{Method}
  & \textbf{Seeds}
  & \textbf{Acc.\ (\%)}
  & \textbf{Succ.} & \textbf{Fail}
  & \textbf{Avg Iter} \\
\midrule
\textsc{Direct} (one-shot, no tools) & 50 & \phantom{0}2.0 & \phantom{0}1 & 49 & \phantom{0}1.0 \\
\textsc{ReAct} baseline             & 50 & \phantom{0}8.0 & \phantom{0}4 & 46 & 22.9 \\
Reflexion ($K{=}2$ trials, 3 runs)  & 50 & $21.3 \pm 2.5$           & $10.7 \pm 1.2$ & $39.3 \pm 1.2$ & $21.2 \pm 0.7$ \\
\textsc{HeXA} (no reward, 3 runs)   & 50 & $50.7 \pm 9.4$ & $25.3 \pm 4.7$ & $24.7 \pm 4.7$ & $16.5 \pm 2.7$ \\
\textsc{HeXA} (Off2On Evol., $k{=}3$, 3 runs) & 50 & $\mathbf{67.3 \pm 9.3}$ & $33.7 \pm 4.6$ & $16.3 \pm 4.6$ & $14.4 \pm 1.8$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/ICMSRL_catapult_variants.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textsc{HeXA} configuration comparison on \texttt{catapult}
  (Claude Sonnet, 25 seeds for every method, sorted by accuracy).
  The five configurations cross two design axes: initialisation
  (\emph{Offline} / Off-to-Online \emph{(Off2On)} / pure \emph{Online})
  and per-round update (\emph{Static} / \emph{Iterative} re-distillation /
  \emph{Evolving} merge).
  The headline configuration --- Off2On Evolving with $x{=}3$ seeds per
  round --- is the one we refer to simply as \textsc{HeXA} elsewhere in
  the paper.
  Per-seed cumulative trajectories are shown in
  Figure~\ref{fig:catapult_variants}.
  The Reflexion ($K{=}2$ trials) baseline is reported below the
  configurations on the same $25$ seeds.
  Failures are counted as the iteration cap in the \emph{Avg Iter}
  column ($25$ for \textsc{HeXA} variants, $24$ for Reflexion).
}
\label{tab:catapult_variants}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llcccc}
\toprule
\textbf{Init} & \textbf{Update}
  & \textbf{Acc.\ (\%)}
  & \textbf{Succ.} & \textbf{Fail}
  & \textbf{Avg Iter} \\
\midrule
Off2On & Evolving ($x{=}3$)
  & \textbf{84.0} & 21 & \phantom{0}4 & 11.8 \\
Offline & Static
  & 60.0 & 15 & 10 & 17.0 \\
Off2On & Iterative
  & 56.0 & 14 & 11 & 15.7 \\
Online & Evolving ($x{=}3$)
  & 44.0 & 11 & 14 & 18.2 \\
Online & Iterative
  & 36.0 & \phantom{0}9 & 16 & 20.4 \\
\midrule
\multicolumn{2}{l}{Reflexion ($K{=}2$ trials)}
  & 20.0 & \phantom{0}5 & 20 & 22.3 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/ICMSRL_results.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textsc{HeXA} configuration comparison on \texttt{pass\_the\_parcel}
  (Claude Sonnet, 50 seeds for every method, sorted by accuracy).
  The five configurations cross two design axes: initialisation
  (\emph{Offline} / Off-to-Online \emph{(Off2On)} / pure \emph{Online})
  and per-round update (\emph{Static} / \emph{Iterative} re-distillation /
  \emph{Evolving} merge).
  The headline configuration --- Off2On Evolving with $x{=}3$ seeds per
  round --- is the one we refer to simply as \textsc{HeXA} elsewhere in
  the paper.
  Per-seed cumulative trajectories are shown in
  Figure~\ref{fig:ptp_cum_accuracy}.
  The \textsc{Direct} baseline (one scripted scene read + one Claude call,
  no simulator feedback) is reported below \textsc{ReAct} for reference;
  its \emph{Avg Iter} column reports the single committed model call per
  seed.
  Reflexion ($K{=}2$ trials with verbal self-reflection between trials) is
  reported below \textsc{ReAct}; the placeholder cells (\textendash) will
  be filled in once the full 50-seed run completes.
}
\label{tab:ptp_variants}
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{llccccc}
\toprule
\textbf{Init} & \textbf{Update}
  & \textbf{Acc.\ (\%)}
  & \textbf{Succ.} & \textbf{Fail}
  & \textbf{Avg Iter}
  \\
\midrule
Off2On & Evolving ($x{=}3$) (HeXA)
  & \textbf{60.0} & 30 & 20 & 17.3  \\
Online & Evolving ($x{=}3$)
  & 58.0 & 29 & 21 & 16.4  \\
Online & Iterative
  & 56.0 & 28 & 22 & 18.7  \\
Off2On & Iterative
  & 48.0 & 24 & 26 & 17.0  \\
Offline & Static
  & 48.0 & 24 & 26 & 18.4  \\
\midrule
\multicolumn{2}{l}{\textsc{ReAct} baseline}
  & 24.0 & 12 & 38 & 21.3  \\
% TODO: fill in Succ/Fail/Avg Iter/Time once the full 50-seed Reflexion-PTP run lands.
\multicolumn{2}{l}{Reflexion ($K{=}2$ trials)}
  & 16 & 8 & 42 & 22.4  \\
\multicolumn{2}{l}{\textsc{Direct} (one-shot, no tools)}
  & \phantom{0}0.0 & \phantom{0}0 & 50 & \phantom{0}1.0  \\
\bottomrule
\end{tabular}
\end{table}


==> tables/baseline_results.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textsc{ReAct} baseline solve rate~(\%) across eight
  \textsc{Interphyre} levels.
  Levels grouped by difficulty tier based on Claude Sonnet performance.
  \textsuperscript{$\dagger$}Evaluated on 50 seeds;
  \textsuperscript{$\ddagger$}25 seeds;
  all others 100 seeds.
  --- = not evaluated.
}
\label{tab:baseline_results}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccc}
\toprule
& \textbf{Random} & \textbf{Qwen-7B} & \textbf{Qwen-14B}
& \textbf{OSS-20B} & \textbf{OSS-120B} & \textbf{Sonnet} \\
\midrule
\multicolumn{7}{l}{\textit{Tier~1: Solvable levels}} \\
\addlinespace[2pt]
\quad Cliffhanger
  & 0 & 2.0 & 6.0 & 30.5 & 64.0 & 100$^{\ddagger}$ \\
\quad Tipping Point
  & 3 & 24.0
  & 42.0 & 80.0 & 90.1 & 96$^{\ddagger}$ \\
\quad Basket Case
  & 4 & 8.0 & 10.0 & 14.0 & 33.0 & 100$^{\ddagger}$ \\
\quad Down to Earth
  & 8 & 62.0 & 72.0 & 35.0 & 72.5 & 100 \\
\quad Two Body
  & 14 & 18 & 24.0 & 26.0 & 77.8 & 100 \\
\quad Falling in Place
  & 1 & 20.0 & 52.0 & 58.0 & 100 & 100$^{\dagger}$ \\
\addlinespace[4pt]
\multicolumn{7}{l}{\textit{Tier~2: Hard levels}} \\
\addlinespace[2pt]
\quad Pass the Parcel
  & 0 & 7.8 & 9.8 & 16 & 22
  & 20$^{\dagger}$ \\
\quad Catapult
  & 0 & 0.0 & 0.0 & 0.0 & 0.0
  & 11 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/benchmark_grid.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textbf{Four benchmark families.} \emph{Tasks} counts the task/level settings
  with a paired no-memory arm. \emph{Actor} is the frozen model that acts;
  \emph{Evolver} is the model that distils skills, and is the same model
  everywhere except the \textsc{InterPhyre} Claude runs. \emph{Split} gives the
  training and held-out partitions.
}
\label{tab:benchmarks}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lllcc}
\toprule
\textbf{Family} & \textbf{Tasks} & \textbf{Actor} & \textbf{Split (train / eval)} & \textbf{$n$/arm} \\
\midrule
\textsc{InterPhyre}      & 4 levels & Claude Sonnet 4.6, Qwen-2.5-\{3B,7B\},   & 51 / 50 & 50 \\
                         &          & GPT-OSS-120B                            &                       &    \\
Interactive games        & 2 games  & \texttt{gpt-oss-120b}, Qwen3-8B         & 80 / 40 (Mastermind)  & 40 \\
                         &          &                                         & 200 / 243 (Maze)      & 243\\
Reasoning \& planning     & 4 tasks  & \texttt{gpt-oss-120b}                   & 60 items / 100 held-out & 100 \\
\textsc{DiscoverPhysics} & 3 worlds & \texttt{claude-sonnet-5}                & 9 worlds / held-out world & 15 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/catapult_memory.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textbf{A distilled bank beats storing the experience itself, at a fraction of
  the context.} \textsc{InterPhyre} \texttt{catapult} with a Claude Sonnet 4.6
  actor; every arm is scored with its memory frozen on the same held-out pool of
  50 seeds. Episodic RAG retrieves past rollouts verbatim and MemRL maintains
  (intent, experience, utility) triplets, so both carry raw experience forward,
  while \textsc{HExA} carries a distilled bank. \emph{Success} is the percentage
  of seeds solved, $\pm$ one standard deviation over three independently built
  memories. \emph{Tokens/ep.}\ is the mean memory block injected into the
  actor's prompt each episode and \emph{Range} its minimum and maximum,
  excluding the task prompt and the accumulated transcript. \textsc{HExA}'s bank
  is fixed at 10 skills and 5 mistakes, so its cost is constant in the number of
  episodes played; the episodic baselines inject whole rollouts, so their cost
  scales with the rollout cap rather than with anything learned. Bold marks the
  best value in each column.
}
\label{tab:catapult_memory}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcrc}
\toprule
\textbf{Method} & \textbf{Success (\%)} & \textbf{Tokens/ep.} & \textbf{Range} \\
\midrule
\textbf{\textsc{HExA}} (frozen bank) & \textbf{82.7} {\scriptsize$\pm$11.4} & \textbf{2{,}392} & 1{,}854--2{,}907 \\
Episodic RAG                         & 60.8 & 6{,}706 & 0--9{,}739 \\
MemRL (numeric key)                  & 33.3 & 8{,}135 & 0--12{,}211 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/hexa_smallmodels.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  HeXA on open-weight solvers, 50 training/evaluation seeds per cell.
  Qwen-2.5 runs use Online-Evolving configuration ($k{=}3$ seeds per round, 17 rounds).
  GPT-OSS-120B uses the same Off2On Evolving configuration. Baselines are the same agent without any skill
  injection. Per-seed cumulative trajectories are unchanged from the
  per-seed metric reported in Figure~\ref{fig:hexa_smallmodels}.
}
\label{tab:hexa_smallmodels}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llccc}
\toprule
\textbf{Level} & \textbf{Method}
  & \textbf{Acc.\ (\%)}
  & \textbf{Avg Iters (max 25)}
  & \textbf{$\Delta$ vs.\ baseline} \\
\midrule
\multirow{4}{*}{Down to Earth}
  & Qwen-2.5-3B \textsc{ReAct} baseline & \phantom{0}8.0 & 23.8 & --- \\
  & Qwen-2.5-3B \textsc{HeXA}            & \textbf{24.0}  & 18.6 & $+16.0$ \\
  & Qwen-2.5-7B \textsc{ReAct} baseline & 62.0           & 12.5 & --- \\
  & Qwen-2.5-7B \textsc{HeXA}            & \textbf{72.0}  & 12.6 & $+10.0$ \\
\midrule
\multirow{4}{*}{Two Body Problem}
  & Qwen-2.5-3B \textsc{ReAct} baseline & \phantom{0}6.0 & 24.0 & --- \\
  & Qwen-2.5-3B \textsc{HeXA}            & \textbf{14.0}  & 21.1 & $+8.0$ \\
  & Qwen-2.5-7B \textsc{ReAct} baseline & 18.0           & 22.2 & --- \\
  & Qwen-2.5-7B \textsc{HeXA}            & \textbf{34.0}  & 18.9 & $+16.0$ \\
\midrule
\multirow{2}{*}{Catapult}
  & GPT-OSS-120B \textsc{ReAct} baseline & \phantom{0}0.0 & 25.0 & --- \\
  & GPT-OSS-120B \textsc{HeXA}            & \textbf{54.0}  & 16.2 & $+54.0$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/icmsrl_qwen3b.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textsc{ICMSRL} on Qwen-2.5-3B with the evolving variant
  ($x{=}3$ seeds / round, 17 rounds), evaluated on seeds $6$--$55$
  (50 seeds, last training seed dropped to align with other tables).
  Baseline rows are the same Qwen-2.5-3B agent without any skill injection.
}
\label{tab:icmsrl_qwen3b}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llccc}
\toprule
\textbf{Level} & \textbf{Method}
  & \textbf{Acc.\ (\%)}
  & \textbf{Succ.\ / Total}
  & \textbf{$\Delta$} \\
\midrule
\multirow{2}{*}{Down to Earth}
  & \textsc{ReAct} baseline       & \phantom{0}6.0 & 3 / 50 & --- \\
  & \textsc{ICMSRL} Online Evol.\ & \textbf{24.0} & 12 / 50 & $+18.0$ \\
\midrule
\multirow{2}{*}{Two Body Problem}
  & \textsc{ReAct} baseline       & \phantom{0}4.0 & 2 / 50 & --- \\
  & \textsc{ICMSRL} Online Evol.\ & \textbf{14.0} & 7 / 50 & $+10.0$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/interphyre_main.tex <==
% Merged InterPhyre results table.
% Supersedes tables/headline.tex, tables/catapult_main.tex, tables/interphyre_qwen.tex
% and the inline zero-shot base-rate table in the main body.  It carries the old
% labels so that \ref's in the appendices keep resolving; the full per-family
% tables (with per-episode metrics, token ranges and significance blocks) now
% live in appendices/app_results.tex.
\begin{table}[h]
\centering
\scriptsize
\caption{%
  \textbf{A frozen skill bank is the only memory that helps a frozen actor on
  every \textsc{InterPhyre} level and every actor we measure.} Solve rate (\%)
  on 50 held-out seeds, $\pm$ one standard deviation over $n{=}3$ independently
  built memories where more than one exists. Every memory is built on the
  training seeds, \emph{frozen}, and scored on a disjoint held-out pool; no
  distillation happens at evaluation. All methods share one agentic harness and
  differ only in what is injected into the prompt, at the same position
  (baselines and protocol: Appendix~\ref{app:baselines}).
  \emph{Tokens/ep.}\ is the injected memory block, measured on \texttt{catapult}
  with the Sonnet actor. \textsc{DtE} is \texttt{down\_to\_earth}, \textsc{TBP}
  is \texttt{two\_body\_problem}, \textsc{PtP} is \texttt{pass\_the\_parcel}.
  Bold marks the best value in each column.
}
\label{tab:interphyre}
\label{tab:catapult_skillrl}
\label{tab:interphyre_qwen}
\label{tab:headline}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lccccccr}
\toprule
& \multicolumn{2}{c}{\textbf{Claude Sonnet 4.6}}
& \multicolumn{2}{c}{\textbf{Qwen2.5-7B}} & \multicolumn{2}{c}{\textbf{Qwen2.5-3B}}
& \textbf{Tokens} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\textbf{Method} & \textbf{cata.} & \textbf{PtP}
& \textbf{DtE} & \textbf{TBP} & \textbf{DtE} & \textbf{TBP} & \textbf{/ep.} \\
\midrule
\multicolumn{8}{l}{\emph{No persistent memory}}\\
\textsc{Zero-shot}
  & \phantom{0}0.0 & \phantom{0}0.0
  & 7.0 & \phantom{0}0.0 & 3.0 & 0.0 & 0 \\
\textsc{ReAct}
  & 11.0 {\tiny$\pm$3.0} & 20.0
  & 63.3 {\tiny$\pm$3.4} & 12.0 {\tiny$\pm$0.0}
  & \phantom{0}8.3 {\tiny$\pm$0.9} & \phantom{0}7.3 {\tiny$\pm$0.9} & 0 \\
Reflexion 
  & 21.3 {\tiny$\pm$2.5} & 32.0
  & 76.0 {\tiny$\pm$0.0} & 27.9 {\tiny$\pm$0.1}
  & \phantom{0}2.0 {\tiny$\pm$0.0} & \phantom{0}8.0 {\tiny$\pm$0.0} & \phantom{0,}287 \\
\midrule
\multicolumn{8}{l}{\emph{External memory}}\\
Episodic RAG
  & 62.9{\tiny$\pm$3.7} & 60.0
  & 42.7 {\tiny$\pm$11.4} & 18.7 {\tiny$\pm$7.6}
  & \phantom{0}4.0 {\tiny$\pm$4.0} & \phantom{0}5.3 {\tiny$\pm$3.1} & 6{,}513 \\
MemRL
  & 49.0{\tiny$\pm$1.0} & 46.0
  & 36.0 {\tiny$\pm$6.0} & 23.3 {\tiny$\pm$4.2}
  & \phantom{0}3.3 {\tiny$\pm$3.1} & \phantom{0}6.0 {\tiny$\pm$2.0} & 10{,}149 \\
\midrule
\textbf{\textsc{HExA}}
  & \textbf{82.7} {\tiny$\pm$9.3} & \textbf{96.0}
  & \textbf{82.7} {\tiny$\pm$5.2} & \textbf{50.0} {\tiny$\pm$3.3}
  & \textbf{23.3} {\tiny$\pm$0.9} & \textbf{12.0} {\tiny$\pm$0.0} & \textbf{2{,}392} \\
\bottomrule
\end{tabular}
\\[3pt]
\end{table}


==> tables/orbit_transfer.tex <==
\begin{table}[t]
\centering
\small
\caption{%
  \textbf{A bank built without a single target-task trajectory matches one
  trained on the target task.} Mastermind, with
  \texttt{gpt-oss-120b} as both actor and evolver. All arms play the same $n=40$
  held-out instances, so every comparison is paired. The within-task bank is
  evolved on Mastermind's own trajectories; each cross-task bank is synthesised
  from banks evolved on the named source tasks together with a short statement
  of Mastermind's rules, and never observes a Mastermind trajectory.
  \emph{Target traj.}\ counts the target-task trajectories used to build the
  bank, \emph{ep1}--\emph{ep3} are per-episode success rates, \texttt{any} is
  success in at least one of the three episodes, and \emph{Tokens} is the size
  of the injected memory block. Bold marks the best value per column.
}
\label{tab:orbit_transfer_full}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcccccr}
\toprule
\textbf{Arm} & \textbf{Target traj.} & \textbf{ep1} & \textbf{ep2} & \textbf{ep3} & \textbf{\texttt{any}} & \textbf{Tokens} \\
\midrule
No memory                               & ---     & .100 & .317 & .650 & .683 & 0 \\
\textsc{HExA} (within-task)             & 1{,}530 & .058 & .408 & \textbf{.875} & \textbf{.883} & 971 \\
\midrule
\textbf{Cross-task $\leftarrow$ Wordle}          & \textbf{0} & .092 & .467 & \textbf{.933} & \textbf{.933} & 946 \\
Cross-task $\leftarrow$ Minesweeper              & 0 & .058 & .267 & .825 & .833 & --- \\
Cross-task $\leftarrow$ Minesweeper\,$+$\,Wordle & 0 & .083 & .300 & .808 & .808 & --- \\
\bottomrule
\end{tabular}
\\[3pt]
{\small Cross-task $\leftarrow$ Wordle vs.\ no memory $+$28.3 ep3, significant in
 9/9 run-pairs; vs.\ the within-task bank $+$5.8 ep3, 0/9 --- the two are
 indistinguishable at $n{=}40$.}
\end{table}


==> tables/zeroshot_baserates.tex <==
% Zero-shot base rates (was inline in the main body; moved to the appendix).
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{%
  \textbf{Base solve rate (\%) with no interaction.}
  baseline shows each model one scripted \texttt{get\_level\_state} readout
  (exact object positions, sizes and dynamic flags) and requires a placement in
  a single turn, with no tools of its own, no probes and no environment
  feedback; it bounds how far parametric physics reasoning goes without
  interaction. \emph{Rand} samples
  uniformly from the valid placement region. The two underlined levels are the
  hard tier: every model scores $0\%$ on both.
  \textsuperscript{$\dagger$}\,Pass the Parcel and Catapult over 50 seeds; all
  others over 100.
}
\label{tab:direct_baseline_results_main}
\begin{tabular}{lcccccc}
\toprule
& \textbf{Rand} & \textbf{Q-3B} & \textbf{Q-7B} & \textbf{O-20B} & \textbf{O-120B} & \textbf{Sonnet} \\
\midrule
Cliffhanger                 & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0             \\
Tipping Point               & 3  & 0.0  & 3.0  & 8.0  & 2.0  & 0.0             \\
Basket Case                 & 4  & 0.0  & 2.0  & 14.0 & 13.0 & 19.0             \\
Down to Earth               & 8  & 3.0 & 7.0  & 5.9 & 3.0  & 14.0            \\
Two Body                    & 14 & 0.0  & 0.0 & 0.0 & 1.0  & 68.0            \\
Falling in Place            & 1  & 0.0  & 1.0  & 3.0  & 29.0 & 33.0            \\
\underline{Pass the Parcel} & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0$^{\dagger}$ \\
\underline{Catapult}        & 0  & 0.0  & 0.0  & 0.0  & 0.0  & 0.0$^{\dagger}$ \\
\bottomrule
\end{tabular}
\end{table}

